A Satake isomorphism in characteristic p

Suppose that G is a connected reductive group over a p-adic field F, that K is a hyperspecial maximal compact subgroup of G(F), and that V is an irreducible representation of K over the algebraic closure of the residue field of F. We establish an analogue of the Satake isomorphism for the Hecke algebra of compactly supported, K-biequivariant functions f: G(F) \to End V. These Hecke algebras were first considered by Barthel-Livne for GL_2. They play a role in the recent mod p and p-adic Langlands correspondences for GL_2(Q_p), in generalisations of Serre's conjecture on the modularity of mod p Galois representations, and in the classification of irreducible mod p representations of unramified p-adic reductive groups.

==> arrsy.tex <==
%  arrsy.tex
%  Anders G S Svensson
%  $Date: 1995/03/31 21:55:00 $
%  $Revision: 1.13 $

\chardef\ArrsycodE=\catcode`\@
\catcode`\@=11

\def\@@bailout@@{\message{again}\catcode`\@=\ArrsycodE\endinput}

\ifx\@@agss@arrsy@@\relax
\else
   \let\@@agss@arrsy@@\relax
   \let\@@bailout@@\relax
\fi

\@@bailout@@


\font\A@tenarr=arrsy10
\font\A@sevenarr=arrsy10 at 7pt
\font\A@fivearr=arrsy10 at 5pt

\newfam\arrfam

\textfont\arrfam=\A@tenarr
\scriptfont\arrfam=\A@sevenarr
\scriptscriptfont\arrfam=\A@fivearr

\let\cmrightarrow\rightarrow
\let\cmleftarrow\leftarrow
\let\cmleftrightarrow\leftrightarrow
\let\cmleftharpoonup\leftharpoonup
\let\cmleftharpoondown\leftharpoondown
\let\cmrightharpoonup\rightharpoonup
\let\cmrightharpoondown\rightharpoondown

\def\hex#1{\ifcase#1 0\or 1\or 2\or 3\or 4\or 5\or 6\or 7\or 8\or 9\or
   A\or B\or C\or D\or E\or F\fi}

\edef\A@arrsy{\hex\arrfam}

\def\A@newarrow#1#2#3#4{%
   \expandafter\mathchardef\csname A@#1\endcsname="#2\A@arrsy#3#4
   \expandafter\expandafter\expandafter\let\expandafter\expandafter
      \csname #1\endcsname\csname A@#1\endcsname}

\A@newarrow{Rightharpoonup}300
\A@newarrow{Leftharpoondown}301
\A@newarrow{Upharpoonleft}302
\A@newarrow{Downharpoonright}303
\A@newarrow{Rightharpoondown}304
\A@newarrow{Leftharpoonup}305
\A@newarrow{Upharpoonright}306
\A@newarrow{Downharpoonleft}307
\A@newarrow{Rrightarrow}308
\A@newarrow{Lleftarrow}309
\A@newarrow{Rrelbar}30A
\A@newarrow{dashbar}30B
\A@newarrow{shortrightarrow}30C
\A@newarrow{shortleftarrow}30D
\A@newarrow{rightmonotail}30E
\A@newarrow{leftmonotail}30F
\A@newarrow{squiggle}310
\A@newarrow{rightarrow}311
\A@newarrow{leftarrow}312
\A@newarrow{leftrightarrow}313
\A@newarrow{leftharpoonup}314
\A@newarrow{leftharpoondown}315
\A@newarrow{rightharpoonup}316
\A@newarrow{rightharpoondown}317
\edef\vect{\mathaccent"0\A@arrsy 18 }
\mathchardef\comp="3\A@arrsy 19
\mathchardef\dotp="3\A@arrsy 1A
\mathchardef\cupp="3\A@arrsy 1B
\mathchardef\capp="3\A@arrsy 1C

\let\of\comp

\let\gets\leftarrow
\let\to\rightarrow

\def\cmarrows{\let\leftrightarrow\cmleftrightarrow
   \let\rightarrow\cmrightarrow\let\leftarrow\cmleftarrow
   \let\gets\leftarrow\let\to\rightarrow
   \let\leftharpoonup\cmleftharpoonup
   \let\leftharpoondown\cmleftharpoondown
   \let\rightharpoonup\cmrightharpoonup
   \let\rightharpoondown\cmrightharpoondown}

\def\rightepi{\A@rightarrow\mkern-13mu\A@shortrightarrow\mkern3mu}
\let\epito\rightepi
\def\leftepi{\A@leftarrow\mkern-15mu\A@shortleftarrow\mkern5mu}
\let\A@rightepi\rightepi \let\A@leftepi\leftepi

\def\rightmono{\A@rightmonotail\mkern-8mu\relbar\mkern-8mu\A@shortrightarrow}
\let\monoto\rightmono
\def\leftmono{\A@shortleftarrow\mkern-8mu\relbar\mkern-8mu\A@leftmonotail}

\def\rightiso{\A@rightmonotail\mkern-5mu\A@shortrightarrow
   \mkern-7mu\A@shortrightarrow}
\let\isoto\rightiso
\def\leftiso{\A@shortleftarrow\mkern-7mu\A@shortleftarrow
   \mkern-5mu\A@leftmonotail}

\def\longrightepi{\relbar\joinrel\A@rightepi}
\def\longleftepi{\A@leftepi\joinrel\relbar}

\def\longrightmono{\A@rightmonotail\mkern-7mu\relbar\mkern-6mu\A@rightarrow}
\def\longleftmono{\A@leftarrow\mkern-6mu\relbar\mkern-7mu\A@leftmonotail}

\def\longrightiso{\A@rightmonotail\mkern-7mu\relbar\mkern-6mu\A@rightepi}
\def\longleftiso{\A@leftepi\mkern-6mu\relbar\mkern-7mu\A@leftmonotail}

\def\Longrightharpoonup{\Relbar\joinrel\A@Rightharpoonup}
\def\Longrightharpoondown{\Relbar\joinrel\A@Rightharpoondown}
\def\Longleftharpoonup{\A@Leftharpoonup\joinrel\Relbar}
\def\Longleftharpoondown{\A@Leftharpoondown\joinrel\Relbar}
\def\Llongrightarrow{\A@Rrelbar\joinrel\A@Rrightarrow}
\def\Llongleftarrow{\A@Lleftarrow\joinrel\A@Rrelbar}
\def\Llongrelbar{\A@Rrelbar\joinrel\A@Rrelbar}

\let\Leftallo\Leftharpoondown
\let\Leftpara\Leftharpoonup
\let\Rightallo\Rightharpoonup
\let\Rightpara\Rightharpoondown

\let\Longleftallo\Longleftharpoondown
\let\Longleftpara\Longleftharpoonup
\let\Longrightallo\Longrightharpoonup
\let\Longrightpara\Longrightharpoondown

\catcode`\@=\ArrsycodE


==> kuvio.tex <==
%  kuvio.tex
%  patchlevel 216
%
%%
%%  Copyright (C) 1994-1996  Anders G S Svensson <svensson@math.ubc.ca>
%%
%%  The file kuvio.tex may be freely distributed and used, with the
%%  following restrictions.
%%
%%  1. Substantial use of kuvio.tex in any published work should be suitably
%%     acknowledged.
%%
%%  2. No changes or modifications are to be made to kuvio.tex.
%%
%%  3. The documentation, "Typesetting diagrams with kuvio.tex", must
%%     be distributed with kuvio.tex.
%%
%%  I would enjoy receiving a copy of any book, journal article or thesis
%%  prepared using kuvio.tex.
%%
%%  Thank you.
%%
\chardef\kuvioletter=\catcode`\@\catcode`\@=11
\chardef\K@aa=\catcode`\? \catcode`\?=7
\gdef\K@ab{\global\let\K@ab\kuviobye}%
\gdef\kuviobye{\gdef\D@kuviolevel{0}%
\K@ac\@\kuvioletter\K@ac\?\K@aa
\K@ac\~\K@ad\K@ac\??Z\K@ae
\K@ac\??Y\K@af\K@ac\??X\K@ag
\K@ac\??W\K@ah\K@ac\??V\K@ai
\K@ac\??U\K@aj\K@ac\??T\K@ak
\K@ac\??S\K@al\K@ac\??R\K@am
\K@ac\??Q\K@an\K@ac\??P\K@ao
\K@ac\??O\K@ap\K@ac\??N\K@aq
\K@ac\??A\K@ar
\endinput}%
\gdef\K@as#1#2{\chardef#2=\catcode`#1 \catcode`#1=14 }%
\K@as\~\K@ad\K@as\??Z\K@ae
\K@as\??Y\K@af\K@as\??X\K@ag
\K@as\??W\K@ah\K@as\??V\K@ai
\K@as\??U\K@aj\K@as\??T\K@ak
\K@as\??S\K@al\K@as\??R\K@am
\K@as\??Q\K@an\K@as\??P\K@ao
\K@as\??O\K@ap\K@as\??N\K@aq
\K@as\??A\K@ar
\ifx\D@kuvioloaded\relax
\ifcase\D@kuviolevel\relax
\gdef\K@ab{\message{again}\kuviobye}%
\or\relax
\or\catcode`\??Z=9 \or\catcode`\??Y=9 \or\catcode`\??X=9
\or\catcode`\??W=9 \or\catcode`\??V=9 \or\catcode`\??U=9
\or\catcode`\??T=9 \or\catcode`\??S=9 \or\catcode`\??R=9
\or\catcode`\??Q=9 \or\catcode`\??P=9 \or\catcode`\??O=9
\or\catcode`\??N=9 \or\catcode`\??A=9
\fi
\else
\chardef\K@at=\catcode`\( \chardef\K@au=\catcode`\_
\chardef\K@av=\catcode`\^ \chardef\K@aw=\catcode`\<
\chardef\K@ax=\catcode`\> \chardef\K@ay=\catcode`\:
\chardef\K@az=\catcode`\/ \chardef\K@ba=\catcode`\*
\chardef\K@bb=\catcode`\| \gdef\D@kuviolevel{1}%
\catcode`\~=9 \let\D@kuvioloaded\relax\global\let\K@ab\relax
\fi
\K@ab
~\def\kuviocs#1{%
~{\escapechar=-1
~\expandafter\ifx\csname D@\string#1@k@D\endcsname\relax
~\xdef\K@bc{\string#1}\else\xdef\K@bc{D@\string#1@k@D}\fi
~}\csname\K@bc\endcsname}
~\def\nonkuviocs#1{%
~{\escapechar=-1
~\expandafter\ifx\csname D@\string#1@nk@D\endcsname\relax
~\xdef\K@bc{\string#1}\else\xdef\K@bc{D@\string#1@nk@D}\fi
~}\csname\K@bc\endcsname}
~\def\K@bd#1#2{%
~{\escapechar=-1
~\expandafter\ifx\csname\string#2\endcsname\relax
~\xdef\K@bc{\string#2}\else
~\aftergroup\K@be\aftergroup#2\xdef\K@bc{D@\string#2@k@D}\fi
~}\def\K@bf{#1}\expandafter\K@bf\csname\K@bc\endcsname}
~\def\K@bg{\K@bd\def}
~\def\K@bh{\K@bd\let}
~\def\K@bi#1#2{%
~{\escapechar=-1
~\expandafter\ifx\csname\string#2\endcsname\relax
~\else\expandafter\expandafter\expandafter\let\expandafter\expandafter
~\csname D@\string#2@nk@D\endcsname\csname\string#2\endcsname
~\aftergroup\K@bj\aftergroup#2\fi
~\xdef\K@bc{\string#2}%
~}\def\K@bf{#1}\expandafter\K@bf\csname\K@bc\endcsname}
~\def\K@bk{\K@bi\def}
~\def\K@bl{\K@bi\let}
~\def\K@bm#1#2{%
~{\escapechar=-1
~\expandafter\ifx\csname\string#1\endcsname\relax
~\xdef\K@bc{\string#1}\else
~\aftergroup\K@be\aftergroup#1\xdef\K@bc{D@\string#1@k@D}\fi
~\expandafter\ifx\csname D@\string#2@k@D\endcsname\relax
~\xdef\K@bf{\string#2}\else\xdef\K@bf{D@\string#2@k@D}\fi
~}\expandafter\expandafter\expandafter\let\expandafter\expandafter
~\csname\K@bc\endcsname\csname\K@bf\endcsname}
~\let\kuviodef\K@bg\let\rekuviodef\K@bk
~\let\kuviolet\K@bh\let\rekuviolet\K@bl
~\let\kuviodefine\K@bd\let\rekuviodefine\K@bi
~\def\kuvioforce#1{%
~{\escapechar=-1
~\expandafter\ifx\csname D@\string#1@k@D\endcsname\relax
~\else\xdef\K@bc{\let\noexpand#1\expandafter\noexpand
~\csname D@\string#1@k@D\endcsname\let\expandafter\noexpand
~\csname D@\string#1@k@D\endcsname\relax}\aftergroup\K@bc\fi
~}}
~\def\K@be#1{\immediate\write16
~{** \ifnum\D@kuviolevel=1 \else(kuvio.tex) \fi
~\string#1\K@bn already defined: use \string\kuviocs\string#1}}
~\def\K@bj#1{\immediate\write16
~{** \ifnum\D@kuviolevel=1 \else(kuvio.tex) \fi
~\string#1\K@bn redefined}}
~\def\K@bn{ }
~{\newlinechar=`\!\catcode`\ =13 \let \K@bn
~\immediate\write16{***************************************************
~!**  Diagrams for dvips users                     **
~!**  patchlevel 216, 19 Feb 1996                  **
~!**  Anders G S Svensson  <svensson@math.ubc.ca>  **
~!***************************************************}}
~\def\K@ac#1#2{\catcode`#1=#2\relax}\def\K@bo{\K@bp{2}{rotation}\global\let
~\K@bo\relax}\def\K@bq{\K@bp{3}{frames and shades}\global\let\K@bq\relax
~}\def\K@br{\K@bp{4}{figures and graphs}\global\let\K@br\relax}\def\K@bs
~{\K@bp{5}{shifts}\global\let\K@bs\relax}\def\K@bt{\K@bp{6}{diagrams}\global
~\let\K@bt\relax}\def\K@bu{\K@bp{7}{kdg files}\global\let\K@bu\relax}\def
~\K@bv{\K@bp{8}{kuv files}\global\let\K@bv\relax}\def\K@bw{\K@bp
~{9}{modification cells}\global\let\K@bw\relax}\def\K@bx{\K@bp{10}{text
~modifications}\global\let\K@bx\relax}\def\K@by{\K@bp
~{11}{modifications}\global\let\K@by\relax}\def\K@bz{\K@bp{12}{rotated
~labels}\global\let\K@bz\relax}\def\K@ca{\K@bp{13}{points}\global\let\K@ca
~\relax}\def\K@cb{\K@bp{14}{box and frame modifications}\global\let\K@cb
~\relax}\def\K@cc{\K@bp{15}{dots}\global\let\K@cc\relax}\def\K@bp#1#2{\gdef
~\D@kuviolevel{#1}\gdef\K@cd{\message{#2}}\input kuvio.tex\relax}\def
~\kuviofmt{\xdef\K@bc{\everyjob={\the\everyjob\message{** kuvio.tex (p216)
~Anders G S Svensson **}}}\K@bc\K@bo\K@bq\K@br\K@bs\K@bt\K@bu\K@bv\K@bw
~\K@bx\K@by\K@bz\K@ca\K@cb\K@cc\let\kuviofmt\relax}\def\K@ce{\K@cd\catcode
~`\(=\K@at\catcode`\_=\K@au\catcode`\^=\K@av\catcode`\<=\K@aw\catcode
~`\>=\K@ax\catcode`\:=\K@ay\catcode`\/=\K@az\catcode`\*=\K@ba\catcode
~`\|=\K@bb\let\K@cf\let\def\let{\global\K@cf}\K@cf\def\gdef}\K@bk
~\dvipsspecial#1{\special{ps:#1}}\def\kuviospecial{\let\K@cg}\kuviospecial
~\dvipsspecial\def\kuvio{{\tt kuvio.tex}}\def\kuviopatchlevel{216}\def
~\kuviodate{19 Feb 1996}\newhelp\K@ch{Expect chaos to ensue.}\def
~\kuviorequire#1{\relax\ifnum#1>\kuviopatchlevel\relax\errhelp=\K@ch
~\errmessage{Hmm. Looks like I'll need a newer patchlevel of kuvio.tex.}\fi
~}\def\K@ci{}\def\K@cj#1{}\def\K@ck#1#2{}\def\K@cl{{}}\def\K@cm{0}\def\K@cn
~{.5}\def\K@co{1}\def\K@cp{-1}\def\K@cq#1#2{#1#2}\def\K@cr#1#2{#2#1}\def
~\K@cs#1#2{{#2}{#1}}\def\K@ct#1#2{\let\K@bf#1\let#1#2\let#2\K@bf}\def\K@cu
~#1\K@cv{\def\K@cw{#1}\K@cx}\def\K@cx{\K@cw\let\K@cy\K@cx\else\let\K@cy
~\relax\fi\K@cy}\let\K@cv\fi\newif\ifkuvio@\def\K@cz{\relax\kuvio@false
~}\newwrite\K@da\newwrite\K@db\newread\K@dc\newread\K@dd\newcount\K@de
~\newcount\K@df\newcount\K@dg\newcount\K@dh\newcount\K@di\newcount\K@dj
~\newcount\K@dk\newcount\K@dl\newdimen\K@dm\newdimen\K@dn\newdimen\K@do
~\newdimen\K@dp\newtoks\K@dq\newtoks\K@dr\newbox\K@ds\newbox\K@dt
~\newbox\K@du
??V\begingroup\K@ce\def\K@dv#1{\bgroup\K@dw\K@dx{\K@dy\K@dr}{\the\K@dr}\def
??V\K@dz{\egroup\egroup\egroup\K@ea}\def\Modify{\egroup\egroup\egroup\K@by
??V\K@eb}\let\K@ec\relax\let\K@ed\relax\let\K@ee\relax\K@ef\setbox\K@du
??V=\hbox\bgroup\vbox\bgroup\halign\bgroup&\K@eg\K@eh{##}\cr}\def\endDiagram
??V{\K@dz\egroup}%
~\def\K@ei{\K@dv}\K@bk\Diagram{\bgroup\K@bt\K@ej\K@ek\K@el\everyDiagram
~\K@ei{Diagram}}\K@bl\everyDiagram\relax
??V\def\K@ea{\K@em\global\setbox\K@ds=\hbox{\hbox to \K@en sp{\hfil\vbox to
??V\K@eo sp{\vfil}}\K@ep\K@eq\K@er}\K@dx{}{{}{1}{\gdef\noexpand\K@es{\K@es
??V}\gdef\noexpand\K@et{\K@et}\gdef\noexpand\K@eu{\K@eu}\gdef\noexpand\K@ev
??V{\K@ev}}}\K@ew\K@ex\K@ey\egroup\Displaybox\K@ds}%
~\let\K@ew\relax\let\K@dw\relax\let\K@dx\K@ck\K@bg\compileto{\bgroup\K@ez
~\K@fa}\def\K@fa#1{\egroup\def\K@ej{\K@fb{#1}\global\let\K@ej\relax\let
~\K@ek\relax}}\def\K@ez{\catcode`\ =9 \catcode`\??I=9 }\K@bg\recompileto
~{\bgroup\K@ez\K@fc}\def\K@fc#1{\egroup\def\K@ej{\K@fd{#1}\global\let\K@ej
~\relax\let\K@ek\relax}}\K@bg\recompile{\let\K@fb\K@fd}\K@bg\nocompile{\let
~\K@fe\K@ck}\K@bg\forcekdg{\def\K@el{\def\K@ei{\K@ff}\def\K@fg{\K@fh}\def
~\K@fi{\K@fj}\K@bu}}\let\K@el\relax\def\K@fb#1{\K@fe0{#1}}\def\K@fd#1{\K@fe
~1{#1}}\K@bg\autocompileto{\bgroup\K@ez\K@fk}\def\K@fk#1{\egroup\K@fl
~\autocompilecounter\def\K@ek{\global\advance\autocompilecounter by 1 \K@fb
~{#1-\the\autocompilecounter}}}\K@bg\autocompile{\kuviocs\autocompileto
~{.\jobname}}\let\K@ej\relax\let\K@ek\relax\edef\K@fl#1{\noexpand\newcount
~#1\gdef\noexpand\K@fl##1{\global##1=0 }}\def\K@fe#1#2{\let\K@el\relax\gdef
~\K@fm{#2}\ifcase#1 \immediate\openin\K@dc=#2.kuv \def\K@fn{\K@fd{#2}}\ifeof
~\K@dc\immediate\closein\K@dc\def\K@bc{\K@fd{#2}}\else\def\K@dw{\K@fo
~{reading #2.kuv}}\def\K@ei{\K@fp}\def\K@fg{\K@fq}\def\K@fi{\K@fr}\let\K@bc
~\K@bv\fi\or\immediate\openout\K@da=#2.kuv \let\K@dx\K@fs\def\K@dw{\K@fo
~{compiling #2.kuv}}\def\K@ei{\K@ff}\def\K@fg{\K@fh}\def\K@fi{\K@fj}\let
~\K@bc\K@bu\let\K@ew\K@ft\fi\K@bc}\def\K@fm{\jobname}\def\K@fs
~#1#2{{#1\immediate\write\K@da{#2}}}\def\K@ft{\immediate\closeout\K@da\K@fu
~{done}}\def\K@fo#1{\message{(#1}}\def\K@fu#1{\message{#1)}}
??U\begingroup\K@ce\def\K@ff{\K@fv\K@dv}\def\K@fh{\K@fv\K@fw}\def\K@fv
??U#1#2{\let\K@fo\message\let\K@fu\message\def\K@fx{\K@fy{\relax
??U}\expandafter\def\csname#2\endcsname{#1{}}\input\K@fm.kdg \K@fy
??U{}}\expandafter\expandafter\expandafter\K@fz\expandafter\expandafter
??U\csname#2\endcsname\csname end#2\endcsname\K@fx}%
~\def\K@ga#1#2#3#4{\def\K@bc##1#3{\def\K@gb{#1#2##1#3}\gdef\K@fy####1{\K@gc
~{#1#2##1#3####1}}#4}\K@bc}\def\K@fz{\K@ga{}}\def\K@gd{\K@ga{\relax}}\def
~\K@ge{\K@ga{\relax\relax}}\def\K@gc#1{\immediate\openout\K@db=\K@fm.kdg
~\K@dr={#1}\immediate\write\K@db{\the\K@dr}\immediate\closeout\K@db}%
??U\def\K@fj#1{\let\K@fo\message\let\K@fu\message\expandafter\expandafter
??U\expandafter\K@gf\expandafter\expandafter\csname#1\endcsname\csname
??Uend#1\endcsname{\K@gg{#1}}}%
~\let\K@gf\K@fz
??U\def\K@gg#1{\expandafter\expandafter\expandafter\K@gh\expandafter
??U\expandafter\csname end#1\endcsname\K@gb\Modify\K@gi\expandafter\def
??U\csname#1\endcsname{\K@gj{}}\K@fy{\relax}\input\K@fm.kdg \K@fy{}}\endgroup
~\def\K@gk#1#2#3#4#5\Modify#6\K@gi{\def\K@gl{#6}\ifx\K@gl\K@ci\def\K@bc
~##1#1{\def\K@gm####1{####1={\vbox {\offinterlineskip\hbox{$##1$}\null
~}}}}\K@bc#5\else\def\K@gm##1{##1={\vbox {\offinterlineskip\hbox
~{$#5$}\null}}}\fi}\let\K@gn\K@gk\def\K@go{\K@gk{}}\def\K@gh{\K@gk{}{}}%
??T\begingroup\K@ce\def\K@fp{\K@gp\K@gq\K@ff\K@dv}\def\K@fq{\K@gp\K@gr\K@fh
??T\K@fw}\def\K@fr{\let\K@gs\K@gt\K@gp\K@gu\K@fj\K@gj}\def\K@gp
??T#1#2#3{\immediate\read\K@dc to\K@bf\ifx\K@bf\K@gv\def\K@bc{\K@gs
??T#1#3}\else\def\K@bc{\immediate\closein\K@dc\K@fn#2}\fi\K@bc}%
~\def\kuviorevision#1{\def\K@dy##1{##1={{kuvio}{216}{#1}}}\def\K@gv
~{{kuvio}{216}{#1} }}\kuviorevision{}
??T\def\K@gs#1#2#3{\def\K@fx{\K@gw#1#2{#3}}\expandafter\expandafter
??T\expandafter\K@fz\expandafter\expandafter\csname#3\endcsname\csname
??Tend#3\endcsname\K@fx}\def\K@gw#1#2#3{\def\K@bc{\K@fy{\relax}\expandafter
??T\def\csname#3\endcsname{\K@fn#2{}}\input\K@fm.kdg \K@fy{}}\immediate\openin
??T\K@dd=\K@fm.kdg \ifeof\K@dd\immediate\closein\K@dd\immediate\closein\K@dc
??T\let\K@fo\message\let\K@fu\message\else\immediate\read\K@dd to \K@bf
??T\immediate\closein\K@dd\ifx\K@bf\K@gb\let\K@bc#1\else\immediate\closein
??T\K@dc\let\K@fo\message\let\K@fu\message\fi\fi\K@bc}\def\K@gt#1#2#3{\def
??T\K@fx{\expandafter\expandafter\expandafter\K@gh\expandafter\expandafter
??T\csname end#3\endcsname\K@gb\Modify\K@gi\K@gw#1#2{#3}}\expandafter
??T\expandafter\expandafter\K@gf\expandafter\expandafter\csname#3\endcsname
??T\csname end#3\endcsname\K@fx}\def\K@gq{\K@dw\def\K@gx{\K@gy\K@gz\let\gr
??T\K@ha}\K@hb\K@hc\K@hd\K@he\K@hf\let\stop\relax\let\grav\relax\let\base
??T\relax\K@hg\K@hh\K@hi\catcode`\@=11 \immediate\read\K@dc to\K@bf
??T\expandafter\K@hj\K@bf\K@fu{done}\K@ex\K@ey\egroup\Displaybox\K@ds}\def
??T\K@gr{\let\K@hk\K@hl\let\K@hm\K@hj\K@gu}\def\K@hj#1#2#3#4#5 {\def\K@en
??T{#1}\def\K@hn{#5}\def\K@ho{#3}\def\K@hp{#4}\global\setbox\K@ds=\hbox{\hbox
??Tto #1sp{\hfil\vbox to #2sp{\vfil}}\K@hq}}\def\K@gu{\K@dw\def\K@gx{\let\gr
??T\K@ha}\catcode`\@=11 \immediate\read\K@dc to\K@bf\expandafter\K@hm\K@bf
??T\K@fu{done}\K@ex\K@hr\egroup\Displaybox\K@ds}\def\K@hm#1#2#3#4 {\def\K@en
??T{#1}\def\K@hp{#4}\global\setbox\K@ds=\hbox{\hbox to #1sp{\hfil\vbox to
??T#2sp{\vfil}}\K@hq}}\def\K@hq{\immediate\read\K@dc to\K@bf\ifeof\K@dc\def
??T\K@bc{\immediate\closein\K@dc}\else\def\K@bc{\expandafter\K@hs\K@bf\K@hq
??T}\fi\K@bc}\def\K@hs#1#2#3 {\def\K@bf{#1}\ifx\K@bf\K@ci\def\K@bc
??T##1{{##1\ifnum#2=0 \immediate\read\K@dc to\K@bf\expandafter\K@ht\K@bf\fi
??T}}\else\def\K@bc{\K@hu{#1}{#2}}\fi\K@bc{#3}}\def\K@ht#1#2#3 {\K@hu
??T{#1}{#2}{#3}}\def\K@hu#1#2#3{\llap{\hbox to \K@en sp{\hskip#1 \smash{\hbox
??T{\raise#2\hbox{\K@hv#3}}}\hss}}}\endgroup
~\K@bk\newDiagram{\bgroup\K@ez\K@hw}\def\K@hw#1{\egroup\expandafter\ifx
~\csname D@every#1@\endcsname\relax\expandafter\expandafter\expandafter\let
~\expandafter\expandafter\csname D@@#1@@\endcsname\csname#1\endcsname
~\expandafter\def\csname D@every#1@\endcsname{\expandafter\expandafter
~\expandafter\let\expandafter\expandafter\csname#1\endcsname\csname
~D@@#1@@\endcsname}\fi\expandafter\K@bk\csname#1\endcsname{\bgroup\K@bt
~\csname D@every#1@\endcsname\K@ej\K@ek\K@el\everyDiagram\csname
~every#1\endcsname\K@ei{#1}}\expandafter\K@bk\csname end#1\endcsname{\K@dz
~\egroup}\expandafter\let\csname every#1\endcsname\relax}
??V\def\K@ef{\K@df=-1\relax\K@de=-1\relax\let\K@hx\K@cp\everycr{\noalign
??V{\global\advance\K@df by 1\relax\ifnum\K@hx<\K@de\xdef\K@hx{\the\K@de}\fi
??V\global\K@de=-1}}\global\K@dg=0 \global\K@dh=0 \let\K@hy\K@ci\let\K@hz
??V\K@ci\let\K@ia\K@ci\let\K@ib\K@ci\let\K@ic\K@ci\let\K@id\K@ci\let\K@ie
??V\K@ci\let\K@if\K@ci\let\K@ig\K@ci\let\K@ih\K@ci\let\K@ii\K@ci\global
??V\let\K@ij\relax\global\let\K@hn\K@cp\global\let\K@ik\K@ci\K@il\let\\\cr
??V\let\K@es\K@cp\let\K@et\K@cp\let\K@eu\K@cm\let\K@ev\K@cm\let\K@im\K@cm
??V\let\K@in\K@ci\K@hg\K@hd\K@he\K@hb\K@gy\let\gr\K@ha}%
~\def\K@hb{\let\K@io(\let\K@ip\(\catcode`\(=\active\let\K@iq_\let\K@ir
~\_\catcode`\_=\active\let\K@is^\let\K@it\^\catcode`\^=\active\let\K@iu
~<\let\K@iv\<\catcode`\<=\active\let\K@iw>\let\K@ix\>\catcode`\>=\active
~\let\K@iy:\let\K@iz\:\catcode`\:=\active}{\catcode`\(=\active\catcode
~`\_=\active\catcode`\^=\active\catcode`\<=\active\catcode`\>=\active
~\catcode`\:=\active\gdef\K@ja{\let(\K@jb\let<\K@jc\let>\K@jd\let_\K@je
~\let^\K@jf\let:\K@jg\let\((\let\__\let\^^\let\<<\let\>>\let\::} \gdef
~\K@gy{\let(\K@io\let\(\K@ip\let_\K@iq\let\_\K@ir\let^\K@is\let\^\K@it
~\let<\K@iu\let\<\K@iv\let>\K@iw\let\>\K@ix\let:\K@iy\let\:\K@iz} \gdef
~\K@hc{\def(##1,##2){}\let_\K@jh\let^\K@jh\let<\K@jh\let>\K@jh\let:\K@cj
~\let\((\let\__\let\^^\let\<<\let\>>\let\::} \gdef\K@ji{\let(\K@jj\let
~_\K@jk\let^\K@jl\let<\K@jm\let>\K@jn\let:\K@jo} }\def\K@jj{(}\def\K@jk
~{_}\def\K@jl{^}\def\K@jm{<}\def\K@jn{>}\def\K@jo{:}\def\K@jh{\def\K@jp
~##1{\K@cj}\let\K@jq\K@cj\futurelet\K@jr\K@js}\def\K@hg{\let\K@jt\dh\let
~\K@ju\dt\let\K@jv\up\let\K@jw\rt\let\K@jx\mv\let\K@jy\nl\let\K@jz\ru
~\let\K@ka\rr\let\K@kb\rm\let\K@kc\ro\let\K@kd\pt\let\K@ke\fd\let\K@kf
~\rl\let\K@kg\br\let\K@kh\pp\let\K@ki\jt\let\K@kj\jh\let\K@kk\jn\let
~\K@kl\rw\let\K@km\hx\let\K@kn\hy\let\K@ko\tx\let\K@kp\ty\let\K@kq\fx
~\let\K@kr\fy\let\K@ks\ts\let\K@kt\hs\let\K@ku\fs\let\K@kv\tr\let\K@kw
~\hr\let\K@kx\fr\let\K@ky\db\let\K@kz\lb\let\K@la\rb\let\K@lb\nw\let
~\K@lc\tl\let\K@ld\hd\let\K@le\pl\let\K@lf\pd\let\K@lg\lw}\def\K@lh{\let
~\dh\K@li\let\dt\K@lj\let\up\K@lk\let\rt\K@ll\let\mv\K@lm\let\nl\K@ln
~\let\ru\K@lo\let\rr\K@lp\let\rm\K@lq\let\ro\K@lr\let\pt\K@ls\let\fd
~\K@lt\let\rl\K@lu\let\br\K@lv\let\pp\K@lw\let\jt\K@lx\let\jh\K@ly\let
~\jn\K@lz\let\rw\K@ma\let\K@mb\K@mc\let\K@md\K@me\let\hx\K@mf\let\hy
~\K@mg\let\tx\K@mh\let\ty\K@mi\let\fx\K@mj\let\fy\K@mk\let\ts\K@ml\let
~\hs\K@mm\let\fs\K@mn\let\tr\K@mo\let\hr\K@mp\let\fr\K@mq\let\db\K@mr
~\let\lb\K@ms\let\rb\K@mt\let\nw\K@mu\let\lw\K@mv}\def\K@gz{\let\dh\K@jt
~\let\dt\K@ju\let\up\K@jv\let\rt\K@jw\let\mv\K@jx\let\nl\K@jy\let\ru
~\K@jz\let\rr\K@ka\let\rm\K@kb\let\ro\K@kc\let\pt\K@kd\let\fd\K@ke\let
~\rl\K@kf\let\br\K@kg\let\pp\K@kh\let\jt\K@ki\let\jh\K@kj\let\jn\K@kk
~\let\rw\K@kl\let\K@mb\K@kl\let\K@md\K@kl\let\hx\K@km\let\hy\K@kn\let
~\tx\K@ko\let\ty\K@kp\let\fx\K@kq\let\fy\K@kr\let\ts\K@ks\let\hs\K@kt
~\let\fs\K@ku\let\tr\K@kv\let\hr\K@kw\let\fr\K@kx\let\db\K@ky\let\lb
~\K@kz\let\rb\K@la\let\nw\K@lb\let\tl\K@lc\let\hd\K@ld\let\pl\K@le\let
~\pd\K@lf\let\lw\K@lg}\def\K@hh{\let\dh\K@cj\let\dt\K@cj\let\up\K@cj\let
~\rt\K@cj\let\mv\K@cj\let\nl\relax\let\ru\K@cj\let\rr\K@cj\let\rm\K@cj
~\let\ro\relax\let\pt\K@cj\let\fd\K@cj\let\rl\relax\let\br\relax\let\pp
~\relax\let\jt\relax\let\jh\relax\let\jn\relax\let\rw\K@cj\let\K@mb
~\K@cj\let\K@md\K@cj\let\hx\K@cj\let\hy\K@cj\let\tx\K@cj\let\ty\K@cj
~\let\fx\K@cj\let\fy\K@cj\let\ts\K@cj\let\hs\K@cj\let\fs\K@cj\let\tr
~\K@cj\let\hr\K@cj\let\fr\K@cj\let\db\relax\let\lb\relax\let\rb\relax
~\let\nw\relax\let\lw\K@jh}
??V\def\K@mw#1{\xdef\K@hy{\K@hy{\the\K@de}{#1}}}\def\K@mx#1{\relax\K@di=\K@df
??V\multiply\K@di by -1 \advance\K@di by \K@ho\xdef\K@hz{{\the\K@di}{#1}\K@hz
??V}}\def\K@my#1{\xdef\K@ia{\K@ia{\the\K@de}{#1}}}\def\K@mz#1{\relax\K@di
??V=\K@df\multiply\K@di by -1 \advance\K@di by \K@ho\xdef\K@ib{{\the\K@di
??V}{#1}\K@ib}}\def\K@na#1{\xdef\K@ic{\K@ic{\the\K@de}{#1}}}\def\K@nb{\xdef
??V\K@id{\K@id{\the\K@df}{\the\K@de}}}\def\K@nc{\xdef\K@ie{\K@ie{\the\K@df
??V}{\the\K@de}}}\def\K@nd{\xdef\K@if{\K@if{\the\K@df}{\the\K@de}}}\def\K@ne
??V{\xdef\K@ig{\K@ig{\the\K@df}{\the\K@de}}}\def\K@nf{\xdef\K@ih{\K@ih{\the
??V\K@df}{\the\K@de}}}\def\K@ng{\xdef\K@ii{\K@ii{\the\K@df}{\the\K@de}}}\def
??V\K@nh{\global\let\K@ni\K@co}\def\K@nj{\xdef\K@ij{\the\K@de}}\def\K@nk{\xdef
??V\K@hn{\the\K@df}}\def\K@nl{\def\grav{\relax\K@nj}\def\base{\relax\K@nk
??V}}\def\K@nm{\let\K@nj\relax\let\K@nk\relax}\def\K@hd{\let\K@nn\stop\let
??V\K@no\grav\let\K@np\base\let\K@nq\safe\let\K@nr\nodot\let\K@ns\dx\let
??V\K@nt\dy\let\K@nu\dl\let\K@nv\dr\let\K@nw\mx\let\K@nx\my\let\K@ny\ml
??V\let\K@nz\mr\let\K@oa\ax\let\K@ob\al\let\K@oc\ar}\def\K@he{\K@nl\def
??V\stop{\relax\K@nh}\def\safe{\relax\K@od}\def\nodot{\relax\K@oe}\def\dl
??V{\relax\K@nb}\def\dr{\relax\K@nc}\def\ml{\relax\K@nd}\def\mr{\relax\K@ne
??V}\def\al{\relax\K@nf}\def\ar{\relax\K@ng}\def\mx{\relax\K@my}\def\my
??V{\relax\K@mz}\def\dx{\relax\K@mw}\def\dy{\relax\K@mx}\def\ax{\relax\K@na
??V}}\def\K@hf{\let\K@nb\relax\let\K@nc\relax\let\K@nd\relax\let\K@ne
??V\relax\let\K@nf\relax\let\K@ng\relax\let\K@my\K@cj\let\K@mz\K@cj\let
??V\K@mw\K@cj\let\K@mx\K@cj\let\K@na\K@cj}\def\K@of{\let\stop\K@nn\let\grav
??V\K@no\let\base\K@np\let\safe\K@nq\let\nodot\K@nr\let\dx\K@ns\let\dy
??V\K@nt\let\dl\K@nu\let\dr\K@nv\let\mx\K@nw\let\my\K@nx\let\ml\K@ny\let
??V\mr\K@nz\let\ax\K@oa\let\al\K@ob\let\ar\K@oc}\def\K@od#1{{\K@of#1}}%
~\def\K@jb#1,#2){\gdef\K@og{#1@#2}}\def\K@jc{\K@oh0}\def\K@jd{\K@oh1}\def
~\K@je{\K@oh2}\def\K@jf{\K@oh3}\def\K@oh#1{\def\K@jp##1{\let\K@oi\K@cl\let
~\K@oj\K@cl\let\K@ok\K@cl\K@ol##1;@\K@oi\K@oj\K@ok\edef\K@bc{\noexpand
~\K@om {#1{\K@oi}{\K@oj}{\K@ok}}}\K@bc} \def\K@jq{\K@om{#1}}\futurelet\K@jr
~\K@js}\def\K@om#1#2{\K@dr={#1@#2}\K@on}\def\K@oo#1#2{\K@dr={#1@#2}\def\K@bc
~{\K@op#1{{}}@{#2}\K@on}\ifnum\K@oq=1\relax\else\ifnum\K@oq=5\relax\else
~\let\K@bc\K@on\fi\fi\K@bc}\def\K@op#1#2#3@#4{\setbox\K@dt\hbox{$\K@gx
~\labelstyle\hskip\K@or sp\hskip\K@os{\K@ot}{}sp \hskip\K@ou sp \hskip\K@ov
~{\K@ot}{}sp \hskip\K@ow#4\hskip\K@ow\hskip\K@os{\K@ot}{}sp\hskip\K@or sp
~\hskip\K@ov{\K@ot}{}sp \hskip\K@ou sp$}\K@di=\wd\K@dt\xdef\K@ox{\K@ox
~{#2}{\the\K@di}}}\def\K@oy#1{\if\noexpand\K@jr\noexpand#1\let\K@bc\K@oz
~\else\if\noexpand\K@jr\K@bn\def\K@bc{\K@pa\futurelet\K@jr\K@js @}\else
~\let\K@bc\K@jq\fi\fi\K@bc}\def\OptDelim#1#2{\def\K@oz#1##1#2{\K@jp
~{##1}}\def\K@js{\K@oy{#1}}}\OptDelim[] \def\K@on{\edef\K@bc{\global\K@dq
~={\the\K@dq{\the\K@dr}}}\K@bc}\def\K@jg#1{\K@ol#1;@\K@pb\K@pc\K@pd}\def
~\K@ol#1;#2@#3#4#5{\def\K@bf{#2}\ifx\K@bf\K@ci\let\K@pe\K@pf\K@pg
~#1;@#3#4#5\else\let\K@ph\K@pi\let\K@pj\K@pk\K@pl#1;#2@#3#4#5\fi}\def
~\K@pg#1;#2@#3#4#5{\def\K@bf{#2}\ifx\K@bf\K@ci\def\K@bf{#1,;}\else\edef
~\K@bf{#1,#2}\fi\expandafter\K@pe\K@bf @#3#4#5}\def\K@pf
~#1,#2;@#3#4#5{\setbox\K@du=\hbox{\K@do=#1pt}\def\K@bf{#2} \ifdim\wd\K@du
~>\z@\ifx\K@bf\K@ci\K@pm#1@#5\else\setbox\K@du=\hbox{\K@do=#2pt}\ifdim\wd
~\K@du>\z@\K@pm#1@#4\K@pm\K@pn#2@#5\else\K@pm#1@#5\xdef#3{\K@pn#2}\fi\fi
~\else\gdef#3{#1}\ifx\K@bf\K@ci\else\K@pm\K@pn#2@#5\fi\fi}\def\K@pn
~#1,{#1}\def\K@po#1;{#1}\def\K@pl#1;#2@#3#4#5{\K@pp#1,@#3#4#5\def\K@bf
~{#2}\ifx\K@bf\K@ci\else\edef\K@bf{\K@po#2}\expandafter\K@pp\K@bf
~,@#3#4#5\fi}\def\K@pp#1,#2@#3#4#5{\def\K@bf{#2}\ifx\K@bf\K@ci\K@ph
~#1@#3#5\else\K@pj#1,#2@#4#5\fi}\def\K@pi#1@#2#3{\setbox\K@du=\hbox{\K@do
~=#1pt}\ifdim\wd\K@du>\z@\K@pm#1@#3\else\gdef#2{#1}\fi}\def\K@pk
~#1,#2,@#3#4{\K@pm#1@#3\K@pm#2@#4}\def\K@pm#1@#2{\K@do=#1 \K@di=\K@do\xdef
~#2{\the\K@di}}\let\K@hp\K@cm\def\K@pq#1{\bgroup\edef\endgr{\noexpand\K@pr
~{\K@hp}\egroup}\K@ps{#1}\K@hp\edef\K@bc{\noexpand\K@pr{\K@hp}}\K@bc}\def
~\K@ha{\relax\K@pq}\def\K@pt#1{\K@ps{#1}\K@pu\global\let\K@pu\K@pu}\let\gr
~\K@ha\def\K@ps#1#2{\K@do=1sp \K@do=#1\K@do\ifdim\K@do>1sp \else\ifdim
~\K@do<\z@\else\def#2{#1}\fi\fi}\def\gray{\gr\K@pv}\let\grey\gray\def
~\endgray{\endgr}\let\endgrey\endgray\def\white{\gr1}\let\endwhite\endgray
~\def\black{\gr0}\let\endblack\endgray\def\K@li#1{\let\K@ph\K@pw\let\K@pj
~\K@px\K@pl#1;@\K@py\K@pz\K@qa}\def\K@mf#1{\gdef\K@pz{#1}}\def\K@mg#1{\K@do
~=#1 \K@di=\K@do\xdef\K@qa{\the\K@di}}\def\K@lj#1{\let\K@ph\K@pw\let\K@pj
~\K@px\K@pl#1;@\K@qb\K@qc\K@qd}\def\K@mh#1{\gdef\K@qc{#1}}\def\K@mi#1{\K@do
~=#1 \K@di=\K@do\xdef\K@qd{\the\K@di}}\def\K@lt#1{\K@li{#1}\K@lj{#1}}\def
~\K@mj#1{\K@mh{#1}\K@mf{#1}}\def\K@mk#1{\K@mi{#1}\K@mg{#1}}\def\K@ml#1{\gdef
~\K@qe{#1}}\def\K@mm#1{\gdef\K@qf{#1}}\def\K@mn#1{\K@ml{#1}\K@mm{#1}}\def
~\K@mo#1{\K@do=#1 \K@di=\K@do\xdef\K@qg{\the\K@di}}\def\K@mp#1{\K@do=#1
~\K@di=\K@do\xdef\K@qh{\the\K@di}}\def\K@mq#1{\K@mo{#1}\K@mp{#1}}\def\K@px
~#1,#2@#3#4{\K@do=#2 \K@di=\K@do\xdef#4{\the\K@di}\gdef#3{#1}}\def\K@lk
~#1{\K@do=#1 \K@di=\K@do\xdef\K@qi{\the\K@di}}\def\K@ll#1{\K@do=#1 \K@di
~=\K@do\xdef\K@qj{\the\K@di}}\def\K@lm#1{\K@qk#1@}\def\K@qk#1,#2@{\K@ll
~{#1}\K@lk{#2}}\def\K@lo#1{\K@do=#1 \K@di=\K@do\xdef\K@ql{\the\K@di}}\def
~\K@lp#1{\K@do=#1 \K@di=\K@do\xdef\K@qm{\the\K@di}}\def\K@lq#1{\K@qn#1@}\def
~\K@qn#1,#2@{\K@lp{#1}\K@lo{#2}}\def\K@mv{\let\K@jp\K@qo\def\K@jq{\global
~\let\K@qp\K@ci}\futurelet\K@jr\K@qq}\let\K@qr\relax\K@bg\kuvioldlabels
~{\K@cz\let\K@qr\K@ci}\def\K@qo#1{\egroup\K@do=#1 \gdef\K@ow{#1}}\def\K@ln
~{\global\let\K@qs\K@ci}\def\K@lr{\global\let\K@qt\K@cl}\def\K@mr{\global
~\let\K@qu\K@qv}\def\K@ms{\gdef\K@qu{2}}\def\K@mt{\gdef\K@qu{3}}\let\K@qw
~\K@cm\let\K@qv\K@co\def\braced{\K@cz\let\K@qw\K@co\let\K@qv\K@cm}\def
~\loose{\K@cz\let\K@qw\K@cm\let\K@qv\K@co\columndist=0pt}\def\K@mu{\global
~\let\K@qx\K@ci}\def\K@ma#1{\K@do=#1 \K@di=\K@do\divide\K@di by 2 \xdef\K@qy
~{=\the\K@di}\def\K@qz{\egroup\K@cj}}\def\K@mc#1{\K@do=#1 \global\K@dr
~={{#1}}}\def\K@me#1{\K@do=#1 \gdef\K@ra{#1}}\def\K@qz#1{\egroup\K@do=#1
~\K@di=\K@do\xdef\K@qy{\the\K@di}}\def\K@lu{\global\let\K@rb\K@ci\global\let
~\K@rc\K@ci\let\K@jp\K@qz\let\K@jq\relax\futurelet\K@jr\K@qq}\def\K@lv
~{\global\let\K@rc\K@ci\let\K@jp\K@qz\let\K@jq\relax\futurelet\K@jr\K@qq
~}\def\K@lw{\global\let\K@rd\K@ci}\def\K@lx{\global\let\K@re\K@cl}\def\K@ly
~{\global\let\K@rf\K@cl}\def\K@lz{\K@lx\K@ly}\let\K@rg\K@cl\def\joined
~{\K@cz\let\K@rg\K@ci}\def\K@ls#1{\K@ca\K@rh#1,@}\def\K@ri#1{\K@ca\K@rj#1,@}
??O\begingroup\K@ce\def\K@rh#1,#2@{{\K@ji\K@ed\def\K@bf{#2}\ifx\K@bf\K@ci
??O\K@rk#1@,@\else\K@rk#1@#2@\fi }}\def\K@rk#1@#2,@{\xdef\K@in{{#1}\K@in
??O}\xdef\K@rl{{#1@#2}\K@rl}}\def\K@rj#1,#2@{{\K@ji\K@ed\def\K@bf{#2}\ifx
??O\K@bf\K@ci\ifx\K@in\K@ci\K@rk#1@,@\else\ifx\K@rm\K@ci\edef\K@gl
??O{#1}\K@dr={\K@rn {\csname D@pt@#1@x\endcsname}{\csname D@pt@#1@y\endcsname
??O}{\csname D@pt@#1@type\endcsname}}\expandafter\K@ro\K@in{}\ifx\K@gl\relax
??O\else\K@rk#1@,@\fi\else\K@rk#1@,@\fi\fi\else\K@rk#1@#2@\fi }}\def
??O\K@ro#1#2{\def\K@bf{#1}\ifx\K@bf\K@gl\the\K@dr\K@dr={}\let\K@gl\relax\fi
??O\def\K@bf{#2}\ifx\K@bf\K@ci\let\K@bc\relax\else\def\K@bc{\K@ro{#2}}\fi
??O\K@bc}\def\K@rn#1#2#3{\ifx\K@rp\K@ci\xdef\K@rp{#1,#2}\expandafter\ifx
??O#3\relax\else\xdef\K@rq{\K@rr{#3}{}}\fi\else\xdef\K@rm
??O{#1,#2}\expandafter\ifx#3\relax\else\xdef\K@rs{\K@rr{#3}{}}\fi\fi}%
~\def\K@pr#1{\K@cg{#1 setgray}}\def\K@pw#1@#2#3{\K@do=#1 \K@di=-\K@do\xdef
~#2{\the\K@di}}
??V\def\K@eg{\global\advance\K@de by 1\relax\global\let\K@ni\K@cm\let\K@rt
??V\K@ru}\def\K@eh#1{\K@dr={#1}\edef\K@bc{\gdef\expandafter\noexpand\csname
??VD@Entry@\the\K@dh @\endcsname{\noexpand\D@\the\K@df @\the\K@de @\the\K@dr
??V@}}\K@bc\global\advance\K@dh by 1\relax\setbox\K@du=\hbox{\K@hi\K@hf
??V\K@hc\K@hh\let\gr\K@cj\let\endgr\relax\global\setbox\K@dt=\hbox\bgroup
??V\K@rv$\vertexstyle\K@gx#1\K@rw}}\def\K@rw{\K@rt\K@di=\wd\K@dt\K@dj=\ht
??V\K@dt\K@dk=\dp\K@dt {\count8=\K@di\advance\count8 by \K@dj\advance\count8
??Vby \K@dk\relax\ifnum\count8>0 \K@nh\fi }\ifnum\K@ni=1\relax\expandafter
??V\xdef\csname D@whd@\the\K@df @\the\K@de @\endcsname{\the\K@di @\the\K@dj
??V@\the\K@dk @}\xdef\K@ik{\K@ik{\the\K@df}{\the\K@de}}\fi}\def\K@em{\advance
??V\K@df by -1 \xdef\K@ho{\the\K@df}\let\K@rx\K@cm\let\K@ry\K@ho\let\K@rz
??V\K@cm\let\K@sa\K@hx\K@sb\let\K@sc\K@sd\K@nm\let\K@nh\relax\K@se\K@sf
??V\ifx\K@sg\relax\else\xdef\K@sh{\K@hy\K@ic\K@ia\K@hz\K@ib\K@id\K@ie\K@if
??V\K@ig\K@ih\K@ii}\ifx\K@sh\K@ci {\K@dm=\K@hx\K@dm\K@di=\K@dm\xdef\K@en
??V{\the\K@di}\K@dn=\K@ho\K@dn\K@di=\K@dn\xdef\K@eo{\the\K@di}}\def\K@bs
??V\K@si{\K@sj}\fi\fi\K@bs\K@si\K@sk{.}\K@dx{}{{\K@en}{\K@eo}{\K@ho}{\K@hp
??V}{\K@hn}}\K@hf\let\st@p\relax\K@nm}%
~\let\K@sk\K@cj
??V\def\K@sb{\def\K@bc{\K@sl{0}{0}}\expandafter\K@bc\K@ik{}{}}\def\K@sl
??V#1#2#3#4{\def\K@bf{#3}\ifx\K@bf\K@ci\def\K@bc{\K@sm{#1}{#2}\K@sn\K@sl
??V{#1}{#2}{}{}}\else\def\K@bc{\K@so{#1}{#2}{#3}{#4}}\fi\ifnum#1>\K@ho
??V\relax\let\K@bc\relax\fi\K@bc}\def\K@so#1#2#3#4{\def\K@bc{\K@sm
??V{#1}{#2}\K@sn\K@sl{#1}{#2}{#3}{#4}}\ifnum#1=#3\relax\ifnum#2=#4\relax
??V\def\K@bc{\K@sn\K@sl{#1}{#2}}\fi\fi\K@bc}\def\K@sn#1#2#3{\ifnum#3<\K@hx
??V\relax\K@di=#3 \advance\K@di by 1 \edef\K@bc{\noexpand#1{#2}{\the\K@di
??V}}\else\K@di=#2 \advance\K@di by 1 \edef\K@bc{\noexpand#1{\the\K@di
??V}{0}}\fi\K@bc}\def\K@sm#1#2{\global\expandafter\let\csname
??VD@whd@#1@#2@\endcsname\relax}\def\K@se{\K@sp\K@sq0\K@sr\K@ja\K@lh\let
??V\gr\K@pt\let\endgr\relax\let\D@\K@ss\K@st0\K@dh\K@su}\def\K@sv{\global
??V\let\K@sw\K@co\global\expandafter\let\csname D@as@1@\endcsname\relax
??V\global\let\K@sx\K@co\global\expandafter\let\csname D@cs@1@\endcsname
??V\relax\global\let\K@sy\K@co\global\expandafter\let\csname
??VD@ws@1@\endcsname\relax\global\let\K@sz\relax}\def\K@ta#1{\global
??V\expandafter\let\csname D@Bindings@#1@\endcsname\K@ci\K@di=#1\relax\ifnum
??V#1<\K@hx\advance\K@di by 1 \edef\K@bc{\noexpand\K@ta{\the\K@di}}\else\let
??V\K@bc\relax\fi\K@bc}\def\K@tb#1{\K@di=#1\relax\ifnum#1<\K@hx\advance
??V\K@di by 1 \edef\K@bc{\noexpand\K@tc{#1}{\the\K@di}}\K@bc{\expandafter\K@td
??V\K@cs}\K@ck\K@td\edef\K@bc{\noexpand\K@tb{\the\K@di}}\else\let\K@bc\relax
??V\fi\K@bc}\def\K@sp{\ifx\K@ij\relax\ifx\K@te\relax\K@di=\K@hx\divide
??V\K@di by 2 \multiply\K@di by 2 \ifnum\K@di=\K@hx\multiply\K@di by 5 \else
??V\multiply\K@di by 5 \advance\K@di by 5 \fi\else\K@di=\K@te\multiply\K@di
??Vby 10 \fi\else\K@di=\K@ij\multiply\K@di by 10 \fi\xdef\K@ij{\the\K@di
??V}}\def\K@su#1{\edef\K@tf{\expandafter\noexpand\csname D@Entry@\the
??V#1@\endcsname}\csname D@Entry@\the#1@\endcsname}\def\K@ss#1@#2@#3@{\K@df
??V=#1\relax\K@de=#2\relax\K@tg#3\K@th}\def\K@eq{\K@gy\K@ec\K@gz\let\gr
??V\K@ha\K@st\K@im\K@dg\K@ti}\def\K@st#1#2#3{\edef\K@bf{#2{\the#2}}\global
??V#2=#1 \expandafter\K@tj\K@bf#3}\def\K@tj#1#2#3{\ifnum#1=#2 \let\K@bc\relax
??V\else\def\K@bc{#3#1\global\advance#1 by 1 \K@tj#1{#2}#3}\fi\K@bc}\def
??V\K@ti#1{\csname D@Cell@\the#1@\endcsname}\def\K@tk#1{\ifcase#1 \relax\or
??V\K@tl0{-1}\K@tm\K@tn{-1}0\K@tl01\K@to\K@tp{-1}\K@hx\or\K@tl{-1}{-1}\K@tm
??V\K@tn00\K@tl11\K@to\K@tp\K@ho\K@hx\or\K@tl{-1}0\K@tm\K@tn0{-1}\K@tl
??V10\K@to\K@tp\K@ho{-1}\or\K@tl{-1}1\K@tm\K@tn0\K@hx\K@tl1{-1}\K@to\K@tp
??V\K@ho0\or\K@tl01\K@tm\K@tn{-1}\K@hx\K@tl0{-1}\K@to\K@tp{-1}0\or\K@tl
??V11\K@tm\K@tn\K@ho\K@hx\K@tl{-1}{-1}\K@to\K@tp00\or\K@tl10\K@tm\K@tn\K@ho
??V{-1}\K@tl{-1}0\K@to\K@tp0{-1}\or\K@tl1{-1}\K@tm\K@tn\K@ho0\K@tl{-1}1\K@to
??V\K@tp0\K@hx\fi}\def\K@tl#1#2#3#4#5#6{\K@di=\K@df\K@dj=\K@de\let#3\relax
??V\K@cu\ifnum\K@di=#5\relax\let\K@bc\K@tq\else\ifnum\K@dj=#6\relax\let
??V\K@bc\K@tq\else\let\K@bc\K@tr\fi\fi\K@bc{#1}{#2}{#3}{#4}\ifx#3\relax
??V\K@cv}\def\K@tq#1#2#3#4{\xdef#3{\the\K@di}\xdef#4{\the\K@dj}}\def\K@tr
??V#1#2#3#4{\advance\K@di by #1\relax\advance\K@dj by #2\relax\K@ts{\the
??V\K@di}{\the\K@dj}\K@bf\ifx\K@bf\relax\else\xdef#3{\the\K@di}\xdef#4{\the
??V\K@dj}\fi}%
~\def\K@tt#1#2#3{\ifx\K@rq\relax\xdef\K@bc{\noexpand\K@sc @\K@tn,\noexpand
~\K@tu @\K@tm,\noexpand\K@tv @}\K@bc\else\let\K@tu\K@tn\let\K@tv\K@tm\fi
~\ifnum#1=9 \let\K@tw\K@tx\else\K@ty1\K@qc\K@tz\K@ty1\K@pz\K@ua\ifnum
~#1=0 \ifx\K@qe\relax\else\K@ub\K@tu by {-1}\K@qe\fi\ifx\K@qg\relax
~\else\K@ub\K@tv by 1\K@qg\fi\fi\K@di=\K@qc\advance\K@di by \K@tu\edef
~\K@tu{\the\K@di}\K@di=\K@qd\advance\K@di by \K@tv\edef\K@tv{\the\K@di}\ifx
~\K@rs\relax\edef\K@bc{\noexpand\K@sc @\K@tp,\noexpand\K@uc @\K@to
~,\noexpand\K@ud @}\K@bc\else\let\K@uc\K@tp\let\K@ud\K@to\fi\ifnum#1=0
~\ifx\K@qf\relax\else\K@ub\K@uc by {-1}\K@qf\fi\ifx\K@qh\relax\else
~\K@ub\K@ud by 1\K@qh\fi\fi\K@di=\K@pz\advance\K@di by \K@uc\edef\K@uc
~{\the\K@di}\K@di=\K@qa\advance\K@di by \K@ud\edef\K@ud{\the\K@di}\K@ue
~\ifnum\K@uf=0 \K@di=\K@ug\relax\ifnum\K@di<0 \multiply\K@di by -1 \fi\edef
~\K@tw{\the\K@di}\else\ifnum\K@ug=0 \K@di=\K@uf\relax\ifnum\K@di<0
~\multiply\K@di by -1 \fi\edef\K@tw{\the\K@di}\else\K@uh\fi\fi\fi
~\ifnum\K@tw>0 \K@ui{#1}{#2}{#3}\fi}\def\K@ue{\K@di=\K@uc\multiply\K@di by
~-1 \advance\K@di by \K@tu\multiply\K@di by -1 \edef\K@ug{\the\K@di}\K@di
~=\K@ud\multiply\K@di by -1 \advance\K@di by \K@tv\multiply\K@di by -1 \edef
~\K@uf{\the\K@di}}\def\K@ui#1#2#3{\ifnum#1=0 \K@uj{#1}\K@oq\else\def\K@oq
~{#1}\fi {\ifnum#1=0 \ifx\K@tz\K@ci\let\K@tz\K@cm\let\K@uk\K@cm\let\K@ul
~\K@cm\fi\K@um\K@tu\K@tv\K@tz\K@uk\K@ul\ifx\K@ua\K@ci\let\K@ua\K@cm\let
~\K@un\K@cm\let\K@uo\K@cm\fi\K@um\K@uc\K@ud\K@ua\K@un\K@uo\fi\K@up\K@oq
~}\K@uq#1{#2}\ifx\K@rl\K@ci\else\K@ur{#1}#2\fi\ifnum\K@us<\K@ut\relax
~\else\ifx\K@pu\K@ci\else\edef\K@pu{\noexpand\K@pr{\K@pu}}\fi\K@uu
~{#1}{#2}{#3}\fi}\def\K@uu#1#2#3{\ifnum#1=9 \K@uv{#1}{#2}{#3}\else\K@uw
~{#1}{#2}{#3}\fi\ifx\K@rb\relax\def\K@gl{#3}\ifx\K@gl\K@ci\else\ifx
~\K@qt\K@ux\def\K@uy{\K@bz\K@uz}\else\let\K@uy\K@va\fi\K@vb
~{#1}{#2}#3{}\fi\fi}
??S\begingroup\K@ce\def\K@uv#1#2#3{\K@di=\K@tu\advance\K@di by \K@qj\edef
??S\K@vc{\the\K@di}\K@di=\K@tv\advance\K@di by \K@qi\edef\K@vd{\the\K@di
??S}\K@um\K@vc\K@vd000\ifx\K@qs\relax {\dimen0=\K@tw sp \K@dx{}{{}{0}{\dimen
??S0=\K@tw sp}}\edef\K@bc##1{\noexpand\K@ve1@\K@vc sp,\K@vd sp@{\noexpand\K@hv
??S0{\noexpand\K@vf\noexpand\K@vg{\K@vh}\hskip\K@qm sp\raise\K@ql sp
??S\noexpand\K@hv2{##1}\noexpand\K@vi}}}\ifx\K@rc\K@ci\K@bc{\K@pr{1}\K@hv
??S0{\hskip\K@qb sp \lower\K@vj\hbox{$\vcenter{ \hbox{\vrule width \K@us sp
??Sheight \K@qy sp depth \K@qy sp}}$}\hskip\K@py sp}\hskip\K@vk\dimen0}\fi
??S\ifx\K@rb\relax\K@dr={\K@vl#2}\K@bc{\K@pu\K@hv0{\hskip\K@qb sp \the\K@dr
??S{\K@us sp}\hskip\K@py sp}\hskip\K@vk\dimen0}\fi }\fi}%
~\def\K@uw#1#2#3{\K@di=\K@tu\advance\K@di by \K@uc\divide\K@di by 2 \advance
~\K@di by \K@qj\edef\K@vc{\the\K@di}\K@di=\K@tv\advance\K@di by \K@ud
~\divide\K@di by 2 \advance\K@di by \K@qi\edef\K@vd{\the\K@di}\ifx\K@qs
~\relax\edef\K@bc##1{\noexpand\K@ve1@\K@vc sp,\K@vd sp@{\noexpand\K@hv
~0{\noexpand\K@vf\noexpand\K@vm{\K@uf}{\K@ug}\hskip\K@qm sp\raise\K@ql sp
~\noexpand\K@hv1{##1}\noexpand\K@vi}}}\ifx\K@rc\K@ci\K@bc{\K@pr{1}\hbox
~{\hskip\K@qb sp \lower\K@vj\hbox{$\vcenter{ \hbox{\vrule width \K@us sp
~height \K@qy sp depth \K@qy sp}}$}\hskip\K@py sp}}\fi\ifx\K@rb\relax\K@dr
~={\K@vl#2}\K@bc{\K@pu\hbox{\hskip\K@qb sp \the\K@dr{\K@us sp}\hskip\K@py
~sp}}\fi\fi}\def\K@vb#1#2#3{\def\K@bf{#3}\ifx\K@bf\K@ci\let\K@bc\relax
~\else\def\K@bc{\K@uy{#1}{#2}#3@\K@vb{#1}{#2}}\fi\K@bc}
??O\def\K@ur#1#2#3{\edef\K@gl{\K@vn{#2}}\def\K@bf{\K@vo{#1}{#2}}\expandafter
??O\K@bf\K@rl{}}\def\K@vo#1#2#3#4{\K@vp{#1}{#2}#3@\def\K@bf{#4}\ifx\K@bf\K@ci
??O\let\K@bc\relax\else\def\K@bc{\K@vo{#1}{#2}{#4}}\fi\K@bc}\def\K@vp
??O#1#2#3@#4@{{\K@ji\K@ed\ifnum#1=9 \global\expandafter\let\csname
??OD@pt@#3@x\endcsname\K@tn\global\expandafter\let\csname D@pt@#3@y\endcsname
??O\K@tm\global\expandafter\let\csname D@pt@#3@type\endcsname\relax\else
??O\def\K@bf{#4}\ifx\K@bf\K@ci\else\let\K@gl\K@bf\fi\K@di=\K@qb\advance\K@di
??Oby \K@qm\relax\K@vq\K@tu\K@ug\K@vq\K@tv\K@uf\K@di=\K@py\multiply\K@di
??Oby -1 \advance\K@di by \K@qm\relax\K@vq\K@uc\K@ug\K@vq\K@ud\K@uf\K@do
??O=\K@tu sp \multiply\K@do by -1 \advance\K@do by \K@uc sp \K@do=\K@gl\K@do
??O\K@di=\K@do\advance\K@di by \K@tu\advance\K@di by \K@qj\relax\K@vr\K@dj
??O=\K@ql\times\K@uf\over{-\K@tw}\advance\K@di by \K@dj\expandafter\xdef
??O\csname D@pt@#3@x\endcsname{\the\K@di}\K@do=\K@tv sp \multiply\K@do by -1
??O\advance\K@do by \K@ud sp \K@do=\K@gl\K@do\K@di=\K@do\advance\K@di by
??O\K@tv\advance\K@di by \K@qi\relax\K@vr\K@dj=\K@ql\times\K@ug\over\K@tw
??O\advance\K@di by \K@dj\expandafter\xdef\csname D@pt@#3@y\endcsname{\the
??O\K@di}\expandafter\gdef\csname D@pt@#3@type\endcsname{#2}\fi }}%
~\def\K@vq#1#2{\K@dk=\K@tw\relax\K@vs\K@dj=\K@di\times#2\over\K@dk\advance
~\K@dj by #1 \edef#1{\the\K@dj}}\def\K@vr#1=#2\times#3\over#4{\K@dk=#2 \K@dl
~=#4\relax\K@vs#1=\K@dk\times#3\over\K@dl}\let\K@ux\K@cl\def\rotatedlabels
~{\let\K@ux\K@ci}\def\K@va#1#2#3#4@#5@{{\def\K@bf{#4}\ifx\K@bf\K@ci\else
~\K@vt#4\fi\K@vu{#1}{#2}\let\K@vv\K@co\K@vw{#3}\multiply\K@dp by \K@vv
~\advance\K@dp by \K@ql sp \edef\K@bc##1{\noexpand\K@vx @\K@vc sp,\K@vd
~sp@{##1}{\the\K@do}{\the\K@dp}}\K@bc{\K@vy{$\labelstyle#5$}}}}\def\K@vt
~#1#2#3{\def\K@bf{#1}\ifx\K@bf\K@cl\else\def\K@pb{#1}\fi\def\K@bf{#2}\ifx
~\K@bf\K@cl\else\def\K@pc{#2}\fi\def\K@bf{#3}\ifx\K@bf\K@cl\else\def\K@pd
~{#3}\fi}
??P\begingroup\K@ce\def\K@uz#1#2#3#4@#5@{{\def\K@bf{#4}\ifx\K@bf\K@ci\else
??P\K@vt#4\fi\K@vu{#1}{#2}\let\K@vv\K@co\let\K@vz\K@wa\K@vw{#3}\multiply
??P\K@dp by \K@vv\advance\K@dp by \K@ql sp \edef\K@bc##1{\noexpand\K@vx
??P@\K@vc sp,\K@vd sp@{##1}{\the\K@do}{\the\K@dp}}\K@bc{\K@vy{$\labelstyle#5$}}}}%
~\def\K@vu#1#2{\def\K@wb{\K@wc}\edef\K@vx{\noexpand\K@wd{\K@uf}{\K@ug}}\edef
~\K@vw{\noexpand\K@vz{\K@oq}}\K@do=\K@us sp \K@do=\K@pb\K@do\advance\K@do
~by \K@pc sp \advance\K@do by \K@qb sp \advance\K@do by \K@qm sp \K@dp=\K@tw
~sp \advance\K@do by -.5\K@dp\K@dp=\K@or sp \advance\K@dp by \K@os#2sp
~\advance\K@dp by \K@pd sp}
??S\def\K@vu#1#2{\ifnum#1=9 \def\K@wb{\K@we}\edef\K@vx{\noexpand\K@wf\K@vh
??S}\edef\K@vw{\noexpand\K@wg{\K@vh}}\K@do=\K@us sp \K@do=\K@pb\K@do
??S\advance\K@do by \K@pc sp \advance\K@do by \K@qb sp \advance\K@do by \K@qm
??Ssp \K@dp=-\K@tw sp \advance\K@do by \K@vk\K@dp\K@dp=\K@or sp \advance\K@dp
??Sby \K@os#2sp \advance\K@dp by \K@pd sp \else\def\K@wb{\K@wc}\edef\K@vx
??S{\noexpand\K@wd{\K@uf}{\K@ug}}\edef\K@vw{\noexpand\K@vz{\K@oq}}\K@do=\K@us
??Ssp \K@do=\K@pb\K@do\advance\K@do by \K@pc sp \advance\K@do by \K@qb sp
??S\advance\K@do by \K@qm sp \K@dp=\K@tw sp \advance\K@do by -.5\K@dp\K@dp
??S=\K@or sp \advance\K@dp by \K@os#2sp \advance\K@dp by \K@pd sp \fi}\def
??S\K@wf#1@#2,#3@#4#5#6{\K@dr={#4}\K@dx{}{{}{0}{\let\noexpand\K@vy\expandafter
??S\noexpand\K@vy\noexpand\K@gx}}\K@ve0@#2,#3@{\K@vf\K@wh{#1}\hskip#5 \raise
??S#6 \hbox{\K@wb{#1}{}\the\K@dr}\K@vi}}%
~\def\K@gx{\K@gy\K@gz\K@ec\let\gr\K@ha}\def\K@wh#1{\edef\K@bc{\noexpand\K@vg
~{#1}}\K@bc}\def\K@we#1#2{\K@di=#1 \multiply\K@di by -1 \edef\K@bc
~{\noexpand\K@vg{\the\K@di}}\K@bc}\def\K@wd#1#2@#3,#4@#5#6#7{\K@dr={#5}\K@dx
~{}{{}{0}{\let\noexpand\K@vy\expandafter\noexpand\K@vy\noexpand\K@gx}}\K@ve
~0@#3,#4@{\K@vf\K@wi{#1}{#2}\hskip#6 \raise#7 \hbox{\K@wb{#1}{#2}\the\K@dr
~}\K@vi}}\def\K@wi#1#2{\edef\K@bc{\noexpand\K@vm{#1}{#2}}\K@bc}\def\K@wc
~#1#2{\K@di=#1 \multiply\K@di by -1 \edef\K@bc{\noexpand\K@vm{\the\K@di
~}{#2}}\K@bc}\def\K@uq#1#2{\ifnum#1=9 \relax\else\ifnum#1=0 \K@wj\K@qb
~\K@re\K@tz\K@rq\K@wk{#2}\K@wj\K@py\K@rf\K@ua\K@rs\K@wl{#2}\else\K@wm\K@qb
~\K@re\K@wk{#2}\K@wm\K@py\K@rf\K@wl{#2}\fi\fi\K@di=\K@qb\advance\K@di by
~\K@py\multiply\K@di by -1 \advance\K@di by \K@tw\edef\K@us{\the\K@di
~}}\def\K@wj#1#2#3#4#5#6{\K@di=#1\relax\ifx#2\K@rg\advance\K@di by \K@wn
~\advance\K@di by \K@wo#6\else\ifx#3\K@ci\else\advance\K@di by #5\relax
~\advance\K@di by \K@wp\advance\K@di by \K@wq#6\fi\fi\edef#1{\the\K@di}}
??O\def\K@wj#1#2#3#4#5#6{\K@di=#1\relax\ifx#2\K@rg\advance\K@di by \K@wn
??O\advance\K@di by \K@wo#6\else\ifx#3\K@ci\ifx#4\relax\else\advance\K@di
??Oby \K@wr\advance\K@di by \K@ws#6\advance\K@di by #4\relax\advance\K@di
??Oby \K@wt\fi\else\advance\K@di by #5\relax\advance\K@di by \K@wp
??O\advance\K@di by \K@wq#6\fi\fi\edef#1{\the\K@di}}%
~\def\K@wm#1#2#3#4{\K@di=#1\relax\ifx#2\K@rg\advance\K@di by \K@wn
~\advance\K@di by \K@wo#4\else\advance\K@di by #3\relax\advance\K@di by
~\K@wp\advance\K@di by \K@wq#4\fi\edef#1{\the\K@di}}
??S\def\K@wg#1#2{\K@wu\K@di=#1\mod{360}\edef\K@vh{\the\K@di}\ifnum\K@di=0 \def
??S\K@gl{{1}}\else\ifnum\K@di=90 \def\K@gl{{7}}\else\ifnum\K@di=180 \def
??S\K@gl{{5}}\else\ifnum\K@di=270 \def\K@gl{{3}}\else\divide\K@di by 90
??S\ifcase\K@di\def\K@gl{{8}}\or\def\K@gl{{6}}\or\def\K@gl{{4}}\or\def
??S\K@gl{{2}}\fi\fi\fi\fi\fi\expandafter\K@vz\K@gl{#2}}%
~\def\K@vz#1#2{\ifcase#1 \relax\or\let\K@bc\K@wv\or\let\K@bc\K@ww\or
~\let\K@bc\K@wx\or\let\K@bc\K@wy\or\let\K@bc\K@wz\or\let\K@bc\K@xa\or
~\let\K@bc\K@xb\or\let\K@bc\K@xc\fi\K@bc{#2}}\def\K@wv#1{\ifcase#1
~\K@cf\K@vy\K@xd\or\K@cf\K@vy\K@xe\let\K@vv\K@cp\or\K@cf\K@vy\K@xe\let
~\K@vv\K@cp\or\K@cf\K@vy\K@xd\fi}\def\K@ww#1{\ifcase#1 \K@cf\K@vy\K@xf
~\let\K@vv\K@cp\or\K@cf\K@vy\K@xg\or\K@cf\K@vy\K@xf\let\K@vv\K@cp\or
~\K@cf\K@vy\K@xg\fi}\def\K@wx#1{\ifcase#1 \K@cf\K@vy\K@xh\let\K@vv\K@cp
~\or\K@cf\K@vy\K@xi\or\K@cf\K@vy\K@xh\let\K@vv\K@cp\or\K@cf\K@vy\K@xi
~\fi}\def\K@wy#1{\ifcase#1 \K@cf\K@vy\K@xj\let\K@vv\K@cp\or\K@cf\K@vy
~\K@xk\or\K@cf\K@vy\K@xk\or\K@cf\K@vy\K@xj\let\K@vv\K@cp\fi}\def\K@wz
~#1{\ifcase#1 \K@cf\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\or\K@cf
~\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\fi}\def\K@xa#1{\ifcase#1
~\K@cf\K@vy\K@xf\or\K@cf\K@vy\K@xg\let\K@vv\K@cp\or\K@cf\K@vy\K@xf\or
~\K@cf\K@vy\K@xg\let\K@vv\K@cp\fi}\def\K@xb#1{\ifcase#1 \K@cf\K@vy\K@xh
~\or\K@cf\K@vy\K@xi\let\K@vv\K@cp\or\K@cf\K@vy\K@xi\let\K@vv\K@cp\or
~\K@cf\K@vy\K@xh\fi}\def\K@xc#1{\ifcase#1 \K@cf\K@vy\K@xj\or\K@cf\K@vy
~\K@xk\let\K@vv\K@cp\or\K@cf\K@vy\K@xk\let\K@vv\K@cp\or\K@cf\K@vy\K@xj
~\fi}\def\K@xh#1{\K@hv2{\lower\K@vj\hbox{#1}}}\def\K@xj#1{\K@hv2{\vbox
~{\offinterlineskip\hbox{#1}\null}}}\def\K@xd#1{\K@hv1{\vbox
~{\offinterlineskip\hbox{#1}\null}}}\def\K@xg#1{\K@hv0{\vbox
~{\offinterlineskip\hbox{#1}\null}}}\def\K@xi#1{\K@hv0{\lower\K@vj\hbox
~{#1}}}\def\K@xk#1{\K@hv0{\vtop{\offinterlineskip\null\hbox{#1}}}}\def\K@xe
~#1{\K@hv1{\vtop{\offinterlineskip\null\hbox{#1}}}}\def\K@xf#1{\K@hv2{\vtop
~{\offinterlineskip\null\hbox{#1}}}}\def\K@xl#1#2{\K@vg{180}}
??P\def\K@wa#1#2{\ifcase#1 \relax\or\let\K@bc\K@xm\or\let\K@bc\K@xn\or
??P\let\K@bc\K@xo\or\let\K@bc\K@xp\or\let\K@bc\K@xq\or\let\K@bc\K@xr\or
??P\let\K@bc\K@xs\or\let\K@bc\K@xt\fi\K@bc{#2}}\def\K@xm#1{\let\K@wb\K@ck
??P\ifcase#1 \K@cf\K@vy\K@xd\or\K@cf\K@vy\K@xe\let\K@vv\K@cp\or\K@cf
??P\K@vy\K@xe\let\K@vv\K@cp\or\K@cf\K@vy\K@xd\fi}\def\K@xn#1{\let\K@wb
??P\K@ck\ifcase#1 \K@cf\K@vy\K@xe\let\K@vv\K@cp\or\K@cf\K@vy\K@xd\or
??P\K@cf\K@vy\K@xe\let\K@vv\K@cp\or\K@cf\K@vy\K@xd\fi}\def\K@xo#1{\K@cf
??P\K@vy\K@xd\ifcase#1 \let\K@vv\K@cp\let\K@wb\K@xl\or\let\K@wb\K@ck\or
??P\let\K@vv\K@cp\let\K@wb\K@xl\or\let\K@wb\K@ck\fi}\def\K@xp#1{\let\K@wb
??P\K@xl\ifcase#1 \K@cf\K@vy\K@xd\let\K@vv\K@cp\or\K@cf\K@vy\K@xe\or
??P\K@cf\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\fi}\def\K@xq#1{\let
??P\K@wb\K@xl\ifcase#1 \K@cf\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\or
??P\K@cf\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\fi}\def\K@xr#1{\let
??P\K@wb\K@xl\ifcase#1 \K@cf\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\or
??P\K@cf\K@vy\K@xe\or\K@cf\K@vy\K@xd\let\K@vv\K@cp\fi}\def\K@xs#1{\K@cf
??P\K@vy\K@xd\ifcase#1 \let\K@wb\K@ck\or\let\K@vv\K@cp\let\K@wb\K@xl\or
??P\let\K@vv\K@cp\let\K@wb\K@xl\or\let\K@wb\K@ck\fi}\def\K@xt#1{\let\K@wb
??P\K@ck\ifcase#1 \K@cf\K@vy\K@xd\or\K@cf\K@vy\K@xe\let\K@vv\K@cp\or
??P\K@cf\K@vy\K@xe\let\K@vv\K@cp\or\K@cf\K@vy\K@xd\fi}\endgroup
~\def\K@cf#1#2{\def#1{#2}}\def\K@uj#1#2{\ifnum\K@uf>0 \ifnum\K@ug>0 \def
~#2{8}\else\ifnum\K@ug=0 \def#2{7}\else\def#2{6}\fi\fi\else\ifnum\K@uf
~=0 \ifnum\K@ug>0 \def#2{1}\else\ifnum\K@ug=0 \relax\else\def#2{5}\fi\fi
~\else\ifnum\K@ug>0 \def#2{2}\else\ifnum\K@ug=0 \def#2{3}\else\def
~#2{4}\fi\fi\fi\fi}\def\K@xu#1#2#3#4{\ifx#1\K@rg\let#2\K@ck\fi\ifx
~#3\K@rg\let#4\K@ck\fi}\def\K@up#1{\global\let\K@wk\K@cm\global\let\K@wl
~\K@cm\K@di=\K@uf\relax\ifnum\K@di<0 \multiply\K@di by -1 \fi\K@dj=\K@ug
~\relax\ifnum\K@dj<0 \multiply\K@dj by -1 \fi\ifcase#1 \let\K@bc\relax\or
~\K@xv\K@bc\or\K@xw\K@bc\or\K@xx\K@bc\or\K@xy\K@bc\or\K@xz\K@bc\or
~\K@ya\K@bc\or\K@yb\K@bc\or\K@yc\K@bc\fi\K@bc}\def\K@xv#1{\K@xu\K@re
~\K@yd\K@rf\K@ye\def#1{\K@yd1\K@wk\K@ye1\K@wl}}\def\K@xw#1{\K@xu\K@re\K@yd
~\K@rf\K@ye\def#1{\K@yd2\K@wk\K@ye2\K@wl}}\def\K@xx#1{\K@xu\K@re\K@yd\K@rf
~\K@ye\def#1{\K@yd3\K@wk\K@ye3\K@wl}}\def\K@xy#1{\K@xu\K@re\K@yd\K@rf\K@ye
~\def#1{\K@yd4\K@wk\K@ye4\K@wl}}\def\K@xz#1{\K@xu\K@re\K@ye\K@rf\K@yd
~\K@ct\K@pz\K@qc\K@ct\K@qa\K@qd\K@ct\K@tz\K@ua\K@ct\K@uk\K@un\K@ct\K@ul
~\K@uo\def#1{\K@yd1\K@wl\K@ye1\K@wk}}\def\K@ya#1{\K@xu\K@re\K@ye\K@rf\K@yd
~\K@ct\K@pz\K@qc\K@ct\K@qa\K@qd\K@ct\K@tz\K@ua\K@ct\K@uk\K@un\K@ct\K@ul
~\K@uo\def#1{\K@yd2\K@wl\K@ye2\K@wk}}\def\K@yb#1{\K@xu\K@re\K@ye\K@rf\K@yd
~\K@ct\K@pz\K@qc\K@ct\K@qa\K@qd\K@ct\K@tz\K@ua\K@ct\K@uk\K@un\K@ct\K@ul
~\K@uo\def#1{\K@yd3\K@wl\K@ye3\K@wk}}\def\K@yc#1{\K@xu\K@re\K@ye\K@rf\K@yd
~\K@ct\K@pz\K@qc\K@ct\K@qa\K@qd\K@ct\K@tz\K@ua\K@ct\K@uk\K@un\K@ct\K@ul
~\K@uo\def#1{\K@yd4\K@wl\K@ye4\K@wk}}\def\K@yd#1#2{\ifcase#1 \relax\or
~\K@yf{#2}\or\K@yg{#2}\or\K@yh{#2}\or\K@yi{#2}\fi}\def\K@yf#1{\K@dk=\K@tz
~\advance\K@dk by \K@uk\advance\K@dk by \K@ul\relax\ifnum\K@dk>0 \K@dk
~=\K@tz\divide\K@dk by -2 \advance\K@dk by \K@qc\multiply\K@dk by -1 \K@vs
~\K@dl=\K@dk\times\K@tw\over\K@dj\xdef#1{\the\K@dl}\fi}\def\K@yg#1{\K@dk
~=\K@tz\advance\K@dk by \K@uk\advance\K@dk by \K@ul\relax\ifnum\K@dk>0
~\K@dk=\K@ul\advance\K@dk by \K@vj\advance\K@dk by \K@qd\K@dl=\K@tz\divide
~\K@dl by -2 \advance\K@dl by \K@qc\multiply\K@dl by -1 \K@yj#1\fi}\def\K@yh
~#1{\K@dk=\K@tz\advance\K@dk by \K@uk\advance\K@dk by \K@ul\relax\ifnum
~\K@dk>0 \K@dk=\K@vj\advance\K@dk by \K@ul\relax\K@vs\K@dl=\K@dk\times\K@tw
~\over\K@di\xdef#1{\the\K@dl}\fi}\def\K@yi#1{\K@dk=\K@tz\advance\K@dk by
~\K@uk\advance\K@dk by \K@ul\relax\ifnum\K@dk>0 \K@dk=\K@ul\advance\K@dk
~by \K@vj\advance\K@dk by \K@qd\K@dl=\K@tz\divide\K@dl by 2 \advance\K@dl
~by \K@qc\relax\K@yj#1\fi}\def\K@ye#1#2{\ifcase#1 \relax\or\K@yk{#2}\or
~\K@yl{#2}\or\K@ym{#2}\or\K@yn{#2}\fi}\def\K@yk#1{\K@dk=\K@ua\advance
~\K@dk by \K@un\advance\K@dk by \K@uo\relax\ifnum\K@dk>0 \K@dk=\K@ua
~\divide\K@dk by 2 \advance\K@dk by \K@pz\relax\K@vs\K@dl=\K@dk\times\K@tw
~\over\K@dj\xdef#1{\the\K@dl}\fi}\def\K@yl#1{\K@dk=\K@ua\advance\K@dk by
~\K@un\advance\K@dk by \K@uo\relax\ifnum\K@dk>0 \K@dk=\K@vj\advance\K@dk
~by -\K@un\advance\K@dk by \K@qa\multiply\K@dk by -1 \K@dl=\K@ua\divide
~\K@dl by 2 \advance\K@dl by \K@pz\relax\K@yj#1\fi}\def\K@ym#1{\K@dk=\K@ua
~\advance\K@dk by \K@un\advance\K@dk by \K@uo\relax\ifnum\K@dk>0 \K@dk
~=-\K@vj\advance\K@dk by \K@un\relax\K@vs\K@dl=\K@dk\times\K@tw\over\K@di
~\xdef#1{\the\K@dl}\fi}\def\K@yn#1{\K@dk=\K@ua\advance\K@dk by \K@un
~\advance\K@dk by \K@uo\relax\ifnum\K@dk>0 \K@dk=\K@vj\advance\K@dk by
~-\K@un\advance\K@dk by \K@qa\multiply\K@dk by -1 \K@dl=\K@ua\divide\K@dl
~by -2 \advance\K@dl by \K@pz\multiply\K@dl by -1 \K@yj#1\fi}\def\K@yj
~#1{\ifnum\K@dk=0 \ifnum\K@dl<0 \K@vs\K@dk=\K@dl\times\K@tw\over\K@dj\xdef
~#1{\the\K@dk}\else\global\let#1\K@cm\fi\else\ifnum\K@dl=0 \ifnum\K@dk
~<0 \K@vs\K@dl=\K@dk\times\K@tw\over\K@di\xdef#1{\the\K@dl}\else\global
~\let#1\K@cm\fi\else\ifnum\K@dk<0 \ifnum\K@dl<0 \K@yo#1\else\K@vs\K@dl
~=\K@dk\times\K@tw\over\K@di\xdef#1{\the\K@dl}\fi\else\ifnum\K@dl<0 \K@vs
~\K@dk=\K@dl\times\K@tw\over\K@dj\xdef#1{\the\K@dk}\else\K@yo#1\fi\fi\fi
~\fi}\def\K@yo#1{\K@do=\K@di sp \divide\K@do by \K@dk\K@dp=\K@dj sp
~\divide\K@dp by \K@dl\ifdim\K@do=\K@dp\K@vs\K@dh=\K@dk\times\K@tw\over
~\K@di\K@vs\K@dg=\K@dl\times\K@tw\over\K@dj\ifnum\K@dh<\K@dg\xdef#1{\the
~\K@dh}\else\xdef#1{\the\K@dg}\fi\else\ifdim\K@dp<\K@do\K@vs\K@dl=\K@dk
~\times\K@tw\over\K@di\xdef#1{\the\K@dl}\else\K@vs\K@dk=\K@dl\times\K@tw
~\over\K@dj\xdef#1{\the\K@dk}\fi\fi}
??V\def\K@er{\K@hc\K@hh\K@ee\let\gr\K@cj\let\endgr\relax\K@hi\let\D@\K@yp
??V\K@st0\K@dh\K@yq\K@yr}%
~\def\K@hi{\def\K@ys##1##2{\K@rt\let\K@rt\relax}\def\K@yt##1##2{\K@rt\let
~\K@rt\relax}\def\K@yu##1##2{\K@rt\let\K@rt\relax}\def\K@yv##1{\K@rt\let
~\K@rt\relax}}
??V\def\K@yq#1{\csname D@Entry@\the#1@\endcsname}\def\K@eb{\K@em\let\K@ec
??V\K@yw\let\K@ed\K@yx\let\K@ee\K@yy\def\K@um{\K@yz}\let\K@dz\K@za\let
??V\K@rt\egroup\global\setbox\K@ds=\hbox\bgroup\hbox to \K@en sp{\hfil\vbox
??Vto \K@eo sp{\vfil}}\K@ep\K@eq\K@er\let\gr\K@pt\let\endgr\relax\K@lh
??V\K@ja\K@zb\K@zc\K@zd\let\\\relax\setbox\K@du=\hbox\bgroup}%
??Q\begingroup\K@ce\def\K@zd{\let\hd\K@ze\let\pd\K@zf\let\tl\K@zg\let\pl
??Q\K@zh\let\pt\K@ri\def\Text{\K@bx\K@zi}\def\Txt{\K@bx\K@zj}\def\Math{\K@bx
??Q\K@zk}\def\Label{\K@bx\K@zl}\def\Vertex{\K@bx\K@zm}\def\Pt{\K@ca\K@zn}\def
??Q\Dot{\K@bx\K@zo}\def\Box{\K@cb\K@zp}\def\Frame{\K@cb\K@zq}}%
~\def\K@ze#1{\gdef\K@zr{\K@dr={#1}}}\def\K@zg#1{\gdef\K@zs{\K@dr={#1}}}\def
~\K@zf#1{\hd{\phantom{#1}}}\def\K@zh#1{\tl{\phantom{#1}}}
??V\def\K@za{\K@rt\egroup\K@dx{}{{}{1}{\gdef\noexpand\K@es{\K@es}\gdef
??V\noexpand\K@et{\K@et}\gdef\noexpand\K@eu{\K@eu}\gdef\noexpand\K@ev{\K@ev
??V}}}\K@ew\K@ex\K@ey\egroup\Displaybox\K@ds}%
??X\begingroup\K@ce\def\K@zt{$\egroup\null\egroup\K@di=\wd\K@ds\xdef\K@en
??X{\the\K@di}\K@dj=\ht\K@ds\xdef\K@eo{\the\K@dj}\K@dx{}{{\K@en}{\K@eo
??X}{}{\K@hp}}\let\K@gi\K@zu\K@zv}\def\K@zw{\K@di=\K@en\relax\K@dj=\K@eo
??X\relax\K@zv}\def\K@zv{\ifx\K@zx\K@ci\K@dm=\K@di sp \divide\K@dm by \K@zy
??X\let\K@hx\K@zy\else\K@dm=\K@zx\divide\K@di by \K@dm\edef\K@hx{\the\K@di
??X}\fi\let\K@rz\K@cm\let\K@sa\K@hx\ifx\K@zz\K@ci\K@dn=\K@dj sp \divide
??X\K@dn by \K@Aa\let\K@ho\K@Aa\else\K@dn=\K@zz\divide\K@dj by \K@dm\edef
??X\K@ho{\the\K@dj}\fi\let\K@rx\K@cm\let\K@ry\K@ho\let\K@sc\K@Ab\let\K@in
??X\K@ci\let\K@ec\K@yw\let\K@ed\K@yx\let\K@ee\K@yy\let\K@rt\egroup\global
??X\setbox\K@ds=\hbox\bgroup\hbox to \K@en sp{\vbox to \K@eo sp{\vss}\hss
??X}\K@Ac\K@ep{\llap{\box\K@ds}\K@Ad{\K@gm\K@dr}{{0pt}{0pt}{0{\the\K@dr
??X}}}}\K@Ae\let\gr\K@pt\let\endgr\relax\K@hg\K@lh\K@hb\K@ja\K@zb\K@zc
??X\K@zd\K@Af\setbox\K@du=\hbox\bgroup}\def\K@zu{\K@rt\egroup\K@ew\K@ex
??X\K@hr\egroup\Displaybox\K@ds}%
??Q\def\K@zb{\let\K@Ag/\let\K@Ah\/\catcode`\/=\active\let\K@Ai|\let\K@Aj
??Q\|\catcode`\|=\active\let\K@Ak*\let\K@Al\*\catcode`\*=\active}{\catcode
??Q`\/=\active\catcode`\|=\active\catcode`\*=\active\catcode`\(=\active
??Q\gdef\K@zc{\let(\K@Am\let/\K@An\let|\K@Ao\let*\K@Ap\let\((\let\//\let
??Q\||\let\**}\gdef\K@yw{\let/\K@Ag\let\/\K@Ah\let|\K@Ai\let\|\K@Aj\let
??Q*\K@Ak\let\*\K@Al}\gdef\K@yy{\let/\K@cj\let|\K@cj\let*\K@cj\let\//\let
??Q\||\let\**}\gdef\K@yx{\let/\K@Aq\let|\K@Ar\let*\K@As}}\def\K@Aq{/}\def
??Q\K@Ar{|}\def\K@As{*}\def\K@Am#1,#2){\ifx\K@rp\K@ci\xdef\K@rp{#1,#2}\else
??Q\ifx\K@rm\K@ci\xdef\K@rm{#1,#2}\fi\fi}\def\K@An#1{\edef\K@bf{\K@At
??Q#1.@}\ifx\K@bf\K@ci\else\global\let\K@vh\K@bf\fi}\def\K@Ao#1{\K@do=#1
??Q\K@di=\K@do\xdef\K@tx{\the\K@di}}\def\K@Ap#1{\gdef\K@vk{#1}}%
~\def\K@At#1.#2@{#1}\def\K@ex#1{#1\K@ds\K@Au\K@ds\K@Av\K@ds\K@Aw\K@ds
~\K@Ax\K@ds}
??V\def\K@ey#1{\ifmmode\ifnum\K@ho=0 \let\K@Av\K@cj\fi\fi\K@do=\K@eu sp
??V\advance\K@do by \K@Ay\K@dp=\K@ev sp \advance\K@dp by \K@Ay\relax\ifx
??V\K@hn\K@cp\else\let\K@Az\K@Ba\let\K@Av\K@cj\fi\global\setbox#1=\hbox
??V{\hskip\K@do\vtop{\offinterlineskip\vbox\bgroup\vskip\K@Ay\K@Az
??V#1\vskip\K@Ay}\hskip\K@dp}}\def\K@Az#1{\ifx\K@Bb\relax\vskip-\K@vj\vskip
??V\ifnum\K@es=-1 \K@vj\else\K@es sp\fi\box#1\vskip\K@vj\egroup\else\vskip
??V\ifnum\K@es=-1 \K@vj\else\K@es sp\fi\egroup\vskip-\K@vj\box#1\vskip\K@vj
??V\fi\vskip\ifnum\K@et=-1 -\K@vj\else\K@et sp\fi}\def\K@Ba#1{\K@di=-\K@ho
??V\advance\K@di by \K@hn\relax\multiply\K@di by -1 \K@di=\csname D@Y\the
??V\K@di @\endcsname\relax\vskip-\K@vj\vskip\ifnum\K@es=-1 \K@vj\else\K@es
??Vsp\fi\hbox{\raise\K@vj\hbox{\lower\K@di sp\box#1}}\egroup\vskip\K@vj
??V\vskip\ifnum\K@et=-1 -\K@vj\else\K@et sp\fi}%
??X\def\K@hr#1{\global\setbox#1=\hbox{\hskip\K@hk\vtop{\offinterlineskip
??X\vbox\bgroup\vskip\K@hk\ifx\K@Bc\relax\box#1\egroup\else\egroup\box#1
??X\fi\vskip\K@hk}\hskip\K@hk}}%
~\def\K@Aw#1{\global\setbox#1=\hbox{\hskip\K@Bd\vtop{\vbox{\vskip\K@Be\box
~#1} \vskip\K@Bf}\hskip\K@Bg}}\def\K@Bh#1{\ifmmode\K@Bi#1\fi}\let\K@Av\K@Bh
~\def\K@Bi#1{\global\setbox#1=\hbox{$\vcenter{\box#1}$}}\K@bg\center{\K@cz
~\let\K@Av\K@Bi}\K@bm\centre\center\def\K@Bj{\K@cz\let\K@Av\K@Bh}\K@bh
~\uncenter\K@Bj\K@bh\uncentre\K@Bj\K@bh\centermath\K@Bj\K@bh\centremath
~\K@Bj\K@bg\deep{\K@cz\let\K@Av\K@cj\let\K@Bb\K@ci\let\K@Bc\K@ci}\K@bg
~\tall{\K@cz\let\K@Av\K@cj\let\K@Bb\relax\let\K@Bc\relax}\let\K@Bb\K@ci\let
~\K@Bc\relax\let\K@Au\K@cj\K@bg\landscape{\K@cz\def\K@Au{\K@bo\K@Bk
~}}\K@bg\oplandscape{\K@cz\def\K@Au{\K@bo\K@Bl}}
??Z\begingroup\K@ce\def\K@Bk#1{\global\setbox#1=\hbox{\K@Bm\box#1\K@Bn}\K@Bo
??Z\K@Bg\K@Bd}\def\K@Bl#1{\global\setbox#1=\hbox{\K@Bp\box#1\K@Bq}\K@Bo\K@Bd
??Z\K@Bg}\def\K@Bo#1#2{\let\K@bf\K@Be\let\K@Be#1\let#1\K@Bf\let\K@Bf#2\let
??Z#2\K@bf}\def\K@Bm{\K@Br\bgroup\setbox\K@du=\hbox\bgroup\K@Bs}\def\K@Bn
??Z{\K@Bt\egroup\K@do=\ht\K@du\advance\K@do by \dp\K@du\hbox to \K@do{\hfil
??Z\vbox to \wd\K@du{\vfill\K@vf\K@vg{90}\K@xg{\box\K@du}\K@vi }}\egroup
??Z}\K@bh\endland\K@Bn\def\K@Bp{\K@Br\bgroup\setbox\K@du=\hbox\bgroup\K@Bs
??Z}\def\K@Bq{\K@Bt\egroup\K@do=\ht\K@du\advance\K@do by \dp\K@du\hbox to
??Z\K@do{\hfil\vbox to \wd\K@du{\vfill\K@vf\K@vg{-90}\K@xf{\box\K@du}\K@vi
??Z}}\egroup}\K@bh\endopland\K@Bq\def\K@Bu{\K@Br\bgroup\setbox\K@du=\hbox
??Z\bgroup\K@Bs}\K@bg\endflip{\K@Bt\egroup\K@do=\ht\K@du\ht\K@du=\dp\K@du\dp
??Z\K@du=\K@do\hbox to \wd\K@du{\hfil\K@vf\K@vg{180}\hbox to \z@{\box\K@du
??Z\hss}\K@vi }\egroup}\def\K@Bv{\K@cg{currentpoint currentpoint translate 1
??Z-1 scale neg exch neg exch translate}}\def\K@Bw{\K@cg{currentpoint
??Zcurrentpoint translate -1 1 scale neg exch neg exch translate}}\def\K@Bx
??Z{\K@Br\bgroup\setbox\K@du=\hbox\bgroup\K@Bs}\K@bg\endhmir{\K@Bt\egroup
??Z\K@do=\ht\K@du\ht\K@du=\dp\K@du\dp\K@du=\K@do\hbox{\K@vf\K@Bv\box\K@du
??Z\K@vi}\egroup}\def\K@By{\K@Br\bgroup\setbox\K@du=\hbox\bgroup\K@Bs}\K@bg
??Z\endvmir{\K@Bt\egroup\hbox to \wd\K@du{\hfil\K@vf\K@Bw\hbox to \z@{\box
??Z\K@du\hss}\K@vi}\egroup}\def\K@Bz#1{\K@Br\bgroup\edef\K@bc{\noexpand\K@vg
??Z{\K@At#1.@}}\setbox\K@du=\hbox\bgroup\K@Bs}\K@bg\endrot{\K@Bt\egroup\K@do
??Z=\ht\K@du\advance\K@do by -\dp\K@du\hbox{\phantom{\copy\K@du}\hbox to \z@
??Z{\hskip-.5\wd\K@du\raise.5\K@do\hbox{\K@vf\K@bc\hbox to \z@{\hss\vbox to
??Z\z@{\vss\box\K@du\vss}\hss}\K@vi}\hss}}\egroup}\endgroup
~\K@bk\land{\relax\K@bo\K@Bm}\K@bg\opland{\relax\K@bo\K@Bp}\K@bg\flip{\relax
~\K@bo\K@Bu}\K@bg\hmir{\relax\K@bo\K@Bx}\K@bg\hmirror{\relax\K@bo\K@Bv}\K@bg
~\vmir{\relax\K@bo\K@By}\K@bg\rot{\relax\K@bo\K@Bz}\def\K@Br#1{\ifmmode
~\ifinner\def\K@Bs{$}\else\def\K@Bs{$\displaystyle}\fi\def\K@Bt{$}\else
~\let\K@Bs\bgroup\let\K@Bt\egroup\fi #1\let\K@Br\relax}\K@bg\squish{\relax
~\ifmmode\def\next{\mathpalette\K@Ca}\else\let\next\K@Cb\fi\next}\def
~\K@Cb#1{\hbox to \z@{\hss#1\hss}}\def\K@Ca#1#2{\hbox to \z@{\hss$\m@th
~#1{#2}$\hss}}\K@bg\squash{\relax\ifmmode\def\next{\mathpalette\K@Cc}\else
~\let\next\K@Cd\fi\next}\def\K@Cd#1{\setbox\z@\hbox to \z@{\hss#1\hss
~}\K@Ce}\def\K@Cc#1#2{\setbox\z@\hbox to \z@{\hss$\m@th#1{#2}$\hss}\K@Ce
~}\def\K@Ce{\ht\z@\z@\dp\z@\z@\box\z@}
??Y\begingroup\K@ce\def\K@Cf{\K@Br\bgroup\hbox\bgroup\K@Cg\vtop\bgroup
??Y\vbox\bgroup\K@Ch\vskip\K@Be\vskip\K@Ci\hbox\bgroup\hskip\K@Bd\hskip
??Y\K@Ci\K@Bs}\K@bg\endframe{\K@Bt\hskip\K@Bg\hskip\K@Ci\egroup\egroup
??Y\vskip\K@Bf\vskip\K@Ci\K@Ch\egroup\K@Cg\egroup\egroup}%
~\K@bg\frame{\relax\K@bq\K@Cf}\K@bg\framed{\let\K@Ax\K@Cj}\let\K@Ax\K@cj
~\def\K@Cj#1{\global\setbox#1=\hbox{\K@Cg\vtop{\vbox{\K@Ch\box#1}\K@Ch
~}\K@Cg}}\def\K@Cg{\K@Ck\vrule width \K@Cl\K@Cm}\def\K@Ch{\K@Ck\hrule
~height \K@Cl\K@Cm}
??Y\def\K@Cn#1#2{\K@Br\bgroup\K@Co#1@\K@qc\K@qd\K@Co#2@\K@pz\K@qa\setbox
??Y8=\hbox\bgroup\K@Cg\vtop\bgroup\vbox\bgroup\K@Ch\vskip\K@Be\vskip\K@Ci
??Y\hbox\bgroup\hskip\K@Bd\hskip\K@Ci\K@Bs}\def\K@Cp{\K@Bt\hskip\K@Bg\hskip
??Y\K@Ci\egroup\egroup\vskip\K@Bf\vskip\K@Ci\K@Ch\egroup\K@Cg\egroup
??Y\dimen4=-\wd8 \advance\dimen4 by \K@qc\relax\multiply\dimen4 by -1
??Y\advance\dimen4 by \K@pz\relax\ifdim\dimen4>\z@\dimen8=\ht8 \dimen6=-\dp
??Y8 \advance\dimen8 by \K@qa\advance\dimen6 by \K@qd\multiply\dimen6 by -1
??Y\K@do=\K@qc\K@dp=\K@pz\multiply\K@dp by -1 \setbox\K@du=\hbox{\ifdim\K@do
??Y>\z@\hskip\K@do\fi\vrule width\dimen4 height \dimen8 depth \dimen6 \ifdim
??Y\K@dp>\z@\hskip\K@dp\fi}\multiply\K@dp by -1 \hbox{\K@Cq\box\K@du\K@Cr
??Y\llap{\K@ha1\vrule width\wd8 height \ht8 depth \dp8 \endgr\ifdim\K@dp>\z@
??Y\hskip\K@dp\fi}\llap{\box8 \ifdim\K@dp>\z@\hskip\K@dp\fi}}\else\box8 \fi
??Y\egroup}\def\K@Cs{\K@Bt\hskip\K@Bg\hskip\K@Ci\egroup\egroup\vskip\K@Bf
??Y\vskip\K@Ci\K@Ch\egroup\K@Cg\egroup\K@do=-\wd8 \advance\K@do by \K@qc
??Y\multiply\K@do by -1 \advance\K@do by \K@pz\relax\ifdim\K@do>\z@\dimen
??Y8=\ht8 \dimen6=-\dp8 \setbox\K@du=\hbox{\phantom{\copy8}}\ifdim\K@qa>\z@
??Y\setbox\K@du=\vbox{\offinterlineskip\hbox to \wd8{\hskip\K@qc\vrule
??Ywidth \K@do height \K@qa\hss} \box\K@du}\setbox8=\vbox{\vskip\K@qa\box8}\fi
??Y\ifdim\K@qd<\z@\K@dp=\K@qd\multiply\K@dp by -1 \setbox\K@du=\vtop
??Y{\offinterlineskip\box\K@du\hbox to \wd8{\hskip\K@qc\vrule width \K@do
??Yheight \K@dp\hss}}\setbox8=\vtop{\box8\vskip\K@dp}\fi\ifdim\K@qa<\z@
??Y\advance\dimen8 by \K@qa\fi\ifdim\K@qd>\z@\advance\dimen6 by \K@qd\fi
??Y\multiply\dimen6 by -1 \K@do=\K@qc\multiply\K@do by -1 \K@dp=\K@pz\setbox
??Y\K@du=\hbox{\ifdim\K@do>\z@\vrule width \K@do height \dimen8 depth \dimen
??Y6 \fi\box\K@du\ifdim\K@dp>\z@\vrule width \K@dp height \dimen8 depth
??Y\dimen6 \fi}\hbox{\K@Cq\box\K@du\K@Cr\llap{\hbox{\ifdim\K@do>\z@\hskip
??Y\K@do\fi\box8 \ifdim\K@dp>\z@\hskip\K@dp\fi}}}\else\box8 \fi\egroup
??Y}\K@bg\endshade{\K@Bt\hskip\K@Bg\hskip\K@Ci\egroup\egroup\vskip\K@Bf
??Y\vskip\K@Ci\K@Ch\egroup\K@Cg\egroup\dimen4=-\wd8 \advance\dimen4 by
??Y\K@qc\relax\multiply\dimen4 by -1 \advance\dimen4 by \K@pz\relax\ifdim
??Y\dimen4>\z@\dimen8=\ht8 \dimen6=-\dp8 \advance\dimen8 by \K@qa\advance
??Y\dimen6 by \K@qd\multiply\dimen6 by -1 \K@do=\K@qc\K@dp=\K@pz\multiply
??Y\K@dp by -1 \setbox\K@du=\hbox{\ifdim\K@do>\z@\hskip\K@do\fi\vrule
??Ywidth\dimen4 height \dimen8 depth \dimen6 \ifdim\K@dp>\z@\hskip\K@dp\fi
??Y}\multiply\K@dp by -1 \hbox{\K@Cq\box\K@du\K@Cr\llap{\K@ha1\dimen6=\K@Cl
??Y\dimen2=\wd8 \K@do=\ht8 \K@dp=\dp8 \ifdim\K@qd<\z@\advance\K@dp by -\dimen
??Y6 \fi\ifdim\K@qa>\z@\advance\K@do by -\dimen6 \fi\ifdim\K@qc<\z@
??Y\advance\dimen2 by -\dimen6 \fi\ifdim\K@pz>\z@\advance\dimen2 by -\dimen
??Y6 \else\dimen6=\z@\fi\vrule width\dimen2 height \K@do depth \K@dp\hskip
??Y\dimen6 \endgr\ifdim\K@dp>\z@\hskip\K@dp\fi}\llap{\box8 \ifdim\K@dp>\z@
??Y\hskip\K@dp\fi}}\else\box8 \fi\egroup}\def\K@Co#1,#2@#3#4{\edef
??Y#3{#1}\edef#4{#2}}\endgroup
~\K@bg\shade{\relax\K@bq\K@Cn}\K@bg\NoTeXviewHack{\def\endshade{\K@Cp}}\K@bg
~\TeXshades{\def\endshade{\K@Cs}}
??N\begingroup\K@ce\def\K@zp{\K@rt\let\K@pu\K@ci\let\K@rp\K@ci\let\K@rm
??N\K@ci\let\K@qj\K@cm\let\K@qi\K@cm\let\K@qm\K@cm\let\K@ql\K@cm\def\K@rt
??N{\egroup\K@Ct}\setbox\K@du=\hbox\bgroup}\def\K@Ct{\ifx\K@rm\K@ci\else
??N\K@Cu\expandafter\K@Cv\K@rp @\K@tn\K@tm\edef\K@bc{\noexpand\K@sc @\K@tn
??N,\noexpand\K@tu @\K@tm,\noexpand\K@tv @}\K@bc\expandafter\K@Cv\K@rm @\K@tp
??N\K@to\edef\K@bc{\noexpand\K@sc @\K@tp,\noexpand\K@uc @\K@to,\noexpand\K@ud
??N@}\K@bc\ifnum\K@tu>\K@uc\relax\K@ct\K@tu\K@uc\fi\ifnum\K@tv>\K@ud\relax
??N\K@ct\K@tv\K@ud\fi\K@di=\K@tu\multiply\K@di by -1 \advance\K@di by \K@uc
??N\relax\K@dj=\K@tv\multiply\K@dj by -1 \advance\K@dj by \K@ud\relax\K@do
??N=\K@tu sp \advance\K@do by \K@qj sp \advance\K@do by \K@qm sp \K@dp=\K@tv
??Nsp \advance\K@dp by \K@qi sp \advance\K@do by \K@ql sp \edef\K@bc{\noexpand
??N\K@ve0@\the\K@do,\the\K@dp @{\noexpand\K@Bs\vrule width \the\K@di sp
??Nheight \the\K@dj sp \noexpand\K@Bt}}\K@bc\fi}%
??Q\def\K@Cu{\ifx\K@pu\K@ci\def\K@Bs{\relax}\def\K@Bt{\relax}\else\edef\K@Bs
??Q{\noexpand\K@ha{\K@pu}}\def\K@Bt{\endgr}\fi}\endgroup
??N\def\K@zq{\K@rt\let\K@pu\K@ci\let\K@rp\K@ci\let\K@rm\K@ci\let\K@qj\K@cm
??N\let\K@qi\K@cm\let\K@qm\K@cm\let\K@ql\K@cm\let\K@ra\K@Cw\def\K@rt
??N{\egroup\K@Cx}\setbox\K@du=\hbox\bgroup\def\rw{\K@md}}\def\K@Cx{\ifx\K@rm
??N\K@ci\else\bgroup\K@Cu\expandafter\K@Cv\K@rp @\K@tn\K@tm\edef\K@bc
??N{\noexpand\K@sc @\K@tn,\noexpand\K@tu @\K@tm,\noexpand\K@tv @}\K@bc
??N\expandafter\K@Cv\K@rm @\K@tp\K@to\edef\K@bc{\noexpand\K@sc @\K@tp
??N,\noexpand\K@uc @\K@to,\noexpand\K@ud @}\K@bc\ifnum\K@tu>\K@uc\relax\K@ct
??N\K@tu\K@uc\fi\ifnum\K@tv>\K@ud\relax\K@ct\K@tv\K@ud\fi\K@di=\K@tu
??N\multiply\K@di by -1 \advance\K@di by \K@uc\relax\K@dj=\K@tv\multiply\K@dj
??Nby -1 \advance\K@dj by \K@ud\relax\K@do=\K@tu sp \advance\K@do by \K@qj
??Nsp \advance\K@do by \K@qm sp \K@dp=\K@tv sp \advance\K@dp by \K@qi sp
??N\advance\K@do by \K@ql sp \edef\K@bc{\noexpand\K@ve0@\the\K@do,\the\K@dp
??N@{\noexpand\K@Bs\noexpand\K@Cy{\the\K@di sp}{\the\K@dj sp}\noexpand\K@Bt
??N}}\K@bc\egroup\fi}\def\K@Cy#1#2{\hbox to #1{\vbox to #2{\vfil}\hfil}\llap
??N{\vbox to #2{ \vfil\hbox to #1{\vrule width \K@ra height #2 \hss\vrule
??Nwidth \K@ra height #2} \vfil}}\llap{\hbox to #1{\hfil\vbox to #2{ \hrule
??Nheight \K@ra width #1 \vss\hrule height \K@ra width #1}\hfil}}}\endgroup
??X\def\K@gj#1{\bgroup\K@dw\K@dx{\K@dy\K@dr}{\the\K@dr}\def\K@gi{\K@Cz}\def
??X\Modify{\K@by\K@Af\K@zt}\global\setbox\K@ds=\vbox\bgroup\offinterlineskip
??X\hbox\bgroup$}\K@bk\endFigure{\K@gi\egroup}%
~\def\K@fi{\K@gj}\K@bk\Figure{\bgroup\K@br\K@ej\K@ek\K@el\everyFigure\K@fi
~{Figure}}\K@bl\everyFigure\relax
??X\def\K@Cz{$\egroup\null\egroup\K@dx{\K@di=\wd\K@ds\K@dj=\ht\K@ds}{{\the
??X\K@di}{\the\K@dj}{}{\K@hp}}\K@ew\K@ex\K@hr\egroup\Displaybox\K@ds}%
~\K@bk\newFigure{\bgroup\K@ez\K@Da}\def\K@Da#1{\egroup\expandafter\ifx
~\csname D@every#1@\endcsname\relax\expandafter\expandafter\expandafter\let
~\expandafter\expandafter\csname D@@#1@@\endcsname\csname#1\endcsname
~\expandafter\def\csname D@every#1@\endcsname{\expandafter\expandafter
~\expandafter\let\expandafter\expandafter\csname#1\endcsname\csname
~D@@#1@@\endcsname}\fi\expandafter\K@bk\csname#1\endcsname{\bgroup\K@br
~\csname D@every#1@\endcsname\K@ej\K@ek\K@el\everyFigure\csname
~every#1\endcsname\K@fi{#1}}\expandafter\K@bk\csname end#1\endcsname{\K@gi
~\egroup}\expandafter\let\csname every#1\endcsname\relax}
??X\def\K@fw#1#2#3{\bgroup\K@dw\K@dx{\K@dy\K@dr}{\the\K@dr}\let\K@pe\K@Db
??X\K@pg#2;@\K@en\K@zx\K@zy\K@pg#3;@\K@eo\K@zz\K@Aa\K@dx{}{{\K@en}{\K@eo
??X}{}{\K@hp}}\let\K@Dc\K@zu\let\K@hk\K@hl\let\K@Ad\K@ck\global\setbox\K@ds
??X=\hbox to \K@en sp {\vbox to \K@eo sp{\vss}\hss}\K@by\K@Af\K@zw}\K@bk
??X\endGraph{\K@Dc\egroup}%
~\def\K@fg{\K@fw}\K@bk\Graph{\bgroup\K@br\K@ej\K@ek\K@el\everyGraph\K@fg
~{Graph}}\K@bl\everyGraph\relax
??X\def\K@Ad{\K@dx}%
~\def\K@Af{\def\K@um##1##2##3##4##5{}}\K@bk\newGraph{\bgroup\K@ez\K@Dd}\def
~\K@Dd#1{\egroup\K@br\expandafter\ifx\csname D@every#1@\endcsname\relax
~\expandafter\expandafter\expandafter\let\expandafter\expandafter\csname
~D@@#1@@\endcsname\csname#1\endcsname\expandafter\def\csname
~D@every#1@\endcsname{\expandafter\expandafter\expandafter\let\expandafter
~\expandafter\csname#1\endcsname\csname D@@#1@@\endcsname}\fi\expandafter
~\K@bk\csname#1\endcsname{\bgroup\K@br\csname D@every#1@\endcsname\K@ej
~\K@ek\K@el\everyGraph\csname every#1\endcsname\K@fg{#1}}\expandafter
~\K@bk\csname end#1\endcsname{\K@Dc\egroup}\expandafter\let\csname
~every#1\endcsname\relax}
??X\def\K@Db#1,#2;@#3#4#5{\K@do=#1\relax\ifdim\K@do<\z@\multiply\K@do by -1
??X\fi\K@di=\K@do\edef#3{\the\K@di}\def\K@bf{#2}\ifx\K@bf\K@ci\else\setbox
??X\K@du=\hbox{\K@do=\K@pn#2pt}\ifdim\wd\K@du>\z@\K@do=\K@pn#2\relax\ifdim
??X\K@do=\z@\else\edef#4{\the\K@do}\fi\else\K@di=\K@pn#2\relax\ifnum\K@di
??X>\z@\edef#5{\the\K@di}\fi\fi\fi}\endgroup
~\K@bg\gridlines{\K@cz\K@De\let\K@gf\K@gd\let\K@gh\K@go}\K@bg\overgrid
~{\K@cz\K@De\let\K@gf\K@ge\let\K@gh\K@gn\let\K@Ac\K@cr}\let\K@Ac\K@cq\def
~\K@De{\let\K@fz\K@gd\let\K@ep\K@Df\let\K@ep\K@Df\def\K@Cz{\K@zt\K@zu
~}}\let\K@ep\relax\def\K@Dg#1#2{\K@do=1sp \K@do=#1\K@do\ifdim\K@do>1sp
~\else\ifdim\K@do<\z@\else\K@do=1000sp \K@do=#1\K@do\ifdim\K@do=\z@\let
~#2\K@ci\else\def#2{#1}\fi\fi\fi}\def\K@Df{\let\K@tz\K@ci\let\K@ua\K@ci
~\let\K@rp\K@ci\let\K@rm\K@ci\let\K@zr\K@ci\let\K@zs\K@ci\let\K@qd\K@cm
~\let\K@qc\K@ci\let\K@qa\K@cm\let\K@pz\K@ci\let\K@qj\K@cm\let\K@qi\K@cm
~\let\K@qm\K@cm\let\K@ql\K@cm\def\K@qb{-65536}\let\K@py\K@qb\let\K@pu\K@Dh
~\let\K@qs\relax\let\K@rb\relax\let\K@rc\relax\let\K@rl\K@ci\let\K@qe
~\relax\let\K@qf\relax\let\K@qg\relax\let\K@qh\relax\let\K@rq\relax\let
~\K@rs\relax\ifnum\K@ho>0 \K@di=0 \K@cu\let\K@tm\K@rx\edef\K@tn{\the\K@di
~}\let\K@to\K@ry\let\K@tp\K@tn {\K@Af\K@tt0{{Line}{}}{}}\ifnum\K@di<\K@hx
~\advance\K@di by 1 \K@cv\fi\ifnum\K@hx>0 \K@di=0 \K@cu\edef\K@tm{\the
~\K@di}\let\K@tn\K@rz\let\K@to\K@tm\let\K@tp\K@sa {\K@Af\K@tt
~0{{Line}{}}{}}\ifnum\K@di<\K@ho\advance\K@di by 1 \K@cv\fi}\K@bk\newcell
~{\bgroup\K@ez\K@Di}\def\K@Di#1{\egroup\expandafter\K@bk\csname#1\endcsname
~{\K@Dj{#1}} \expandafter\K@bk\csname a#1\endcsname{\null\K@yu0{#1}}
~\expandafter\K@bk\csname r#1\endcsname{\null\K@yu1{#1}} \expandafter\K@bk
~\csname rd#1\endcsname{\null\K@yu2{#1}} \expandafter\K@bk\csname
~d#1\endcsname{\null\K@yu3{#1}} \expandafter\K@bk\csname ld#1\endcsname
~{\null\K@yu4{#1}} \expandafter\K@bk\csname l#1\endcsname{\null\K@yu5{#1}}
~\expandafter\K@bk\csname lu#1\endcsname{\null\K@yu6{#1}} \expandafter\K@bk
~\csname u#1\endcsname{\null\K@yu7{#1}} \expandafter\K@bk\csname
~ru#1\endcsname{\null\K@yu8{#1}} \expandafter\K@bk\csname b#1\endcsname
~{\null\K@yu{10}{#1}} \expandafter\edef\csname D@#1b@x\endcsname
~##1##2{\lower\K@vj\hbox{$\expandafter\noexpand\csname#1box\endcsname
~{##2}$}} \expandafter\ifx\csname#1box\endcsname\relax\expandafter\K@bi
~\expandafter\edef\csname#1box\endcsname##1{\hbox to ##1{$\expandafter
~\noexpand\csname#1fill\endcsname$}} \fi\expandafter\let\csname
~D@#1@lwp@\endcsname\K@cm\expandafter\let\csname D@#1@lp@\endcsname\K@cm
~\expandafter\let\csname D@#1@cp@\endcsname\K@cm\expandafter\let\csname
~D@#1@jp@\endcsname\K@cm\expandafter\let\csname D@#1@bp@\endcsname\K@cm
~\expandafter\let\csname D@#1@lpt@\endcsname\K@ci\expandafter\let\csname
~D@#1@ppt@\endcsname\K@ci\expandafter\let\csname D@#1@pp@\endcsname\K@cm
~\expandafter\let\csname D@#1@ap@\endcsname\K@cm}\def\K@Dj#1{\K@rt\K@bw
~\K@Dk\edef\K@pb{\K@Dl{#1}{}}\let\K@oi\K@pb\global\K@dr={{#1}{}}\def\K@rt
~{\egroup\K@Dm}\setbox\K@du=\hbox\bgroup}
??S\def\K@Dn#1{\K@rt\K@Dk\edef\K@pb{\K@Dl{Fillcell}{}}\let\K@oi\K@pb\global
??S\K@dr={{Fillcell}{#1}}\def\K@rt{\egroup\K@Dm}\setbox\K@du=\hbox\bgroup}\def
??S\K@Do#1{\K@rt\K@Dk\edef\K@pb{\K@Dl{Boxcell}{}}\let\K@oi\K@pb\global\K@dr
??S={{Boxcell}{#1}}\def\K@rt{\egroup\K@Dm}\setbox\K@du=\hbox\bgroup}\def\K@Dp
??S{\K@rt\K@Dk\edef\K@pb{\K@Dl{Rule}{}}\let\K@oi\K@pb\edef\K@bc{\global
??S\K@dr={{\K@Dq}}}\K@bc\def\K@rt{\egroup\expandafter\K@Dr\the\K@dr\K@Dm
??S}\setbox\K@du=\hbox\bgroup\def\rw{\K@mb}}\def\K@Dr#1{\K@do=#1 \divide
??S\K@do by 2 \K@di=\K@pd\advance\K@di by \K@do\xdef\K@pd{\the\K@di}\K@di
??S=\K@qy\advance\K@di by \K@do\xdef\K@qy{\the\K@di}\global\K@dr
??S={{Rule}{#1}}}\def\K@Dk{\let\K@rp\K@ci\let\K@rm\K@ci\let\K@vh\K@cm\let
??S\K@vk\K@cn\let\K@tx\K@Ds\let\K@zr\K@ci\let\K@zs\K@ci\let\K@pu\K@ci\let
??S\K@qs\relax\let\K@rc\relax\let\K@rb\relax\let\K@qy\K@cm\let\K@rl\K@ci
??S\let\K@pc\K@cm\let\K@oj\K@pc\let\K@pd\K@cm\let\K@ok\K@pd\let\K@qt\K@ci
??S\let\K@re\K@ci\let\K@rf\K@ci\let\K@rq\relax\let\K@rs\relax\let\K@qe\relax
??S\let\K@qf\relax\let\K@qg\relax\let\K@qh\relax\let\K@qj\K@cm\let\K@qi\K@cm
??S\let\K@qm\K@cm\let\K@ql\K@cm\let\K@qb\K@cm\let\K@qd\K@cm\let\K@qc\K@ci
??S\let\K@py\K@cm\let\K@qa\K@cm\let\K@pz\K@ci\K@dq={}}\def\K@Dm{\ifx\K@rc
??S\K@ci\expandafter\K@Dt\K@qy @\K@di\K@Du {\expandafter\K@Dv\the\K@dr}\edef
??S\K@qy{\the\K@di}\fi\ifx\K@rp\K@ci\else\expandafter\K@Dw\fi}\def\K@Dw{\ifx
??S\K@rm\K@ci\ifnum\K@tx>0 \expandafter\K@Cv\K@rp @\K@tn\K@tm\edef\K@bc
??S{\noexpand\K@tt9{\the\K@dr}{\the\K@dq}}{\K@gx\let\K@up\K@cj\K@bc }\fi
??S\else\let\K@Dx\relax\let\K@Dy\relax\def\K@Dz{\let\K@up\K@cj\K@bc
??S}\expandafter\K@Cv\K@rp @\K@tn\K@tm\expandafter\K@Cv\K@rm @\K@tp\K@to
??S\let\K@tz\K@ci\let\K@ua\K@ci\K@Ea\K@zs\K@qe\K@qg\K@rq\K@re\K@rp\K@tz
??S\K@uk\K@ul\K@Eb\K@Ec\K@tn\K@tm\K@Dy\K@Ea\K@zr\K@qf\K@qh\K@rs\K@rf\K@rm
??S\K@ua\K@un\K@uo\K@Ed\K@Ee\K@tp\K@to\K@Dx\edef\K@bc{\noexpand\K@tt0{\the
??S\K@dr}{\the\K@dq}}{\K@gx\K@Dz\K@Dy\K@Dx }\fi}\def\K@Ea
??S#1#2#3#4#5#6#7#8#9{\ifx#1\K@ci\def\K@fx{\K@Ef#2#3#4#5#6#7#8#9}\else\def
??S\K@fx{\K@Eg#1#7#8#9#2#3#4}\fi\K@fx}\def\K@Ef#1#2#3#4#5#6#7#8{\let#1\relax
??S\let#2\relax\ifx\K@sc\K@Ab\else\ifx#3\relax\ifx#4\K@ci\expandafter
??S\K@Eh#5@#6#7#8\fi\fi\fi\def\K@fx##1##2##3##4##5{}\K@fx}\def\K@Eg
??S#1#2#3#4#5#6#7#8#9{\def\K@Dz{\K@bc}\setbox\K@dt=\hbox{$\vertexstyle\K@gx
??S#1\the\K@dr$}\K@do=\wd\K@dt\K@di=\K@do\edef#2{\the\K@di}\K@do=\ht\K@dt\K@di
??S=\K@do\edef#3{\the\K@di}\K@do=\dp\K@dt\K@di=\K@do\edef#4{\the\K@di}\ifx
??S#5\relax\def#8{\relax}\else\K@ty{-1}#5#2\K@di=#5\relax\multiply\K@di by
??S-2 \edef#8{\hskip\the\K@di sp}\fi\ifx#6\relax\def#9{\lower\noexpand\K@vj
??S}\else\K@di=-\K@vj\advance\K@di by #6\relax\edef#9{\raise\the\K@di
??Ssp}\fi\def\K@fx{\K@Ei#1#7#8#9}\K@fx}\def\K@Ei#1#2#3#4#5#6#7{\edef
??S#7{\noexpand#1\ifx#2\relax\noexpand\K@Ej1@#5,#6@\else\noexpand\K@ve
??S1@#5sp,#6sp@\fi {#4\hbox{#3\noexpand\noexpand\noexpand\K@gx $\noexpand
??S\noexpand\noexpand\vertexstyle\noexpand\the\noexpand\K@dr$}}}}\def\K@Eh
??S#1,#2@#3#4#5{\K@Ek#1.,#2.@#3#4#5}\def\K@Ek#1.#2,#3.#4@#5#6#7{\def\K@bf
??S{#2#4}\ifx\K@bf\K@ci\ifnum#1>-1 \ifnum#1>\K@hx\relax\else\ifnum#3>-1
??S\ifnum#3>\K@ho\relax\else\K@di=-\K@ho\advance\K@di by #3 \multiply\K@di
??Sby -1 \K@ts{\the\K@di}{#1}\K@bf\ifx\K@bf\relax\else\expandafter\K@El
??S\K@bf#5#6#7\def\K@Dz{\K@bc}\fi\fi\fi\fi\fi\fi}%
~\def\K@Cv#1,#2@#3#4{\gdef#3{#1}\gdef#4{#2}}
??V\def\K@yu#1#2{\K@rt\K@Em\def\K@oq{#1}\def\K@ot{#2}\global\K@dr
??V={{#2}{}}\def\K@rt{\egroup\K@En{#1}}\setbox\K@du=\hbox\bgroup}\def\K@ys
??V#1#2{\K@rt\K@Em\def\K@oq{#1}\def\CellName{Fillcell}\global\K@dr
??V={{Fillcell}{#2}}\def\K@rt{\egroup\K@En{#1}}\setbox\K@du=\hbox\bgroup}\def
??V\K@yt#1#2{\K@rt\K@Em\def\K@oq{#1}\def\CellName{Boxcell}\global\K@dr
??V={{Boxcell}{#2}}\def\K@rt{\egroup\K@En{#1}}\setbox\K@du=\hbox\bgroup}\def
??V\K@yv#1{\K@rt\K@Em\def\K@oq{#1}\def\CellName{Rule}\edef\K@bc{\global\K@dr
??V={{\K@Dq}}}\K@bc\def\K@rt{\egroup\expandafter\K@Eo\the\K@dr\K@En
??V{#1}}\setbox\K@du=\hbox\bgroup\def\rw{\K@mb}}\def\K@Eo#1{\K@do=#1 \divide
??V\K@do by 2 \K@di=\K@pd\advance\K@di by \K@do\xdef\K@pd{\the\K@di}\K@di
??V=\K@qy\advance\K@di by \K@do\xdef\K@qy{\the\K@di}\global\K@dr
??V={{Rule}{#1}}}\def\K@Em{\let\K@qu\K@qw\let\K@qx\relax\let\K@pu\K@ci\let
??V\K@qs\relax\let\K@qp\K@qr\def\K@ow{0pt}\let\K@rc\relax\let\K@rb\relax
??V\let\K@qy\K@cm\let\K@rd\relax\let\K@py\K@cm\let\K@qb\K@cm\let\K@pb\K@ci
??V\let\K@rl\K@ci\let\K@pc\K@cm\let\K@pd\K@cm\let\K@qt\K@ci\let\K@re\K@ci
??V\let\K@rf\K@ci\let\K@qj\K@cm\let\K@qi\K@cm\let\K@qm\K@cm\let\K@ql\K@cm
??V\let\K@qd\K@cm\let\K@qc\K@ci\let\K@qa\K@cm\let\K@pz\K@ci\let\K@og\K@ci
??V\let\K@ox\K@ci\K@dq={}}\def\K@Ep#1#2#3#4#5#6#7#8#9{\ifcase#1 #2\or#3\or
??V#4\or#5\or#6\or #7\or#8\or#9\fi}\def\K@En#1{\def\K@oq{#1}\let\K@fx\K@ci
??V\ifx\K@og\K@ci\ifnum#1=0 \let\K@fx\relax\else {\K@tk{#1}}\fi\else\ifnum
??V#1=10 \edef\K@to{\the\K@df}\edef\K@tp{\the\K@de}\expandafter\K@Eq\K@og
??V@\K@tm\K@tn\K@Er{\let\K@fx\relax}\K@Es\K@oq\else\ifnum#1=0 \edef\K@tm
??V{\the\K@df}\edef\K@tn{\the\K@de}\expandafter\K@Eq\K@og @\K@to\K@tp\K@Er
??V{\let\K@fx\relax}\K@Es\K@oq\else {\K@tk{#1}}\fi\fi\fi\let\K@Et\K@cm
??V\ifx\K@qp\relax\expandafter\K@Eu\K@ox{}{}\fi\K@Ev\K@oq\ifx\K@fx\K@ci\ifx
??V\K@qs\K@ci\let\K@pu\K@cl\fi\ifx\K@rc\K@ci\expandafter\K@Dt\K@qy @\K@dk
??V\K@Du {\expandafter\K@Dv\the\K@dr}\edef\K@qy{\ifx\K@rb\relax1\else2\fi\the
??V\K@dk}\fi\ifx\K@rd\relax\K@Ew\K@oq{\the\K@dg}\K@fx\global\advance\K@dg
??Vby 1 \else\K@dk=\K@im\advance\K@dk by -1 \xdef\K@im{\the\K@dk}\K@Ew\K@oq
??V\K@im\K@fx\fi\fi\K@fx}\def\K@Eu#1#2{\def\K@bf{#1}\ifx\K@bf\K@ci\let
??V\K@bc\relax\else\ifx\K@bf\K@cl\ifx\K@pb\K@ci\def\K@bf{\K@Dl{\K@ot
??V}{}}\else\let\K@bf\K@pb\fi\fi\ifdim\K@bf pt=.5pt \ifnum#2>\K@Et\relax
??V\def\K@Et{#2}\fi\fi\let\K@bc\K@Eu\fi\K@bc}\def\K@Es#1{\ifnum\K@to>\K@tm
??V\ifnum\K@tp>\K@tn\def#1{2}\else\ifnum\K@tp=\K@tn\def#1{3}\else\def
??V#1{4}\fi\fi\else\ifnum\K@to=\K@tm\ifnum\K@tp>\K@tn\def#1{1}\else
??V\ifnum\K@tp=\K@tn\relax\else\def#1{5}\fi\fi\else\ifnum\K@tp>\K@tn\def
??V#1{8}\else\ifnum\K@tp=\K@tn\def#1{7}\else\def#1{6}\fi\fi\fi\fi}\def
??V\K@Er#1{\ifnum\K@to<0\relax #1\else\ifnum\K@to>\K@ho\relax #1\else\ifnum
??V\K@tp<0\relax #1\else\ifnum\K@tp>\K@hx\relax #1\fi\fi\fi\fi}\def\K@Dt
??V#1#2@#3#4#5{\if#1=#3=#2 \else #3=#1#2 \advance#3 by #4 \advance#3 by #5
??V\fi}\def\K@Ew#1#2#3{\edef#3{\gdef\expandafter\noexpand\csname
??VD@Cell@#2@\endcsname{\noexpand\K@Ex#1@\the\K@dr @\K@tm @\K@tn @\K@to @\K@tp
??V@{\the\K@dq}@{{\K@pb}{\K@rl}}{{\K@pc}{\K@pd}}{{\K@qb}{\K@py}}{{\K@qc
??V}{\K@qd}}{{\K@pz}{\K@qa}}{{\K@pu}{\K@qt}}{{\K@qj}{\K@qm}}{{\K@qi}{\K@ql
??V}}@{\K@qy}{\K@re}{\K@rf}@}}}\def\K@Eq#1@#2@#3#4{\K@di=\K@At#2.@\relax
??V\multiply\K@di by -1 \advance\K@di by \K@df\edef#3{\the\K@di}\K@di=\K@At
??V#1.@\relax\advance\K@di by \K@de\edef#4{\the\K@di}}\def\K@Ey#1{\ifnum
??V#1=1\relax\ifx\K@qx\relax\K@Ez\K@tm\K@tn\K@tp\K@Et\fi\else\ifnum
??V#1=5\relax\ifx\K@qx\relax\K@Ez\K@tm\K@tp\K@tn\K@Et\fi\else\ifnum\K@tn
??V=\K@tp\else\K@Fa\fi\fi\fi}\def\K@Ez#1#2#3#4{{\K@di=\K@sw\relax\advance
??V\K@di by 1 \K@Fb{A:r#1,c#2-#3}\expandafter\xdef\csname D@as@\K@sw
??V@\endcsname{\noexpand\K@Fc{#1}{#2}{#3}{#4}\expandafter\noexpand\csname
??VD@as@\the\K@di @\endcsname}\xdef\K@sw{\the\K@di}}\global\expandafter\let
??V\csname D@as@\K@sw @\endcsname\relax}\def\K@Fa{{\ifnum\K@tn>\K@tp\relax
??V\K@ct\K@tn\K@tp\K@ct\K@tm\K@to\fi\K@Fb{W:r\K@tm-\K@to,c\K@tn-\K@tp}\K@di
??V=\K@sy\relax\advance\K@di by 1 \expandafter\xdef\csname D@ws@\K@sy
??V@\endcsname{\noexpand\K@Fd {\K@tm}{\K@tn}{\K@to}{\K@tp}{\K@qu}\expandafter
??V\noexpand\csname D@ws@\the\K@di @\endcsname}\xdef\K@sy{\the\K@di}}\global
??V\expandafter\let\csname D@ws@\K@sy @\endcsname\relax}%
~\K@bk\displaystretches{\K@cz\let\K@Fb\K@Fe\let\K@sk\K@Fe}\let\K@Fb\K@cj
~\def\K@vl#1#2{\csname D@#1b@x\endcsname{#2}}\def\K@ov#1#2{\csname
~D@#1@lwp@\endcsname}\def\K@os#1#2{\csname D@#1@lp@\endcsname}\def\K@Dv
~#1#2{\csname D@#1@bp@\endcsname}\def\K@wq#1#2{\csname D@#1@cp@\endcsname
~}\def\K@wo#1#2{\csname D@#1@jp@\endcsname}
??O\def\K@ws#1#2{\csname D@#1@pp@\endcsname}\def\K@rr#1#2{\csname
??OD@#1@ap@\endcsname}%
~\def\K@Dl#1#2{\expandafter\ifx\csname D@#1@lpt@\endcsname\K@ci\K@Ff\else
~\csname D@#1@lpt@\endcsname\fi}
??O\def\K@vn#1{\expandafter\ifx\csname D@#1@ppt@\endcsname\K@ci\K@Fg\else
??O\csname D@#1@ppt@\endcsname\fi}%
~\def\D@Fillcellb@x#1#2{\lower\K@vj\hbox to #2{$#1$}}\K@bk\aFillcell#1{\null
~\K@ys0{#1}}\K@bk\rFillcell#1{\null\K@ys1{#1}}\K@bk\rdFillcell#1{\null\K@ys
~2{#1}}\K@bk\dFillcell#1{\null\K@ys3{#1}}\K@bk\ldFillcell#1{\null\K@ys
~4{#1}}\K@bk\lFillcell#1{\null\K@ys5{#1}}\K@bk\luFillcell#1{\null\K@ys
~6{#1}}\K@bk\uFillcell#1{\null\K@ys7{#1}}\K@bk\ruFillcell#1{\null\K@ys
~8{#1}}\K@bk\bFillcell#1{\null\K@ys{10}{#1}}\K@bk\Fillcell#1{\K@bw\K@Dn
~{#1}}\def\D@Boxcellb@x#1#2{\lower\K@vj\hbox{$#1{#2}$}}\K@bk\aBoxcell
~#1{\null\K@yt0{#1}}\K@bk\rBoxcell#1{\null\K@yt1{#1}}\K@bk\rdBoxcell#1{\null
~\K@yt2{#1}}\K@bk\dBoxcell#1{\null\K@yt3{#1}}\K@bk\ldBoxcell#1{\null\K@yt
~4{#1}}\K@bk\lBoxcell#1{\null\K@yt5{#1}}\K@bk\luBoxcell#1{\null\K@yt
~6{#1}}\K@bk\uBoxcell#1{\null\K@yt7{#1}}\K@bk\ruBoxcell#1{\null\K@yt
~8{#1}}\K@bk\bBoxcell#1{\null\K@yt{10}{#1}}\K@bk\Boxcell#1{\K@bw\K@Do
~{#1}}\def\D@Ruleb@x#1#2{\lower\K@vj\hbox{$\vcenter{ \hbox{\vrule width#2
~height #1}}$}}\K@bk\aRule{\null\K@yv0}\K@bk\rRule{\null\K@yv1}\K@bk\rdRule
~{\null\K@yv2}\K@bk\dRule{\null\K@yv3}\K@bk\ldRule{\null\K@yv4}\K@bk\lRule
~{\null\K@yv5}\K@bk\luRule{\null\K@yv6}\K@bk\uRule{\null\K@yv7}\K@bk\ruRule
~{\null\K@yv8}\K@bk\bRule{\null\K@yv{10}}\K@bk\Rule{\K@bw\K@Dp}\def\K@hv
~#1#2{\hbox to \z@{\ifnum#1=0 \else\hss\fi\smash{#2}\ifnum#1=2 \else\hss\fi
~}}\def\K@ve#1@#2,#3@#4{\llap{\hbox to \K@en sp{\hskip#2 \smash{\hbox{\raise
~#3\hbox{\K@hv#1{#4}}}}\hss}}\K@dx{\K@Fh\K@hv\K@Fh\K@wi\K@Fh\K@wh\K@Fh
~\K@vm\K@Fh\K@vg\K@Fh\K@wc\K@Fh\K@we\K@Fh\K@ha\K@Fh\K@pt\K@Fh\endgr\K@Fh
~\K@vj\K@Fh\K@cg}{{#2}{#3}{#1{#4}}}}\def\K@Fh#1{\def#1{\noexpand#1}}\def
~\K@Ej#1@#2,#3@#4{\K@sc @#2,\K@Fi @#3,\K@Fj @\K@ve#1@\K@Fi sp,\K@Fj
~sp@{#4}}\def\K@Fk @#1,#2@#3,#4@{\K@do=#1\K@dm\ifdim\K@do<\z@\K@di=\K@do
~\edef#2{\the\K@di}\else\K@Fl#1.@\K@Fm\K@Fn\ifnum\K@Fm<\K@hx\K@di=\csname
~D@X\K@Fm @\endcsname\ifnum\K@Fn>0 \K@do=\csname D@dx\K@Fm @\endcsname sp
~\K@do=.\K@Fn\K@do\advance\K@di by \K@do\fi\edef#2{\the\K@di}\else\K@di
~=\K@Fm\advance\K@di by -\K@hx\K@do=\csname D@X\K@hx @\endcsname sp
~\advance\K@do by \the\K@di\K@dm\advance\K@do by .\K@Fn\K@dm\K@di=\K@do
~\edef#2{\the\K@di}\fi\fi\K@do=#3\K@dn\ifdim\K@do<\z@\K@di=\K@do\edef
~#4{\the\K@di}\else\K@Fl#3.@\K@Fo\K@Fp\ifnum\K@Fo<\K@ho\K@di=\csname
~D@Y\K@Fo @\endcsname\ifnum\K@Fp>0 \K@do=\csname D@dy\K@Fo @\endcsname sp
~\K@do=.\K@Fp\K@do\advance\K@di by \K@do\fi\edef#4{\the\K@di}\else\K@di
~=\K@Fo\advance\K@di by -\K@ho\K@do=\K@eo sp \advance\K@do by \the\K@di
~\K@dn\advance\K@do by .\K@Fp\K@dn\K@di=\K@do\edef#4{\the\K@di}\fi\fi
~}\def\K@sd @#1,#2@#3,#4@{\K@do=#1\K@dm\K@di=\K@do\edef#2{\the\K@di}\K@do
~=#3\K@dn\K@di=\K@do\edef#4{\the\K@di}}\def\K@Ab @#1,#2@#3,#4@{\setbox
~\K@du=\hbox{\global\K@do=#1\K@dm=0pt}\K@di=\K@do\edef#2{\the\K@di}\setbox
~\K@du=\hbox{\global\K@do=#3\K@dn=0pt}\K@di=\K@do\edef#4{\the\K@di}}\def
~\K@Fl#1.#2@#3#4{\def\K@gl{#1}\ifx\K@gl\K@ci\let#3\K@cm\else\def#3{#1}\fi
~\def\K@gl{#2}\ifx\K@gl\K@ci\let#4\K@cm\else\edef#4{\K@At#2@}\fi}\def
~\K@vm#1#2{\K@cg{currentpoint currentpoint translate #1 neg #2 atan rotate
~neg exch neg exch translate}}\def\K@vg#1{\K@cg{currentpoint currentpoint
~translate #1 neg rotate neg exch neg exch translate}}\def\K@vf{\K@cg
~{gsave}}\def\K@vi{\K@cg{grestore}}\def\K@Fq#1,#2@#3,#4@#5{\K@Ej
~#2@#3,#4@{\hbox{\K@vf\K@vg{#1}\K@hv{#2}{#5}\K@vi}}}
??R\begingroup\K@ce\def\K@zl#1{\K@Fr{\lower\K@vj\hbox{$\labelstyle#1$}}}\def
??R\K@zm#1{\K@Fr{\lower\K@vj\hbox{$\vertexstyle#1$}}}\def\K@zi#1{\K@Fr
??R{#1}}\def\K@zj#1{\K@Fr{\lower\K@vj\hbox{$\vcenter{\hbox{#1}}$}}}\def\K@zk
??R#1{\K@Fr{\lower\K@vj\hbox{$#1$}}}\def\K@zo{\K@zm{\diagramdot}}%
??O\def\K@zn#1{\K@rt\let\K@rp\K@ci\def\K@rt{\egroup\K@Fs{#1}}\setbox\K@du
??O=\hbox\bgroup}\def\K@Fs#1{\ifx\K@rp\K@ci\else\def\K@bf{\K@Ft
??O{#1}}\expandafter\K@bf\K@rp @\fi}\def\K@Ft#1#2,#3@{{\K@ji\K@ed
??O\expandafter\xdef\csname D@pt@#1@x\endcsname{#2}\expandafter\xdef\csname
??OD@pt@#1@y\endcsname{#3}\global\expandafter\let\csname
??OD@pt@#1@type\endcsname\relax\xdef\K@in{{#1}\K@in}}}\endgroup
??R\def\K@Fr#1{\K@rt\def\K@rt{\egroup\K@Fu}\let\K@pu\K@ci\let\K@rp\K@ci\let
??R\K@rm\K@ci\let\K@rq\relax\let\K@rs\relax\let\K@vh\K@cm\let\K@vk\K@cn\let
??R\K@pb\K@cn\let\K@qj\K@cm\let\K@qi\K@cm\let\K@qm\K@cm\let\K@ql\K@cm
??R\setbox\K@dt=\hbox{\K@gx#1}\K@dx{\K@dr={\K@gx#1}\edef\K@bf{\the\wd\K@dt
??R}}{{}{0}{\K@do=\K@bf\setbox\K@dt=\hbox{\the\K@dr}}}\setbox\K@du=\hbox
??R\bgroup}\def\K@Fu{\ifx\K@rp\K@ci\else\K@Cu\relax\ifx\K@rm\K@ci\K@Fv
??R\else\K@Fw\fi\K@bc{\hskip\K@qm sp\raise\K@ql sp \K@hv2{\K@hv0{\K@Bs\box
??R\K@dt\K@Bt}\hskip\K@vk\K@do}}\fi}\def\K@Fv{\expandafter\K@Cv\K@rp @\K@tn
??R\K@tm\ifx\K@rq\relax\edef\K@bc{\noexpand\K@sc @\K@tn,\noexpand\K@tu
??R@\K@tm,\noexpand\K@tv @}\else\def\K@bc{\let\K@tu\K@tn\let\K@tv\K@tm}\fi
??R\K@bc\K@di=\K@tu\advance\K@di by \K@qj\relax\K@dj=\K@tv\advance\K@dj by
??R\K@qi\relax\K@do=\wd\K@dt\edef\K@bc##1{\noexpand\K@ve0@\the\K@di sp,\the
??R\K@dj sp@{\noexpand\K@vf\noexpand\K@vg{\K@vh}##1\noexpand\K@vi}}}\def\K@Fw
??R{\expandafter\K@Cv\K@rp @\K@tn\K@tm\ifx\K@rq\relax\edef\K@bc{\noexpand
??R\K@sc @\K@tn,\noexpand\K@tu @\K@tm,\noexpand\K@tv @}\else\def\K@bc{\let
??R\K@tu\K@tn\let\K@tv\K@tm}\fi\K@bc\expandafter\K@Cv\K@rm @\K@tp\K@to\ifx
??R\K@rs\relax\edef\K@bc{\noexpand\K@sc @\K@tp,\noexpand\K@uc @\K@to
??R,\noexpand\K@ud @}\else\def\K@bc{\let\K@uc\K@tp\let\K@ud\K@to}\fi\K@bc
??R\K@ue\K@uh\K@di=\K@tu\advance\K@di by \K@qj\relax\K@dj=\K@tv\advance\K@dj
??Rby \K@qi\relax\K@do=\wd\K@dt\K@dp=\K@tw sp \edef\K@bc##1{\noexpand\K@ve
??R0@\the\K@di sp,\the\K@dj sp@{\noexpand\K@vf\noexpand\K@vm{\K@uf}{\K@ug
??R}\K@dp=\the\K@dp\hskip\K@pb\K@dp\noexpand\K@wc{\K@uf}{\K@ug}\noexpand
??R\K@vg{\K@vh}##1\noexpand\K@vi}}}\endgroup
??W\begingroup\K@ce\def\K@si{\K@sg\expandafter\K@Fx\expandafter\K@Fy\K@hy
??W{}{}\expandafter\K@Fx\expandafter\K@Fz\K@ic{}{}\expandafter\K@Fx
??W\expandafter\K@Ga\K@ia{}{}\expandafter\K@Fx\expandafter\K@Gb\K@id
??W{}{}\expandafter\K@Gc\expandafter\K@ie\K@ie{}{}\expandafter\K@Fx
??W\expandafter\K@Gd\K@ie{}{}\expandafter\K@Fx\expandafter\K@Ge\K@ih
??W{}{}\expandafter\K@Gc\expandafter\K@ii\K@ii{}{}\expandafter\K@Fx
??W\expandafter\K@Gf\K@ii{}{}\expandafter\K@Fx\expandafter\K@Gg\K@if
??W{}{}\expandafter\K@Gc\expandafter\K@ig\K@ig{}{}\expandafter\K@Fx
??W\expandafter\K@Gh\K@ig{}{}\K@Gi\global\expandafter\let\expandafter\K@en
??W\csname D@X\K@sa @\endcsname\expandafter\K@Fx\expandafter\K@Gj\K@hz
??W{}{}\expandafter\K@Fx\expandafter\K@Gk\K@ib{}{}\K@Gl\global\expandafter
??W\let\expandafter\K@eo\csname D@Y\K@ry @\endcsname\K@sj}\def\K@Fx
??W#1#2#3{\def\K@bf{#3}\ifx\K@bf\K@ci\let\K@bc\relax\else\def\K@bc
??W{#1{#2}{#3}\K@Fx#1}\fi\K@bc}\def\K@Gc#1{\let#1\K@ci\let\K@bf\K@ci\K@di
??W=0 \K@Gm#1}\def\K@Gm#1#2#3{\def\K@gl{#2}\ifx\K@gl\K@ci\xdef#1{#1\K@bf}\let
??W\K@bc\relax\else\def\K@bc{\K@Gm#1}\ifnum#2>\K@di\xdef#1{#1\K@bf}\def
??W\K@bf{{#2}{#3}}\K@di=#2 \else\xdef\K@bf{{#2}{#3}\K@bf}\fi\fi\K@bc}\def
??W\K@Gb#1#2{\K@Gn{#2}{#1}{#2}{-1}{<0}{\K@Go d\K@Gp}}\def\K@Gg#1#2{\K@Gn
??W{#2}{#1}{#2}{-1}{<0}{\K@Go m\K@Gq}}\def\K@Ge#1#2{\K@Gn
??W{#2}{#1}{#2}{-1}{<0}{\K@Go a\K@Gr}}\def\K@Go#1#2#3#4#5{\K@Gs{#1l}\K@Gt
??W{#4}{#5}{#3}{#5}\multiply\K@dj by -1 #2{#5}{\K@dj}}\def\K@Gd#1#2{\K@Gn
??W{#2}{#1}{#2}1{>\K@hx}{\K@Gu d\K@Gv}}\def\K@Gh#1#2{\K@Gn{#2}{#1}{#2}1{>\K@hx
??W}{\K@Gu m\K@Gq}}\def\K@Gf#1#2{\K@Gn{#2}{#1}{#2}1{>\K@hx}{\K@Gu a\K@Gr}}\def
??W\K@Gu#1#2#3#4#5{\K@Gs{#1r}\K@Gt{#4}{#5}{#5}{#3}#2{#5}{\K@dj}}\def\K@Gt
??W#1#2#3#4{\K@sg\K@ts{#1}{#2}\K@bf\expandafter\K@El\K@bf\K@ua\K@un\K@uo
??W\K@dj=\K@tz\advance\K@dj by \K@ua\divide\K@dj by 2 \advance\K@dj by
??W\csname D@X#3@\endcsname\multiply\K@dj by -1 \advance\K@dj by \csname
??WD@X#4@\endcsname\relax}\def\K@Fy#1#2{\K@Gs{dx}\K@Gw X{#1}{#2}\K@Gp\K@hx
??W1}\def\K@Gj#1#2{\K@Gs{dy}\K@Gw Y{#1}{#2}\K@Gx\K@ho1}\def\K@Ga#1#2{\K@Gs
??W{mx}\K@Gw X{#1}{#2}\K@Gq\K@hx0}\def\K@Gk#1#2{\K@Gs{my}\K@Gw Y{#1}{#2}\K@Gy
??W\K@ho0}\def\K@Fz#1#2{\K@Gs{ax}\K@Gw{}{#1}{#2}\K@Gr0{}}\def\K@Gw
??W#1#2#3#4#5#6{\setbox\K@du=\hbox{$\K@dp=#3pt$}\def\K@bc{#4{#2}}\ifdim\wd
??W\K@du=\z@\K@di=#2 \advance\K@di by 1 \ifnum\K@di>#5 \K@dp=\z@\else\K@dp
??W=\csname D@#1\the\K@di @\endcsname sp \multiply\K@dp by -1 \advance\K@dp
??Wby \csname D@#1#2@\endcsname sp \K@dp=#3\K@dp\ifcase#6 \multiply\K@dp by
??W-1 \or\edef\K@bc{\noexpand#4{\the\K@di}}\fi\fi\else\K@dp=#3 \fi\K@dk
??W=\K@dp\K@bc{\K@dk}}\endgroup
~\K@bg\flexible{\K@cz\def\K@Gz{\K@Ha}\def\K@Ev{\K@Ey}\def\K@Hb{\K@Hc}\def
~\K@sq{\K@ta}\def\K@sr{\K@sv}\let\K@om\K@oo\def\K@sf{\K@Hd}}\def\K@He{\def
~\K@Gz{\K@Hf}\let\K@Ev\K@cj\let\K@Hb\relax\def\K@sq{\K@ta0\K@tb}\let\K@sr
~\relax\let\K@sf\relax}\let\K@te\relax
??V\def\K@Hd{\K@Gs{A}\csname D@as@1@\endcsname\K@Gs{W}\csname
??VD@ws@1@\endcsname\K@Gs{C}\csname D@cs@1@\endcsname}%
~\K@bg\gravitateleft{\K@cz\let\K@te\K@cm}\K@bg\gravitateright{\K@cz\def\K@te
~{\K@hx}}
??V\def\K@Hg#1#2{\K@Gn{#2}{#1}{#2}{-1}{<0}\K@Hh}\def\K@Gn#1#2#3#4#5#6{\K@di
??V=#1 \advance\K@di by #4\relax\ifnum\K@di#5\relax\let\K@bc\K@ck\else
??V\K@ts{#2}{\the\K@di}\K@bf\ifx\K@bf\relax\edef\K@bc{\noexpand\K@Gn{\the
??V\K@di}{#2}{#3}{#4}}\else\expandafter\K@El\K@bf\K@tz\K@uk\K@ul\edef\K@bc
??V{\noexpand\K@Hi{\the\K@di}{#2}{#3}{#4}}\fi\fi\K@bc{#5}{#6}}\def\K@Hi
??V#1#2#3#4#5#6{#6{#1}{#2}{#3}}\def\K@Hh#1#2#3{\K@sg\K@ts{#2}{#3}\K@bf
??V\expandafter\K@El\K@bf\K@ua\K@un\K@uo\K@dk=\K@tz\advance\K@dk by \K@ua
??V\divide\K@dk by 2 \advance\K@dk by \csname D@X#1@\endcsname\multiply\K@dk
??Vby -1 \advance\K@dk by \csname D@X#3@\endcsname\K@dj=\csname
??VD@X#1@\endcsname\advance\K@dj by \K@dm\multiply\K@dj by -1 \advance\K@dj
??Vby \csname D@X#3@\endcsname\relax\ifnum\K@dk<\K@dj\K@dj=\K@dk\fi\ifnum
??V\K@dj<0\relax\def\K@bc{\global\let\K@sc\K@Fk\K@tc{#1}{#3}\K@Hj\K@Hk\K@Hl
??V}\else\let\K@bc\relax\fi\K@bc}\def\K@Hj#1#2{\K@Gr{#1}{\K@dj}\K@td
??V{#2}{#1}}\def\K@Hl#1#2{\multiply\K@dj by -1 \K@Gr{#2}{\K@dj}\K@td
??V{#1}{#2}}\def\K@Hk#1#2{\K@dj=\K@ua\divide\K@dj by 2 \advance\K@dj by
??V\csname D@X#1@\endcsname\multiply\K@dj by -1 \K@Gr{#1}{\K@dj}\K@dj=\K@tz
??V\divide\K@dj by 2 \multiply\K@dj by -1 \advance\K@dj by \csname
??VD@X#2@\endcsname\multiply\K@dj by -1 \K@Gr{#2}{\K@dj}}\def\K@tc
??V#1#2#3#4#5{{\K@di=#1 \multiply\K@di by 10 \advance\K@di by -\K@ij\K@dj=#2
??V\multiply\K@dj by 10 \advance\K@dj by -\K@ij\K@dk=\K@di\multiply\K@dk by
??V\K@dj\ifnum\K@dk<0 \gdef\K@bc{#4}\else\ifnum\K@di<0 \gdef\K@bc{#3}\else
??V\gdef\K@bc{#5}\fi\fi }\K@bc{#1}{#2}}\def\K@td#1#2{\K@Hm
??V{B:c#1-#2}\expandafter\xdef\csname D@Bindings@#1@\endcsname{{#2}\csname
??VD@Bindings@#1@\endcsname}}%
~\K@bk\displaybindings{\K@cz\let\K@Hm\K@Fe\let\K@sk\K@Fe}\let\K@Hm\K@cj
~\K@bg\displayall{\K@cz\let\K@Hm\K@Fe\let\K@Gs\K@Fe\let\K@Fb\K@Fe\let
~\K@sk\K@Fe}
??V\def\K@Hn#1#2#3{\def\K@bf{#3}\ifx\K@bf\K@ci\let\K@bc\K@ck\else
??V\expandafter\ifx\csname D@Bound@#2@#3@\endcsname\relax {\advance#1 by
??V\csname D@X#3@\endcsname\expandafter\xdef\csname D@X#3@\endcsname{\the
??V#1}}\K@Gs{X#3}\expandafter\let\csname D@Bound@#2@#3@\endcsname\K@ci\def
??V\K@bc{\def\K@bc{\K@Hn{#1}{#3}}\expandafter\expandafter\expandafter\K@bc
??V\csname D@Bindings@#3@\endcsname{}\K@Hn}\else\let\K@bc\K@Hn\fi\fi\K@bc
??V{#1}{#2}}\def\K@Fc#1#2#3#4{\let\K@tz\K@cm\K@Ho{#1}{#2}\K@tz\K@uk\K@ul
??V\let\K@ua\K@cm\K@Ho{#1}{#3}\K@ua\K@un\K@uo\K@sg\K@dj=\K@tz\divide\K@dj
??Vby 2 \advance\K@dj by \csname D@X#2@\endcsname\relax\ifnum#4>\K@Hp\relax
??V\advance\K@dj by #4\else\advance\K@dj by \K@Hp\fi\multiply\K@dj by -1
??V\advance\K@dj by \csname D@X#3@\endcsname\K@di=\K@ua\divide\K@di by -2
??V\advance\K@dj by \K@di\ifnum\K@dj<0 \K@tc{#2}{#3}\K@Hq{\K@Hr{#4}}\K@Hs\fi
??V}\def\K@Hq#1#2{\K@Gr{#1}{\K@dj}\K@td{#2}{#1}}\def\K@Hs#1#2{\multiply\K@dj
??Vby -1 \K@Gr{#2}{\K@dj}\K@td{#1}{#2}}\def\K@Hr#1#2#3{\K@dj=\K@ua\advance
??V\K@dj by \K@tz\divide\K@dj by 2 \ifnum#1>\K@Hp\relax\advance\K@dj by
??V#1\else\advance\K@dj by \K@Hp\fi\divide\K@dj by 2 \K@di=\csname
??VD@X#3@\endcsname\multiply\K@di by -1 \advance\K@di by \K@dj\K@Gr{#3}{\K@di
??V}\K@di=\csname D@X#2@\endcsname\advance\K@di by \K@dj\multiply\K@di by
??V-1 \K@Gr{#2}{\K@di}}\def\K@Gr#1#2{\K@Gq{#1}{#2}\def\K@bc{\K@Hn
??V{#2}{#1}}{\expandafter\expandafter\expandafter\K@bc\csname
??VD@Bindings@#1@\endcsname{}}}%
~\def\displaymovements{\K@cz\let\K@Gs\K@Fe\let\K@sk\K@Fe}\let\K@Gs\K@cj
~\def\K@Fe#1{\message{(#1)}}
??V\def\K@Gp#1#2{\K@Ht X{#1}{#2}1{<\K@hx}}\def\K@Gv#1#2{\K@Ht
??VX{#1}{#2}{-1}{>0}}\def\K@Gx#1#2{\K@Ht Y{#1}{#2}1{<\K@ho}}\def\K@Ht
??V#1#2#3#4#5{\K@di=#2 \K@cu\K@Hu{#1}{\the\K@di}{#3}\ifnum\K@di#5 \advance
??V\K@di by #4 \K@cv}\def\K@Gq#1#2{\K@Hu X{#1}{#2}}\def\K@Gy#1#2{\K@Hu
??VY{#1}{#2}}\def\K@Hu#1#2#3{\global\let\K@sc\K@Fk\K@Gs{#1#2}{\advance#3 by
??V\csname D@#1#2@\endcsname\expandafter\xdef\csname D@#1#2@\endcsname{\the
??V#3}}}\def\K@Fd#1#2#3#4#5{\ifcase#5\relax\K@Hv{#2}{#4}\or\K@Hw
??V{#1}{#2}{#3}{#4}\or\K@Hx{#1}{#2}{#3}{#4}\or\K@Hy{#1}{#2}{#3}{#4}\fi}\def
??V\K@Hv#1#2{\K@sg\K@dj=\csname D@X#1@\endcsname\advance\K@dj by \K@Hz\relax
??V\multiply\K@dj by -1 \advance\K@dj by \csname D@X#2@\endcsname\relax
??V\ifnum\K@dj<0 \K@tc{#1}{#2}\K@Hq\K@Ia\K@Hs\fi}\def\K@Hw#1#2#3#4{\K@sg\let
??V\K@tz\K@cm\let\K@gl\K@cm\K@Ho{#1}{#2}\K@tz\K@uk\K@ul\K@Ho{#1}{#4}\K@gl
??V\K@un\K@uo\K@Ib{#2}{#4}\K@dj\K@tz\K@gl\let\K@gl\K@cm\let\K@ua\K@cm\K@Ho
??V{#3}{#2}\K@gl\K@uk\K@ul\K@Ho{#3}{#4}\K@ua\K@un\K@uo\K@Ib{#2}{#4}\K@dk
??V\K@gl\K@ua\relax\ifnum\K@dk<\K@dj\K@dj=\K@dk\fi\ifnum\K@dj<0 \K@tc
??V{#2}{#4}\K@Hq\K@Ic\K@Hs\fi}\def\K@Hx#1#2#3#4{\K@sg\let\K@tz\K@cm\let
??V\K@ua\K@cm\let\K@gl\K@cm\K@Ho{#1}{#2}\K@tz\K@uk\K@ul\K@Ho{#3}{#4}\K@ua
??V\K@un\K@uo\K@Ho{#3}{#2}\K@gl\K@uk\K@ul\K@Ib{#2}{#4}\K@dj\K@gl\K@ua\relax
??V\ifnum\K@dj<0 \K@tc{#2}{#4}\K@Hq\K@Ic\K@Hs\fi}\def\K@Hy#1#2#3#4{\K@sg\let
??V\K@tz\K@cm\let\K@ua\K@cm\let\K@gl\K@cm\K@Ho{#1}{#2}\K@tz\K@uk\K@ul\K@Ho
??V{#3}{#4}\K@ua\K@un\K@uo\K@Ho{#1}{#4}\K@gl\K@un\K@uo\K@Ib{#2}{#4}\K@dj
??V\K@tz\K@gl\relax\ifnum\K@dj<0 \K@tc{#2}{#4}\K@Hq\K@Ic\K@Hs\fi}\def\K@Ib
??V#1#2#3#4#5{#3=#4 \advance#3 by #5 \divide#3 by 2 \advance#3 by \csname
??VD@X#1@\endcsname\advance#3 by \K@Id\multiply#3 by -1 \advance#3 by
??V\csname D@X#2@\endcsname}\def\K@Ic#1#2{\K@dk=\K@tz\multiply\K@dk by -1
??V\advance\K@dk by \K@ua\divide\K@dk by 2 \advance\K@dk by \csname
??VD@X#1@\endcsname\advance\K@dk by \csname D@X#2@\endcsname {\advance\K@dj
??Vby \K@dk\divide\K@dj by -2 \K@Gr{#2}{\K@dj}}{\advance\K@dj by -\K@dk\divide
??V\K@dj by 2 \K@Gr{#1}{\K@dj}}}\def\K@Ia#1#2{\K@di=\K@Hz\divide\K@di by 2
??V\K@dj=\csname D@X#2@\endcsname\multiply\K@dj by -1 \advance\K@dj by \K@di
??V\K@Gr{#2}{\K@dj}\K@dj=\csname D@X#1@\endcsname\advance\K@dj by \K@di
??V\multiply\K@dj by -1 \K@Gr{#1}{\K@dj}}\def\K@Ho#1#2#3#4#5{\K@ts
??V{#1}{#2}\K@bf\ifx\K@bf\relax\else\expandafter\K@El\K@bf#3#4#5\fi}\def
??V\K@Ie#1#2#3{{\K@di=0 \K@dk=0 \K@cu\expandafter\xdef\csname D@#1\the\K@di
??V@\endcsname{\the\K@dk}\ifnum\K@di<#3\relax\advance\K@di by 1 \advance\K@dk
??Vby #2\relax\K@cv }}\def\K@Hf{\K@Ie X\K@dm\K@hx}\def\K@Ha{\K@Ie X\z@\K@hx
??V}\def\K@If{\K@Ie Y\K@dn\K@ho}\def\K@sg{\K@Gz\K@If\let\K@sg\relax}\def\K@Ig
??V#1#2#3{\K@di=0 \K@cu\ifnum\K@di<#3\relax\K@dj=\K@di\K@dk=\csname
??VD@#1\the\K@di @\endcsname\multiply\K@dk by -1 \advance\K@di by 1 \advance
??V\K@dk by \csname D@#1\the\K@di @\endcsname\expandafter\xdef\csname
??VD@d#2\the\K@dj @\endcsname{\the\K@dk}\K@cv}\def\K@sj{\K@sg\K@Ig Xx\K@hx
??V\K@Ig Yy\K@ho}\def\K@Ih#1#2#3#4{\K@di=\csname D@#10@\endcsname\K@dj=0
??V\K@dk=\K@di\global\let#3\K@cm\global\let#4\K@cm\K@cu\ifnum\csname
??VD@#1\the\K@dj @\endcsname<\K@di\xdef#3{\the\K@dj}\K@di=\csname D@#1\the
??V\K@dj @\endcsname\fi\ifnum\csname D@#1\the\K@dj @\endcsname>\K@dk\xdef
??V#4{\the\K@dj}\K@dk=\csname D@#1\the\K@dj @\endcsname\fi\ifnum\K@dj<#2
??V\advance\K@dj by 1 \K@cv\ifnum\K@di=0 \else\multiply\K@di by -1 \K@dj=0
??V\K@cu\K@dk=\csname D@#1\the\K@dj @\endcsname\advance\K@dk by \K@di
??V\expandafter\xdef\csname D@#1\the\K@dj @\endcsname{\the\K@dk}\ifnum\K@dj
??V<#2\relax\advance\K@dj by 1 \K@cv\fi}\def\K@Gi{\K@Ih X\K@hx\K@rz\K@sa
??V}\def\K@Gl{\K@Ih Y\K@ho\K@rx\K@ry}\def\K@tg{\let\K@rt\K@ru\let\K@ni\K@cm
??V\K@Ii\global\setbox\K@dt=\hbox\bgroup$\vertexstyle\K@gy\K@gz\K@rv}%
~\def\K@rv{\let\box\copy\let\unhbox\unhcopy\let\unvbox\unvcopy}\def\K@ru
~{$\egroup}
??A\begingroup\K@ce\def\K@Ij{\ifx\K@Ik\relax\expandafter\global\expandafter
??A\edef\K@tf{\let\expandafter\noexpand\csname D@\the\K@df @\the\K@de
??A@\endcsname\noexpand\K@ci}\else\expandafter\global\expandafter\let\K@tf
??A\relax\fi}%
~\def\K@Il{\expandafter\global\expandafter\let\K@tf\relax}\K@bg\dotted{\K@cz
~\K@cc\def\K@yr{\K@Im}\def\K@Ii{\K@In}\def\K@Il{\K@Ij}\def\K@Io{\K@Ip}}\let
~\K@yr\relax\let\K@Ii\relax\let\K@Io\K@ck\def\K@oe{\global\let\K@Ik\relax}
??A\def\K@In{\let\K@Ik\K@ci}\def\K@Ip#1#2{\expandafter\let\csname
??AD@#1@#2@\endcsname\K@ci}%
??V\def\K@th{\K@rt\K@ts{\the\K@df}{\the\K@de}\K@bf\ifx\K@bf\relax\K@Il
??V\else\K@Hb\fi}%
??A\def\K@Im{\K@di=0 \K@dj=0 \K@cu\K@cu\expandafter\let \expandafter\K@bf
??A\csname D@\the\K@di @\the\K@dj @\endcsname\ifx\K@bf\K@ci\else\K@dk=\K@ho
??A\advance\K@dk by -\K@di\edef\K@bc{\noexpand\K@Ej1@\the\K@dj,\the\K@dk
??A@}{\K@bc{\lower\K@vj\hbox{$\vertexstyle\diagramdot$}}}\fi\ifnum\K@dj<\K@hx
??A\advance\K@dj by 1 \K@cv\ifnum\K@di<\K@ho\advance\K@di by 1 \K@dj=0
??A\K@cv}\endgroup
??V\def\K@Hc{{\K@di=\K@sx\relax\advance\K@di by 1 \K@Fb{C:r\the\K@df,c\the
??V\K@de}\K@dj=\K@de\multiply\K@dj by 10 \ifnum\K@dj<\K@ij\relax\let\K@bc
??V\K@cr\else\let\K@bc\K@cq\fi\expandafter\xdef\csname D@cs@\K@sx
??V@\endcsname{\K@bc{\noexpand\K@Hg{\the\K@df}{\the\K@de}}{\expandafter
??V\noexpand\csname D@cs@\the\K@di @\endcsname}}\xdef\K@sx{\the\K@di}}\global
??V\expandafter\let\csname D@cs@\K@sx @\endcsname\relax}\def\K@Ex
??V#1@#2@#3@#4@#5@#6@#7@#8@#9@{\def\K@tm{#3}\def\K@tn{#4}\def\K@to{#5}\def
??V\K@tp{#6}\K@Iq\K@tm\K@tn\K@tz\K@uk\K@ul\K@Iq\K@to\K@tp\K@ua\K@un\K@uo
??V\edef\K@pb{\K@Ep0#8}\expandafter\K@Ir\K@pb\K@pb\K@rl\edef\K@pc{\K@Ep
??V1#8}\expandafter\K@Ir\K@pc\K@pc\K@pd\edef\K@qb{\K@Ep2#8}\expandafter\K@Ir
??V\K@qb\K@qb\K@py\edef\K@qc{\K@Ep3#8}\expandafter\K@Ir\K@qc\K@qc\K@qd\edef
??V\K@pz{\K@Ep4#8}\expandafter\K@Ir\K@pz\K@pz\K@qa\edef\K@pu{\K@Ep
??V5#8}\expandafter\K@Ir\K@pu\K@pu\K@qt\ifx\K@pu\K@cl\let\K@qs\K@ci\else
??V\let\K@qs\relax\fi\edef\K@qj{\K@Ep6#8}\expandafter\K@Ir\K@qj\K@qj\K@qm
??V\edef\K@qi{\K@Ep7#8}\expandafter\K@Ir\K@qi\K@qi\K@ql\let\K@rq\relax\let
??V\K@rs\relax\K@di=\K@ho\advance\K@di by -\K@tm\edef\K@tm{\the\K@di}\K@di
??V=\K@ho\advance\K@di by -\K@to\edef\K@to{\the\K@di}\edef\K@qy{\K@Ep
??V0#9{}{}{}{}{}}\edef\K@re{\K@Ep1#9{}{}{}{}{}}\edef\K@rf{\K@Ep
??V2#9{}{}{}{}{}}\expandafter\K@Is\K@qy @\ifx\K@rb\relax\ifx\K@pb\K@ci\edef
??V\K@pb{\K@Dl#2}\fi\fi\expandafter\K@tt{#1}{#2}{#7}}\def\K@Is#1#2@{\ifcase
??V#1 \let\K@rc\relax\let\K@rb\relax\or\let\K@rc\K@ci\let\K@rb\relax\def
??V\K@qy{#2}\or\let\K@rc\K@ci\let\K@rb\K@ci\def\K@qy{#2}\fi}\def\K@Ir
??V#1#2#3#4{\def#3{#1}\def#4{#2}}\def\K@Iq#1#2#3#4#5{\K@ts{#1}{#2}\K@bf\ifx
??V\K@bf\relax\let#3\K@cm\let#4\K@cm\let#5\K@cm\else\expandafter\K@El\K@bf
??V#3#4#5\fi}\def\K@El#1@#2@#3@#4#5#6{\def#4{#1}\def#5{#2}\def#6{#3}}\def
??V\K@ts#1#2#3{\expandafter\let \expandafter#3\csname D@whd@#1@#2@\endcsname}%
~\def\K@ub#1by #2#3{\K@di=#3 \multiply\K@di by #2 \advance\K@di by #1 \edef
~#1{\the\K@di}}\def\K@ty#1#2#3{\ifx#2\K@ci\let#2\K@cm\else\setbox\K@du
~=\hbox{\K@do=#2pt}\ifdim\wd\K@du>\z@\K@do=#2 \K@di=\K@do\multiply\K@di by
~#1 \edef#2{\the\K@di}\else\ifx#3\K@ci\let#2\K@cm\else\K@do=#3sp \K@do
~=#2\K@do\K@di=\K@do\multiply\K@di by -2 \advance\K@di by #3 \divide\K@di
~by -2 \edef#2{\the\K@di}\fi\fi\fi}\def\K@vs#1=#2\times#3\over#4{\ifnum
~#3<10737418 #1=#3 \multiply#1 by 100 \divide#1 by #4\relax\multiply#1 by
~#2\relax\divide#1 by 100 \else {\ifnum#2<0 \multiply#2 by -1 \multiply#4
~by -1 \fi\K@It#1=#2\times#3\over#4}\fi}\def\K@It#1=#2\times#3\over#4{\K@de
~=1 \K@cu\multiply\K@de by 2 \ifnum#2>\K@de\K@cv\K@df=#3 \divide\K@df by
~\K@de\divide#4 by \K@de\multiply\K@df by #2\relax\divide\K@df by
~#4\relax\xdef\K@bc{#1=\the\K@df}\aftergroup\K@bc}\def\K@uh{\K@di=\K@ug
~\relax\ifnum\K@di<0 \multiply\K@di by -1 \fi\K@dj=\K@uf\relax\ifnum\K@dj
~<0 \multiply\K@dj by -1 \fi\K@dk=1 \let\K@bf\K@ci\K@cu\ifnum\K@di<23171
~\ifnum\K@dj<23171 \let\K@bf\relax\fi\fi\ifx\K@bf\K@ci\divide\K@di by 2
~\divide\K@dj by 2 \multiply\K@dk by 2 \K@cv\multiply\K@di by \K@di
~\multiply\K@dj by \K@dj\advance\K@di by \K@dj\expandafter\K@Iu\the\K@di
~=\K@dj\multiply\K@dj by \K@dk\edef\K@tw{\the\K@dj}}\def\K@Iu#1=#2{{\K@dh
~=#1\relax\K@df=32768 \K@de=0 \K@cu\divide\K@df by 2 \K@dg=\K@de\advance
~\K@dg by \K@df\multiply\K@dg by \K@dg\ifnum\K@dg>\K@dh\else\advance
~\K@de by \K@df\fi\ifnum\K@df>1 \K@cv\global#2=\K@de}}\def\K@wu#1=#2\mod
~#3{#1=#2\relax\ifnum#1<0 \K@cu\advance#1 by #3\relax\ifnum#1<0 \K@cv
~\else\K@cu\ifnum#1>#3\relax\advance#1 by -#3\relax\K@cv\ifnum
~#1=#3\relax #1=0 \fi\fi}
??V\def\K@yp#1@#2@#3@{\K@Io{#1}{#2}\setbox\K@du=\hbox{\K@Iv#3\K@rt}\K@dx{\K@dr
??V={\K@Iv#3\K@rt}}{{}{0}{\setbox\K@du=\hbox{\the\K@dr}}}\K@Iw{#1}{#2}\K@di
??V=\K@ho\advance\K@di by -#1 \edef\K@bc{\noexpand\K@Ej1@#2,\the\K@di @}\K@bc
??V{\lower\K@vj\hbox{\box\K@dt}}}\def\K@Iw#1#2{\K@di=\wd\K@dt\divide\K@di by
??V2 \K@dj=\K@di\advance\K@dj by \csname D@X#2@\endcsname\advance\K@dj by
??V-\K@en\advance\K@dj by -\K@ev\relax\ifnum\K@dj>0 \advance\K@dj by \K@ev
??V\xdef\K@ev{\the\K@dj}\fi\K@dj=\K@di\advance\K@dj by -\csname
??VD@X#2@\endcsname\advance\K@dj by -\K@eu\relax\ifnum\K@dj>0 \advance\K@dj
??Vby \K@eu\xdef\K@eu{\the\K@dj}\fi\K@di=\wd\K@dt\advance\K@di by \ht\K@dt
??V\advance\K@di by \dp\K@dt\ifnum\K@di>0 \ifnum#1=\K@rx\K@dj=\ht\K@dt
??V\ifnum\K@dj>\K@es\xdef\K@es{\the\K@dj}\fi\fi\ifnum#1=\K@ry\K@dj=\dp
??V\K@dt\relax\ifnum\K@dj>\K@et\xdef\K@et{\the\K@dj}\fi\fi\fi}%
??S\def\K@yz#1#2#3#4#5{\K@di=#3 \divide\K@di by 2 \K@dj=\K@di\advance\K@dj
??Sby #1 \advance\K@dj by -\K@en\advance\K@dj by -\K@ev\relax\ifnum\K@dj>0
??S\advance\K@dj by \K@ev\xdef\K@ev{\the\K@dj}\fi\K@dj=#1\advance\K@dj by
??S\K@eu\multiply\K@dj by -1 \advance\K@dj by \K@di\relax\ifnum\K@dj>0
??S\advance\K@dj by \K@eu\xdef\K@eu{\the\K@dj}\fi\K@di=#4 \advance\K@di by
??S#2\relax\ifnum\K@di>\K@eo\relax\advance\K@di by -\K@eo\relax\ifnum\K@di
??S>\K@es\relax\xdef\K@es{\the\K@di}\fi\fi\K@di=#2 \multiply\K@di by -1
??S\advance\K@di by #5\relax\ifnum\K@di>0\relax\ifnum\K@di>\K@et\relax\xdef
??S\K@et{\the\K@di}\fi\fi}\endgroup
??V\def\K@Iv{\let\K@rt\K@ru\global\setbox\K@dt=\hbox\bgroup$\vertexstyle\K@gx
??V}\endgroup
~\def\K@vj{\fontdimen22\textfont2}\def\K@Ix#1#2#3#4{\let\K@gl\K@ci\K@Iy
~#1#2{}\ifx\K@gl\relax#3\else#4\fi}\def\K@Iy#1#2#3{\if\noexpand#1#2\let
~\K@gl\relax\fi\def\K@bf{#3}\ifx\K@bf\K@ci\let\K@bc\relax\else\def\K@bc
~{\K@Iy#1#3}\fi\K@bc}\def\K@Iz{\let\K@Ja\relax\K@dr={}\futurelet\K@jr\K@Jb
~}\def\K@Jb{\if=\noexpand\K@jr\def\K@bc{\K@Jc\expandafter\futurelet
~\expandafter\K@jr\expandafter\K@Jd @}\else\if\noexpand\K@jr\K@bn\def
~\K@bc{\K@pa\expandafter\futurelet\expandafter\K@jr\expandafter\K@Jb
~@}\else\def\K@bc{\expandafter\futurelet\expandafter\K@jr\expandafter
~\K@Je}\fi\fi\K@bc}\def\K@Jd{\if\noexpand\K@jr\K@bn\def\K@bc{\K@pa
~\expandafter\futurelet\expandafter\K@jr\expandafter\K@Je @}\else\let\K@bc
~\K@Je\fi\K@bc}\def\K@Jc#1@#2{#1}\def\K@pa#1@ {#1}\def\K@Je{\if-\noexpand
~\K@jr\def\K@bc{\K@dr={-}\K@Jc\expandafter\futurelet\expandafter\K@jr
~\expandafter\K@Jf @}\else\let\K@bc\K@Jg\fi\K@bc}\def\K@Jf{\if\noexpand
~\K@jr\K@bn\def\K@bc{\K@pa\expandafter\futurelet\expandafter\K@jr
~\expandafter\K@Jg @}\else\let\K@bc\K@Jg\fi\K@bc}\def\K@Jg{\if.\noexpand
~\K@jr\ifx\K@Ja\relax\let\K@Ja\K@ci\let\K@bc\K@Jh\else\if\noexpand\K@jr
~\K@bn\def\K@bc{\K@pa\K@Ji @}\else\let\K@bc\K@Ji\fi\fi\else\K@Ix\K@jr
~{0123456789}{\let\K@Ji\K@Jj\let\K@bc\K@Jh}{\if\noexpand\K@jr\K@bn\def\K@bc
~{\K@pa\K@Ji @}\else\let\K@bc\K@Ji\fi}\fi\K@bc}\def\K@Jh#1{\edef\K@bc
~{\K@dr={\the\K@dr#1}}\K@bc\futurelet\K@jr\K@Jg}\def\K@qq{\ifcat\noexpand
~\K@jr\bgroup\def\K@bc{\bgroup\K@ez\K@jp}\else\let\K@bc\K@jq\fi\K@bc
~}\def\K@Jk#1#2{\K@cz\def\K@jp##1{\egroup\def\K@Ji{\expandafter\let\csname
~D@##1@#1@\endcsname\K@ci}\def\K@Jj{\expandafter\edef\csname
~D@##1@#1@\endcsname{\the\K@dr}}\K@Iz}\def\K@jq{\let\K@Ji\relax\def\K@Jj
~{\edef#2{\the\K@dr}}\K@Iz}\futurelet\K@jr\K@qq}\K@bk\labelpoint{\K@Jk
~{lpt}\K@Ff}\K@bk\ptpoint{\K@Jk{ppt}\K@Fg}\def\K@Jl{\if\noexpand\K@jr\K@bn
~\def\K@bc{\K@pa\futurelet\K@jr\K@Jl @}\else\if+\noexpand\K@jr\def\K@bc
~{\K@Jc\futurelet\K@jr\K@Jm @}\else\def\K@bc{\afterassignment\K@Jn\K@do}\fi
~\fi\K@bc}\def\K@Jm{\if\noexpand\K@jr\K@bn\def\K@bc{\K@pa\futurelet\K@jr
~\K@Jm @}\else\if=\noexpand\K@jr\def\K@bc{\afterassignment\K@Jo\K@do}\else
~\def\K@bc{\afterassignment\K@Jn\K@do}\fi\fi\K@bc}\def\K@Jp#1{\edef
~#1{\the\K@do}}\def\K@Jq#1{\edef#1{\the\K@di}}\def\K@Jr#1{\K@di=\K@do\K@Jq
~#1}\def\K@Js#1{\advance\K@do by #1\edef#1{\the\K@do}}\def\K@Jt#1{\advance
~\K@di by #1\edef#1{\the\K@di}}\def\K@Ju#1{\K@di=\K@do\K@Jt#1}\def\K@Jv
~#1#2{\K@cz\def\K@jp##1{\egroup\def\K@Jo{\expandafter\K@Ju\csname
~D@##1@#1@\endcsname}\def\K@Jn{\expandafter\K@Jr\csname D@##1@#1@\endcsname
~}\futurelet\K@jr\K@Jl}\def\K@jq{\def\K@Jo{\K@Ju#2}\def\K@Jn{\K@Jr
~#2}\futurelet\K@jr\K@Jl}\futurelet\K@jr\K@qq}\K@bk\labelwidthpad{\K@Jv
~{lwp}\K@ou}\K@bk\labelpad{\K@Jv{lp}\K@or}\K@bk\breakpad{\K@Jv{bp}\K@Du
~}\K@bk\cellpush{\K@Jv{cp}\K@wp}\K@bk\ptpush{\K@Jv{pp}\K@wr}\K@bk\atpush
~{\K@Jv{ap}\K@wt}\K@bk\joinpush{\K@Jv{jp}\K@wn}\def\K@Jw#1#2{\K@cz\def\K@Jo
~{#1}\def\K@Jn{#2}\futurelet\K@jr\K@Jl}\K@bg\MinimumCellLength{\K@Jw {\K@Ju
~\K@ut}{\K@Jr\K@ut}}\K@bg\celllength{\K@Jw {\K@Ju\K@Ds}{\K@Jr\K@Ds}}\K@bg
~\cellwidth{\K@Jw {\K@Ju\K@Hp}{\K@Jr\K@Hp}}\K@bg\columndist{\K@Jw {\K@Ju
~\K@Hz}{\K@Jr\K@Hz}}\K@bg\bracewidth{\K@Jw {\K@Ju\K@Id}{\K@Jr\K@Id}}\K@bk
~\Diagrampad{\K@Jw {\K@Js\K@Ay}{\K@Jp\K@Ay}}\K@bk\Figurepad{\K@Jw {\K@Js
~\K@hk}{\K@Jp\K@hk}}\K@bk\Graphpad{\K@Jw {\K@Js\K@hl}{\K@Jp\K@hl}}\K@bg\tpad
~{\K@Jw {\K@Js\K@Be}{\K@Jp\K@Be}}\K@bg\bpad{\K@Jw {\K@Js\K@Bf}{\K@Jp\K@Bf
~}}\K@bg\lpad {\K@Jw{\K@Js\K@Bd}{\K@Jp\K@Bd}}\K@bg\rpad {\K@Jw{\K@Js\K@Bg
~}{\K@Jp\K@Bg}}\K@bg\vpad{\K@Jw {\K@dp=\K@do\K@Js\K@Be\K@do=\K@dp\K@Js\K@Bf
~}{\K@Jp\K@Be\let\K@Bf\K@Be}}\K@bg\hpad{\K@Jw {\K@dp=\K@do\K@Js\K@Bd\K@do
~=\K@dp\K@Js\K@Bg}{\K@Jp\K@Bd\let\K@Bg\K@Bd}}\K@bg\framepad{\K@Jw {\K@Js
~\K@Ci}{\K@Jp\K@Ci}}\K@bg\framerulewidth{\K@Jw {\K@Js\K@Cl}{\K@Jp\K@Cl
~}}\K@bg\Rulewidth{\K@Jw {\K@Js\K@Dq}{\K@Jp\K@Dq}}\K@bg\Framerulewidth{\K@Jw
~{\K@Js\K@Cw}{\K@Jp\K@Cw}}\def\K@il{\let\xgrid\K@dm\let\ygrid\K@dn}\def
~\K@Ae{\let\xunit\K@dm\let\yunit\K@dn}\def\K@Jx#1#2{\ifdim#1<\z@\else#2\fi
~}\K@bg\xgrid{\K@Jw {\advance\K@do by \K@dm\K@Jx\K@do{\K@dm=\K@do\let\K@Jy
~\K@co}}{\K@Jx\K@do{\K@dm=\K@do\let\K@Jy\K@co}}}\K@bg\ygrid{\K@Jw {\advance
~\K@do by \K@dn\K@Jx\K@do{\K@dn=\K@do\let\K@Jz\K@co}}{\K@Jx\K@do{\K@dn
~=\K@do\let\K@Jz\K@co}}}\K@bg\grid{\K@Jw {\K@dp=\K@do\advance\K@do by \K@dm
~\K@Jx\K@do{\K@dm=\K@do\let\K@Jy\K@co}\advance\K@dp by \K@dn\K@Jx\K@dp
~{\K@dn=\K@dp\let\K@Jz\K@co}}{\K@Jx\K@do{\K@dm=\K@do\let\K@Jy\K@co\K@dn
~=\K@do\let\K@Jz\K@co}}}\def\K@Ka#1#2{\ifdim#1>\z@#2\fi}\K@bg\xunit{\K@Jw
~{\ifx\K@zx\K@ci\else\advance\K@do by \K@zx\fi\K@Ka\K@do{\K@Jp\K@zx}}{\K@Ka
~\K@do{\K@Jp\K@zx}}}\K@bg\yunit{\K@Jw {\ifx\K@zz\K@ci\else\advance\K@do by
~\K@zz\fi\K@Ka\K@do{\K@Jp\K@zz}}{\K@Ka\K@do{\K@Jp\K@zz}}}\K@bg\unit{\K@Jw
~{\K@dp=\K@do\ifx\K@zx\K@ci\else\advance\K@do by \K@zx\fi\K@Ka\K@do{\K@Jp
~\K@zx}\ifx\K@zz\K@ci\else\advance\K@dp by \K@zz\fi\K@Ka\K@dp{\edef\K@zz
~{\the\K@dp}}}{\K@Ka\K@do{\K@Jp\K@zx\let\K@zz\K@zx}}}\K@bg\xscale{\K@cz\let
~\K@Ji\relax\def\K@Jj{\K@do=\the\K@dr\K@dm\ifdim\K@do<\z@\else\K@dm=\K@do
~\edef\K@Jy{\the\K@dr}\fi}\K@Iz}\K@bg\yscale{\K@cz\let\K@Ji\relax\def\K@Jj
~{\K@do=\the\K@dr\K@dn\ifdim\K@do<\z@\else\K@dn=\K@do\edef\K@Jz{\the\K@dr
~}\fi}\K@Iz}\K@bg\scale{\K@cz\let\K@Ji\relax\def\K@Jj{\K@do=\the\K@dr\K@dm
~\ifdim\K@do<\z@\else\K@dm=\K@do\K@dn=\the\K@dr\K@dn\edef\K@Jy{\the\K@dr
~}\let\K@Jz\K@Jy\fi}\K@Iz}\def\K@Kb{\ifnum\K@di>0 \K@Ji\fi}\K@bg\xrange
~{\K@cz\def\K@Ji{\K@Jq\K@zy\let\K@zx\K@ci}\afterassignment\K@Kb\K@di}\K@bg
~\yrange{\K@cz\def\K@Ji{\K@Jq\K@Aa\let\K@zz\K@ci}\afterassignment\K@Kb\K@di
~}\K@bg\range{\K@cz\def\K@Ji{\K@Jq\K@zy\let\K@Aa\K@zy\let\K@zx\K@ci\let
~\K@zz\K@ci}\afterassignment\K@Kb\K@di}\K@bg\gridgray{\K@cz\let\K@Ji\relax
~\def\K@Jj{\edef\K@bc{\noexpand\K@Dg{\the\K@dr}}\K@bc\K@Dh}\K@Iz}\K@bm
~\gridgrey\gridgray\K@bg\graygray{\K@cz\let\K@Ji\relax\def\K@Jj{\edef
~\K@bc{\noexpand\K@Dg{\the\K@dr}}\K@bc\K@pv}\K@Iz}\K@bm\greygrey\graygray
~\K@bg\framegray{\K@cz\let\K@Ji\relax\def\K@Jj{\edef\K@bc{\noexpand\K@Dg
~{\the\K@dr}}\K@bc\K@Kc\ifx\K@Kc\K@ci\let\K@Ck\relax\let\K@Cm\relax\else
~\edef\K@Ck{\noexpand\K@ha{\K@Kc}}\def\K@Cm{\endgr}\fi}\K@Iz}\K@bm
~\framegrey\framegray\K@bg\shadegray{\K@cz\let\K@Ji\relax\def\K@Jj{\edef
~\K@bc{\noexpand\K@Dg{\the\K@dr}}\K@bc\K@Kd\ifx\K@Kd\K@ci\let\K@Cq\relax
~\let\K@Cr\relax\else\edef\K@Cq{\noexpand\K@ha{\K@Kd}}\def\K@Cr{\endgr}\fi
~}\K@Iz}\K@bm\shadegrey\shadegray\kuviocs\MinimumCellLength=0pt \K@He\ifx
~\@@agss@arrsy@@\relax\else\let\A@rightarrow\rightarrow\let\A@leftarrow
~\leftarrow\let\A@leftrightarrow\leftrightarrow\let\A@leftharpoonup
~\leftharpoonup\let\A@leftharpoondown\leftharpoondown\let\A@rightharpoonup
~\rightharpoonup\let\A@rightharpoondown\rightharpoondown\fi\K@bg\latexTo
~{\font\K@Ke=line10 \def\K@Kf{\smash{\hbox{\kern-4pt\raise\K@vj\hbox{\K@Ke
~\char"2D}\hskip.5pt}}}\newfill{srightarrow}--\K@Kf\newfill
~{sleftarrow}\K@Kf--\let\Tofill\srightarrowfill}\K@bk\newfill{\bgroup\K@ez
~\K@Kg}\def\K@Kg#1{\egroup\K@Kh{#1}}\def\K@Kh#1#2#3#4{\expandafter\def
~\csname D@@#1fill\endcsname{\m@th\mathord{#2}\mkern-8mu \cleaders\hbox
~{$\mkern-2mu\mathord{#3}\mkern-2mu$}\hfill\mkern-8mu\mathord
~{#4}}\expandafter\K@bk\csname#1fill\endcsname{\ifmmode\csname
~D@@#1fill\endcsname\else $\csname D@@#1fill\endcsname$\fi}}
\K@ab
%-----------------------------------------------------------------------------
\rekuviodef\into{\lhook\joinrel\A@rightarrow}
\rekuviodef\cdotfill{\cleaders
   \hbox{$\m@th\mkern1.5mu\mathord\cdot\mkern1.5mu$}\hfill}
\rekuviolet\cmleftarrowfill\leftarrowfill

\newfill{leftarrow}\A@leftarrow--
\newfill{rleftarrow}{-\mkern-12mu\A@leftarrow\mkern-5mu}--
\newfill{Leftarrow}\Leftarrow==
\newfill{leftharpoonup}\A@leftharpoonup--
\newfill{leftharpoondown}\A@leftharpoondown--
\newfill{hookleftarrow}\A@leftarrow-{-\mkern-8mu\rhook}
\rekuviolet\leftintofill\hookleftarrowfill
\newfill{lleftarrow}{\A@leftarrow\mkern-13mu\A@leftarrow\mkern-5mu}--
\newfill{leftepi}{\A@leftarrow\mkern-15mu\A@leftarrow\mkern-3mu}--
\newfill{rlleftarrow}{-\mkern-12mu\A@leftarrow\mkern-13mu\A@leftarrow
   \mkern-5mu}--
\newfill{llleftarrow}{\A@leftarrow\mkern-13mu\A@leftarrow
   \mkern-13mu\A@leftarrow\mkern-10mu}--
\newfill{rllleftarrow}{-\mkern-12mu\A@leftarrow\mkern-13mu\A@leftarrow
   \mkern-13mu\A@leftarrow\mkern-10mu}--

\rekuviolet\cmrightarrowfill\rightarrowfill
\newfill{rightarrow}--\A@rightarrow
\newfill{lrightarrow}--{\mkern-5mu\A@rightarrow\mkern-12mu-}
\newfill{Rightarrow}==\Rightarrow
\newfill{rightharpoonup}--\A@rightharpoonup
\newfill{rightharpoondown}--\A@rightharpoondown
\newfill{hookrightarrow}{\lhook\mkern-8mu-}-\A@rightarrow
\rekuviolet\rightintofill\hookrightarrowfill
\newfill{rrightarrow}--{\mkern-5mu\A@rightarrow\mkern-13mu\A@rightarrow}
\newfill{rightepi}--{\mkern-3mu\A@rightarrow\mkern-15mu\A@rightarrow}
\newfill{lrrightarrow}--{\mkern-5mu\A@rightarrow\mkern-13mu\A@rightarrow
   \mkern-12mu-}
\newfill{rrrightarrow}--{\mkern-10mu\A@rightarrow\mkern-13mu\A@rightarrow
   \mkern-13mu\A@rightarrow}
\newfill{lrrrightarrow}--{\mkern-10mu\A@rightarrow\mkern-13mu\A@rightarrow
   \mkern-13mu\A@rightarrow\mkern-12mu-}

\newfill{relbar}---
\rekuviolet\linefill\relbarfill
\newfill{Relbar}===
\rekuviolet\barfill\Relbarfill
\newfill{mapsto}{\mapstochar\mkern-5mu-}-\A@rightarrow
\newfill{leftrightarrow}\A@leftarrow-\A@rightarrow
\newfill{Leftrightarrow}\Leftarrow=\Rightarrow

\def\kuviojoin{\hbox{$\mkern-8mu$}}

\kuviodef\leftarrowxfill{\leftarrowfill\kuviojoin\relbarfill}
\kuviodef\leftarrowxxfill{\leftarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill}
\kuviodef\xleftarrowxfill{\relbarfill\kuviojoin\leftarrowfill
   \kuviojoin\relbarfill}
\kuviodef\leftarrowxxxfill{\leftarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill\kuviojoin\relbarfill}
\kuviodef\xxleftarrowxfill{\relbarfill\kuviojoin\relbarfill
   \kuviojoin\leftarrowfill\kuviojoin\relbarfill}

\kuviodef\rightarrowxfill{\rightarrowfill\kuviojoin\relbarfill}
\kuviodef\rightarrowxxfill{\rightarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill}
\kuviodef\xrightarrowxfill{\relbarfill\kuviojoin\rightarrowfill
   \kuviojoin\relbarfill}
\kuviodef\rightarrowxxxfill{\rightarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill\kuviojoin\relbarfill}
\kuviodef\xxrightarrowxfill{\relbarfill\kuviojoin\relbarfill
   \kuviojoin\rightarrowfill\kuviojoin\relbarfill}

\kuviodef\lleftarrowxfill{\lleftarrowfill\kuviojoin\relbarfill}
\kuviodef\lleftarrowxxfill{\lleftarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill}
\kuviodef\xlleftarrowxfill{\relbarfill\kuviojoin\lleftarrowfill
   \kuviojoin\relbarfill}
\kuviodef\lleftarrowxxxfill{\lleftarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill\kuviojoin\relbarfill}
\kuviodef\xxlleftarrowxfill{\relbarfill\kuviojoin\relbarfill
   \kuviojoin\lleftarrowfill\kuviojoin\relbarfill}

\kuviodef\rrightarrowxfill{\rrightarrowfill\kuviojoin\relbarfill}
\kuviodef\rrightarrowxxfill{\rrightarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill}
\kuviodef\xrrightarrowxfill{\relbarfill\kuviojoin\rrightarrowfill
   \kuviojoin\relbarfill}
\kuviodef\rrightarrowxxxfill{\rrightarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill\kuviojoin\relbarfill}
\kuviodef\xxrrightarrowxfill{\relbarfill\kuviojoin\relbarfill
   \kuviojoin\rrightarrowfill\kuviojoin\relbarfill}

\kuviodef\llleftarrowxfill{\llleftarrowfill\kuviojoin\relbarfill}
\kuviodef\llleftarrowxxfill{\llleftarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill}
\kuviodef\xllleftarrowxfill{\relbarfill\kuviojoin\llleftarrowfill
   \kuviojoin\relbarfill}

\kuviodef\llleftarrowxxxfill{\llleftarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill\kuviojoin\relbarfill}
\kuviodef\xxllleftarrowxfill{\relbarfill\kuviojoin\relbarfill
   \kuviojoin\llleftarrowfill\kuviojoin\relbarfill}

\kuviodef\rrrightarrowxfill{\rrrightarrowfill\kuviojoin\relbarfill}
\kuviodef\rrrightarrowxxfill{\rrrightarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill}
\kuviodef\xrrrightarrowxfill{\relbarfill\kuviojoin\rrrightarrowfill
   \kuviojoin\relbarfill}
\kuviodef\rrrightarrowxxxfill{\rrrightarrowfill\kuviojoin\relbarfill
   \kuviojoin\relbarfill\kuviojoin\relbarfill}
\kuviodef\xxrrrightarrowxfill{\relbarfill\kuviojoin\relbarfill
   \kuviojoin\rrrightarrowfill\kuviojoin\relbarfill}

\rekuviolet\labelstyle\scriptstyle
\rekuviolet\vertexstyle\displaystyle
\rekuviolet\diagramdot\bullet

\rekuviodef\Displaybox#1{%
   \ifvmode
      \ifinner
         \box#1%
      \else
         \vskip-\lastskip
         \vskip\baselineskip
         \box#1%
         {\advance\parskip by -\baselineskip\vskip-\parskip}%
      \fi
   \else
      \box#1%
   \fi}

\kuviocs\grid=1cm
\kuviocs\range=1

\Diagrampad=5pt
\Figurepad=0pt
\Graphpad=0pt

\kuviocs\vpad=0pt
\kuviocs\hpad=0pt

\kuviocs\gridgray=.5
\kuviocs\framegray=0
\kuviocs\shadegray=0
\kuviocs\graygray=.5

\kuviocs\framepad=5pt
\kuviocs\framerulewidth=.4pt
\kuviocs\Framerulewidth=.4pt
\kuviocs\Rulewidth=5pt

\kuviocs\celllength=1cm
\kuviocs\cellwidth=1cm
\kuviocs\columndist=15mm
\kuviocs\bracewidth=1cm

\labelpoint=.5
\labelpoint{Fillcell}={}
\labelpoint{Boxcell}={}
\labelpoint{Rule}={}

\ptpoint=.5
\ptpoint{Fillcell}={}
\ptpoint{Boxcell}={}
\ptpoint{Rule}={}

\labelwidthpad=5pt
\labelwidthpad{Fillcell}=0pt
\labelwidthpad{Boxcell}=0pt
\labelwidthpad{Rule}=0pt

\labelpad=3pt
\labelpad{Fillcell}=0pt
\labelpad{Boxcell}=0pt
\labelpad{Rule}=0pt

\breakpad=2.5pt
\breakpad{Fillcell}=0pt
\breakpad{Boxcell}=0pt
\breakpad{Rule}=0pt

\cellpush=2pt
\cellpush{Fillcell}=0pt
\cellpush{Boxcell}=0pt
\cellpush{Rule}=1pt

\ptpush=0pt
\ptpush{Fillcell}=0pt
\ptpush{Boxcell}=0pt
\ptpush{Rule}=1pt

\atpush=3pt
\atpush{Fillcell}=0pt
\atpush{Boxcell}=0pt
\atpush{Rule}=0pt

\joinpush=-1pt
\joinpush{Fillcell}=0pt
\joinpush{Boxcell}=0pt
\joinpush{Rule}=1pt

\newcell{To}
\rekuviolet\Tofill\rightarrowfill

\newcell{One}
\rekuviolet\Onefill\rightarrowfill

\newcell{Bij}
\rekuviolet\Bijfill\leftrightarrowfill

\newcell{Mapsto}
\rekuviolet\Mapstofill\mapstofill

\newcell{Into}
\rekuviolet\Intofill\rightintofill

\newcell{Epi}
\rekuviolet\Epifill\rightepifill

\newcell{Line}
\rekuviolet\Linefill\linefill

\newcell{Nul}
\rekuviolet\Nulfill\hfil

\newcell{Dots}
\rekuviolet\Dotsfill\cdotfill

\newcell{Two}
\rekuviolet\Twofill\Rightarrowfill
\labelpad{Two}=.8pt
\atpush{Two}=.8pt
\breakpad{Two}=.8pt

\newcell{Impl}
\rekuviolet\Implfill\Rightarrowfill
\labelpad{Impl}=.8pt
\atpush{Impl}=.8pt
\breakpad{Impl}=.8pt

\newcell{Bar}
\rekuviolet\Barfill\barfill
\labelpad{Bar}=.8pt
\atpush{Bar}=.8pt
\breakpad{Bar}=.8pt

\newcell{Null}
\rekuviolet\Nullfill\hfil
\labelpad{Null}=.8pt
\atpush{Null}=.8pt
\breakpad{Null}=.8pt

\newcell{Eq}
\rekuviodef\Eqfill{\hfil=\hfil}
\labelpad{Eq}=.8pt
\atpush{Eq}=.8pt
\breakpad{Eq}=.8pt

\newDiagram{Diag}
\rekuviodef\everyDiag{\kuviocs\flexible\kuviocs\xgrid=0pt}

\newDiagram{Dg}
\rekuviodef\everyDg{\kuviocs\flexible\kuviocs\xgrid=0pt
   \kuviocs\ygrid+=-2mm\kuviocs\cellwidth+=3mm
   \kuviocs\bracewidth+=-2.5mm}

\newDiagram{Long}
\rekuviodef\everyLong{\kuviocs\flexible\kuviocs\xgrid=0pt
   \kuviocs\ygrid+=-5mm\kuviocs\bracewidth+=-2.5mm}

\def\inputarrsy{\input arrsy\relax}
\rekuviodefine{\long\def}\arrsy{
   \inputarrsy

   \rekuviolet\epi\rightepi
   \rekuviolet\mono\rightmono

   \newfill{Leftharpoonup}\A@Leftharpoonup==
   \rekuviolet\Leftparafill\Leftharpoonupfill
   \newfill{Leftharpoondown}\A@Leftharpoondown==
   \rekuviolet\Leftallofill\Leftharpoondownfill

   \newfill{Rightharpoonup}==\A@Rightharpoonup
   \rekuviolet\Rightallofill\Rightharpoonupfill
   \newfill{Rightharpoondown}==\A@Rightharpoondown
   \rekuviolet\Rightparafill\Rightharpoondownfill

   \newfill{Lleftarrow}\A@Lleftarrow\A@Rrelbar\A@Rrelbar
   \newfill{Rrightarrow}\A@Rrelbar\A@Rrelbar\A@Rrightarrow
   \newfill{Rrelbar}\A@Rrelbar\A@Rrelbar\A@Rrelbar
   \rekuviolet\equivfill\Rrelbarfill
   \newfill{Lleftrightarrow}\A@Lleftarrow\A@Rrelbar\A@Rrightarrow

   \newfill{dashbar}{\mkern8mu}\A@dashbar{\mkern8mu}
   \rekuviolet\dashfill\dashbarfill
   \newfill{rightdash}{\mkern8mu}\A@dashbar\A@shortrightarrow
   \newfill{leftdash}\A@shortleftarrow\A@dashbar{\mkern8mu}

   \newfill{rightepi}--\A@rightepi
   \newfill{leftepi}\A@leftepi--
   \newfill{rightmono}{\A@rightmonotail\mkern2mu}-\A@rightarrow
   \newfill{leftmono}\A@leftarrow-{\mkern2mu\A@leftmonotail}
   \newfill{rightmonotail}{\A@rightmonotail\mkern2mu}--
   \newfill{leftmonotail}--{\mkern2mu\A@leftmonotail}
   \newfill{rightiso}{\A@rightmonotail\mkern2mu}-\A@rightepi
   \newfill{leftiso}\A@leftepi-{\mkern2mu\A@leftmonotail}

   \newfill{rightdashmono}{\A@rightmonotail\mkern2mu}\A@dashbar
      \A@shortrightarrow
   \newfill{leftdashmono}\A@shortleftarrow\A@dashbar{\mkern2mu\A@leftmonotail}
   \newfill{rightdashmonotail}{\A@rightmonotail\mkern2mu}\A@dashbar{\mkern8mu}
   \newfill{leftdashmonotail}{\mkern8mu}\A@dashbar{\mkern2mu\A@leftmonotail}
   \newfill{rightdashepi}{\mkern8mu}\A@dashbar
      {\mkern-2.5mu\A@shortrightarrow\mkern-7.5mu\A@shortrightarrow}
   \newfill{leftdashepi}{\A@shortleftarrow\mkern-7.5mu\A@shortleftarrow
      \mkern-2.5mu}\A@dashbar{\mkern8mu}
   \newfill{rightdashiso}{\A@rightmonotail\mkern4mu}\A@dashbar
      {\mkern-2.5mu\A@shortrightarrow\mkern-7.5mu\A@shortrightarrow}
   \newfill{leftdashiso}{\A@shortleftarrow\mkern-7.5mu\A@shortleftarrow
      \mkern-2.5mu}\A@dashbar{\mkern4mu\A@leftmonotail}

   \newfill{squiggle}{\mkern8mu}\A@squiggle{\mkern8mu}

   \newcell{Allo}
   \rekuviolet\Allofill\Rightallofill
   \labelpad{Allo}=.8pt
   \atpush{Allo}=.8pt
   \breakpad{Allo}=.8pt

   \newcell{Para}
   \rekuviolet\Parafill\Rightparafill
   \labelpad{Para}=.8pt
   \atpush{Para}=.8pt
   \breakpad{Para}=.8pt

   \newcell{Three}
   \rekuviolet\Threefill\Rrightarrowfill
   \labelpad{Three}=1.5pt
   \atpush{Three}=1.5pt
   \breakpad{Three}=1.5pt

   \newcell{Equiv}
   \rekuviolet\Equivfill\Rrelbarfill
   \labelpad{Equiv}=1.5pt
   \atpush{Equiv}=1.5pt
   \breakpad{Equiv}=1.5pt

   \newcell{Nulll}
   \rekuviolet\Nulllfill\hfil
   \labelpad{Nulll}=1.5pt
   \atpush{Nulll}=1.5pt
   \breakpad{Nulll}=1.5pt

   \newcell{Dash}
   \rekuviolet\Dashfill\dashfill

   \newcell{Dashto}
   \rekuviolet\Dashtofill\rightdashfill

   \newcell{Mono}
   \rekuviolet\Monofill\rightmonofill

   \newcell{Tail}
   \rekuviolet\Tailfill\rightmonotailfill

   \newcell{Iso}
   \rekuviolet\Isofill\rightisofill
}

\kuviobye

%  kuvio.fw:  $Revision: 2.8 $
%  COPYRIGHT.fw:  $Revision: 1.2 $
%  Diagrams.fw:  $Revision: 1.72 $
%  _prepare.fw:  $Revision: 2.75 $
%  _parse.fw:  $Revision: 1.13 $
%  _process.fw:  $Revision: 2.31 $
%  _explode.fw:  $Revision: 2.44 $
%  _setnodes.fw:  $Revision: 1.26 $
%  _setcells.fw:  $Revision: 2.30 $
%  _place.fw:  $Revision: 2.51 $
%  _modify.fw:  $Revision: 2.47 $
%  _display.fw:  $Revision: 1.42 $
%  Cells.fw:  $Revision: 1.29 $
%  _cellmod.fw:  $Revision: 2.37 $
%  _cellentry.fw:  $Revision: 1.45 $
%  _extent.fw:  $Revision: 2.10 $
%  _predefined.fw:  $Revision: 1.23 $
%  Labelling.fw:  $Revision: 2.33 $
%  Registers.fw:  $Revision: 2.26 $
%  Fill.fw:  $Revision: 1.19 $
%  Arrsy.fw:  $Revision: 1.19 $
%  macros.fw:  $Revision: 1.15 $

%  Tangle completed Mon Feb 19 13:43:03 PST 1996.
%  Mangle completed Mon Feb 19 13:43:15 PST 1996.

